Runtime Variation in Big Data Analytics

The dynamic nature of resource allocation and runtime conditions on Cloud can result in high variability in a job's runtime across multiple iterations, leading to a poor experience. Identifying the sources of such variation and being able to predict and adjust for them is crucial to cloud service providers to design reliable data processing pipelines, provision and allocate resources, adjust pricing services, meet SLOs and debug performance hazards. In this paper, we analyze the runtime variation of millions of production SCOPE jobs on Cosmos, an exabyte-scale internal analytics platform at Microsoft. We propose an innovative 2-step approach to predict job runtime distribution by characterizing typical distribution shapes combined with a classification model with an average accuracy of >96%, out-performing traditional regression models and better capturing long tails. We examine factors such as job plan characteristics and inputs, resource allocation, physical cluster heterogeneity and utilization, and scheduling policies. To the best of our knowledge, this is the first study on predicting categories of runtime distributions for enterprise analytics workloads at scale. Furthermore, we examine how our methods can be used to analyze what-if scenarios, focusing on the impact of resource allocation, scheduling, and physical cluster provisioning decisions on a job's runtime consistency and predictability.

==> Background.tex <==
\section{Platform and Datasets}
\label{sec:bg}

%\subsection{Background}
\cosmos is an exabyte-scale big data platform developed at \msft since 2002~\cite{power2021cosmos}, consisting of more than 300k machines across multiple data centers worldwide~\cite{zhu2021kea}. Using a YARN-based~\cite{vavilapalli2013apache} resource manager, the system processes >600k jobs per day from tens of thousands of \msft internal users. Each job can be authored using a SQL-like dialect, named SCOPE~\cite{boutin2015jetscope} with heavy use of C\verb|#| and user-defined functions (UDFs). Upon submission, the job will be compiled to an optimized execution plan as a DAG of operators and distributed across different machines.
Over the past decades, a multitude of research projects and engineering efforts have been designated to improve its efficiency, security, scalability and reliability~\cite{jindal2019peregrine, zhang2012optimizing, bruno2012recurring, bruno2013continuous,boutin2014apollo,boutin2015jetscope,karanasos2015mercury,jyothi2016morpheus,curino2019hydra,qiao2019hyper,chaiken2008scope,ferguson2012jockey,ramakrishnan2017azure,zhou2012advanced,zhu2021kea,zhou2010incorporating,wing2020osdi,phoebe,sen2021autoexecutor}. As a result, \cosmos operates at consistently high utilization (>70\%) and low failure rates~\cite{zhu2021kea}. 

\subsection{Job Groups}
In this work, we focus on understanding and predicting the variation in run times over repeated runs of jobs. Variation is meaningful only when jobs recur (i.e., sample size $>$ 1). Prior studies~\cite{jyothi2016morpheus,wing2020osdi,phoebe} have shown that 40--60\% of jobs on Cosmos are recurring jobs. We identify recurrences by matching on a key that combines the following.
\begin{enumerate}[leftmargin=*]
    \item The normalized job name, which is the job name with specific information like submission time and input data set removed~\cite{phoebe,jindal2019peregrine}. 
    \item The job signature~\cite{jindal2019peregrine}, which is a hash value computed recursively over the DAG of operators in the compiled plan. The signature does not include job input parameters.
\end{enumerate}
We thus have \textit{job groups} and \textit{job instances} belonging to each group, corresponding to recurrences of the job. Job instances have the same key value within each job group.

\subsection{Potential Sources of Variation}
\label{subsec:sources-of-variation}

Within each job group, the run times of job instances can vary due to any of the following reasons.

\textbf{Intrinsic Characteristics}: The key used for grouping jobs includes information on their execution plan (e.g., type of operators, estimated cardinality, dependency between operators) while not including the job input parameters (e.g., parameters for filter predicates) or input data sets. Different instances can have different values for these parameters, data sets, and their sizes. This can lead to different run times within the group if the parameter changes are not accompanied by a change in the compiled plan. In our datasets, we have observed input data sizes vary by a factor of 50 within the same job group.

\begin{figure}
	\centering
		\includegraphics[width=\columnwidth]{img/tokenusage.pdf}
	\caption{Token usage for an example job during its run.
	}\label{fig:token}
\end{figure}
\textbf{Resource Allocation}: On \cosmos, the unit of resource allocation is a \textit{token}~\cite{power2021cosmos}, which is analogous to the notion of a container. The number of tokens guaranteed for a job can be specified by users at the time of job submission or it may be recommended by the system~\cite{autotoken}. To further improve the utilization of the existing infrastructure, unused resources are repurposed as pre-emptive opportunistic tokens~\cite{boutin2014apollo} that can be leveraged by any jobs freely. Though their availability is less predictive, which often results in longer or shorter run times. Figure~\ref{fig:token} shows the skyline of token usage for a \cosmos job that was allocated with 66 tokens; including opportunistic tokens it used up to 198 tokens in total throughout its processing time. 

The maximum number of tokens ultimately utilized by a job depends on how much parallelism it can exploit subject to the number of tokens allocated to it (guaranteed and opportunistic). In our datasets, we have observed maximum token counts vary by a factor of 10 within the same job group.

%To better manage the capacity of such enormous infrastructure, the concept of ``\textit{tokens}'' was introduced to control the amount of resources, measured by the number of containers, that can be allocated to a particular job~\cite{power2021cosmos}. 
%The allocated tokens can be specified by customers to limit the maximum number of resource that can be used simultaneously. 

While the number of tokens indicate the amount of resources used, there is also variation in the characteristics of allocated resources. Tokens map to computational resources on SKUs, and being established over the decade, the \cosmos cluster consists of 10--20 different SKUs\footnote{Stock Keeping Unit} with different processing speeds~\cite{zhu2021kea}. In our datasets, we have observed different job instances within the same job group run on 1 to 9 different SKU types.

%some of the newer generation of machines have faster processing speed~\cite{zhu2021kea} 

\begin{figure}
	\centering
	\centering
	\includegraphics[width=.6\columnwidth]{img/cpu.pdf}
	\caption{CPU utilization for different SKUs in one of the \cosmos clusters.
	}\label{fig:cpu}
\end{figure}
\textbf{Cluster Conditions}: Finally, cluster conditions can also lead to variations in run times. This includes both the availability of opportunistic tokens (discussed above) as well as load on the individual machines. Figure~\ref{fig:cpu} shows significant differences in the CPU utilizations of machines with different SKU types in one of the \cosmos clusters. For example, 
utilization for Gen6 varies from 2\% to 33\% with an average of 17\% whereas for Gen3.5 it varies from 10\% to 100\% with an average of 68\%.
Higher utilizations (loads) are likely to cause more contention for shared resources, and a larger range of loads may increase variation in run times.

\subsection{Datasets}

Since we want to develop insights into the various potential sources of variation as discussed above, we collected data along those dimensions from production workloads on our clusters. We extract information about intrinsic characteristics such as operator counts in the plan, input data sizes, and cardinalities, costs, etc. estimated by the SCOPE optimizer using the Peregrine framework~\cite{jindal2019peregrine}. We obtain token usage information from the job execution logs, and SKU and machine load information using the KEA framework~\cite{zhu2021kea}. Finally we join all this information together by matching on the job ID, machine name that execute each vertex and the corresponding job submission time.

\begin{table}[ht]
\centering
\caption{Datasets used for this study. \textit{Support} denotes the minimum number of job instances per group. We include groups after filtering for this criteria.}
\label{tab:datasets}
\resizebox{\columnwidth}{!}{\begin{tabular}{|c|c|c|c|c|}\hline
     \textbf{Dataset}&  \textbf{Interval}& \textbf{Job Groups}& \textbf{Job Instances}& \textbf{Support}\\\hline\hline
     \textbf{D1}& 6 months& 9.5K& 3.2M& 20\\\hline
     \textbf{D2}& 15 days& 11.9K& 737K& 3\\\hline
     \textbf{D3}& 5 days& 11.6K& 215K& 3\\\hline
\end{tabular}}
\end{table}
Table~\ref{tab:datasets} summarizes the datasets that we use for our study. The datasets consist of a subset of jobs run over the corresponding interval, and are included if the number of instances per group (support) exceeds a minimum theshold. We use dataset D1 to identify and group distributions of run times (see Section~\ref{sec:clustering} for details). We used dataset D2 to train a predictor for run time variation and dataset D3 to test the accuracy of the predictor (Section~\ref{sec:model}).

%In this analysis, we set-off to gather data at the job-template level, which indicates a series of recurrent jobs processing different input data sources. To evaluate the reasoning of the variances, we combine a multitude of data sources, including (1) a set of environmental variables (including the utilization of each computing machine) that reflects the system status of the execution environment, (2) job characteristics (such as information for the execution plan) to indentify the type of jobs can potentially have higher runtime variation, and (3) resource usage for a particular job as the input to the estimators to predict the coefficient of variance of the job runtime. 


\section{Characterizing Runtime Variation}
\label{sec:metrics}

We now discuss how we characterize and quantify run time variation for recurring jobs. This will form the basis for our prediction strategy that we dicuss in Section~\ref{sec:model}.

\subsection{Scalar Metrics}

As we discussed previously (Section~\ref{sec:intro}), a job's average run time does not give much insight into variations across repeated runs, or how long the next run of the job will take. Thus, it is not very useful for characterizing, predicting, or explaining the variations.

\begin{figure}
	\centering
		\subfloat[Historic Median vs Run Times]{\includegraphics[width=0.5\columnwidth]{img/median_compare_train_all.png}\label{fig:median-vs-runtime}}
		\subfloat[Historic COV vs COV]{\includegraphics[width=0.5\columnwidth]{img/cov2.png}\label{fig:cov-as-predictor}}
	\caption{Correlations between historic median run time and job run times, and historic COV and COV of all run times observations.}
	%{Job runtime/COV compared with historic median/COV.}
	\label{fig:medianbenchmark}
\end{figure}
Next, we investigate how well a job's median run time is correlated with run times over the different repetitions of the job. Figure~\ref{fig:median-vs-runtime} shows how the run times for individual repetitions of the job compared with its historic median using dataset D2. 
\yz{from Bob: I think you should point out that the stalagmite is offset from the diagonal by a fixed amount of time. This is a bigger relative delay for faster-running jobs, while for very long-running jobs this delay makes only a small difference in the total runtime (which is why a constant time delay looks curved in log space).}

We observe two distinct patterns in the figure---a set of points are clustered along the diagonal, indicating a good correlation of individual run times to the median, whereas another set of points are clustered separately in a pattern resembling a stalagmite\footnote{A stalagmite is a rocky formation that arises from the floor of a cave and may reach the ceiling~\cite{stalagmite}.}. The runs corresponding to the points in the stalagmite are much slower than the median run time and contribute to the (long) tail of the run time distributions. Such runs are rare (comprising less than 5\% of all runs), with the probability reducing with larger median values. But we have found it to be very difficult to predict upfront if the time for a new run will end up on the diagonal or on the stalagmite. The existence of these two patterns, as well as the difficulty of predicting to which pattern a new run will belong, even if the median run time is stable and known, makes the median a poor choice to use for predicting run times or for characterizing variations. A similar trend can be found for the average and $95^{th}$ percentile of historic runtime (see Figure~\ref{fig:avgbenchmark}).

\begin{figure}
	\centering
		\subfloat[Historic Average vs Runtimes]{\includegraphics[width=0.5\columnwidth]{img/avg_compare_train_all.png}\label{fig:avg-vs-runtime}}
		\subfloat[$95^{th}$ Percentile vs Runtimes]{\includegraphics[width=0.5\columnwidth]{img/p95_compare_train_all.png}\label{fig:95-vs-runtime}}
	\caption{Correlations between historic average/$95^{th}$ percentile and job runtimes using dataset D2.}
	%{Job runtime/COV compared with historic median/COV.}
	\label{fig:avgbenchmark}
\end{figure}

% \todo{can we discuss what happens with 95\% or some other quantile vs run time?}

Coefficient of Variation (COV) is another commonly-used metric that is used to characterize variation. It is defined as the ratio of standard deviation to the average, and is an unitless quantity. COV is straight-forward to compute and interpret. Prior work~\cite{schad:ec2-variance:vldb:2010} has used COV to characterize variation in job run times.
%
%Coefficient of Variation (COV), defined by the ratio of standard deviation to the average, is a commonly used metric to evaluate runtime variation. 
%
However, using COV also has several limitations as follows.
\begin{enumerate}[leftmargin=*]
    \item \textbf{Bias}: The run times of SCOPE jobs that we study range from seconds to days, with significant differences in the average values. This may cause COV to be biased and one could always observe very large COV for short-running jobs.
    \item \textbf{Instability}: The average run times can increase due to the existence of outliers (in such large distributed systems, some jobs inevitably run slow occasionally). Thus, COV can be unstable with addition of more jobs in the dataset. Unlike the average, COV does not converge with large sample size thus does not have a consistent estimator~\cite{fischer2011history}.
    \item \textbf{Coarse-grained}: COV does not capture many characteristics of a distribution, such as its shape (such as unimodal, bimodal, and the existence of outliers). Hence, it cannot readily explain variation in a fine-grained manner.
    % \item \textbf{Lack of convergence}: COV does not converge with sample size thus does not have a consistent estimator \yz{look this up}. So, in this case, it is less predictable and less stable.\todo{are (2) and (4) different, or can they be combined?}
\end{enumerate}

Figure~\ref{fig:cov-as-predictor} shows how well the COV computed from historic runs for each job instance compares with COV of times from all runs in D3. Similar to the discussion for medians above, we see multiple groups of points, with the same historic COV appearing for different COV values from new runs and it is difficult to predict for a new run to which group it will belong. Additionally, the COV metric suffers from the limitations mentioned above. 

Overall, we found that scalar metrics such as average, median, quantiles, and COV by themselves are not sufficient for understanding or predicting run time variations. 

%Several interesting findings: 

%i) a stalagmite can be observed from the left figure, indicating a group of job instances that are much slower than median runtime. By further examining those jobs, we found little evidence for their slow down reasons. Most of those jobs share no differences with other job instances that have the same job template. The occurrences are also rare (less than 5\% of job instances might encounter such slow down, and it is un-predictable). And for job templates with less occurrences, one might not observe such cases at all. Therefore, we turn to predict the existence of those job instances and their probability (see Section~\ref{sec:model}) as opposed to predicting the runtime of each job instances (or whether the job instance will be in such stalagmite).

%COV is much less predictable with historic data due to the reasons mentioned before. For customer jobs, it would be interesting to infer the probability of such slow downs with better predictors. Therefore, we change our focus on this paper to the distribution of the jobs and its detailed shapes.

\subsection{Distributions}
\label{sec:clustering}

We now turn to characterizing variations based on the detailed \textit{runtime distribution} for each recurrent job group. Although there is a large variety in the run times of SCOPE jobs, we found that many different jobs have similar shapes of their run time distribution curves. So, we first normalize the job run times, then compute their distributions, and finally group them based on similarity. This helps to generalize the analysis across similar distributions from different jobs and reduce the number of groupings to a small number that can be more easily understood and kept track of by the users.

%moreover, to better generalize the analysis across different jobs which might have significantly different ranges of job runtime (but might share similar variation/shape of distribution), we normalize the job runtime by:

We use the following two normalization strategies, corresponding to different usage scenarios, for the job run times.
\begin{enumerate}[leftmargin=*]
	\item \textbf{\rationorm}: we take the ratio of job run time to median run time. For this scenario, we are interested in understanding the similarity in variation in terms of percentage change in run times.
	\item \textbf{\deltanorm}: we take the difference of the two, i.e., job run time - median run time. For this scenario, we are interested in understanding the the similarity in variation in terms of absolute change (seconds) in run times.
\end{enumerate}  

%We believe that both the distributions of the normalized runtime by \rationorm and \deltanorm are important in different scenarios. The ratio indicates the percentage variation benchmarked to the median, while the \deltanorm reveals the absolute deviation in the unit of seconds/minutes. 


To better examine the ``typical'' distribution shape across jobs with different templates, we conduct a clustering analysis using 2021-June to 2021-Nov's data with 3.2M job instances and 9,532 job groups with $\geq 20$ occurrences in the whole period (see D1 in Table~\ref{tab:datasets}). For each job group, we derive its histogram for the distribution of normalized runtime and then use un-supervised machine learning algorithm for the clustering. 

Our principal design choices for the runtime distribution clustering method is as the following:
\begin{itemize}[leftmargin=*]
%	\item For the clustering analysis, we want to evaluate the distribution of runtime variances. In this case, we normalize the runtime by its median value in this distribution. There can be two possible way for this normalization: (1) divided by the median runtime to consider the ratio between the instance's runtime benchmarked to the median or (2) minus the median runtime to consdier the absolute deviation from the median time. Maybe we can use either one that has better predictability, i.e., if jobs runtime variation has more consistency measured in \% changes, we can use this as the prediction value and we can convert to the absolute runtime deviation. Similar for the inverse.
	\item \textbf{Bin size and Range}: For calculating the distribution of the normalized runtime, the design of the bin size and range is critical. The range should cover the majority of the values with relatively fine granularity (but not too small such that we will have a lot of fluctuation due to noises in the derived distribution). We also want to cover the outliers (points in the stalagmites, that is, tails of the distributions) such that we can predict their probability of existence. Since they are rare, we merge the outliers into one bin in this distribution (based on being $\leq$ or $\geq$ some threshold). For \deltanorm, we use [-900, 900] (where <2\% of jobs are more than 900s slower than median, and for \rationorm, we use [0, 10] (where <1.5\% of jobs are 10x slower than median. Jobs with >900s or 10x slower than median are defined as outliers. For the bins size, we evaluated 50, 100, 200 and 500 bins, and chose 200 bins that has relatively smooth PDF curves and a sufficient level of granularity.
\item \textbf{Clustering algorithm}: We evaluated several clustering algorithms. Hierarchy clustering using dendrogram~\cite{nielsen2016introduction} and Agglomerative clustering~\cite{rokach2005clustering} are both flexible and can use different distance metrics and linkage methods, and users can specify the number of clusters to be formed. However, they both result in imbalanced clusters (some with >90\% of the jobs groups in one cluster). K-means clustering~\cite{sculley2010web} results in balanced clusters and can also take number of clusters as input. Therefore, we use this K-means clustering for the following analysis. 
	\item \textbf{Number of Clusters}: We determined the the number of clusters based on: (i) numeric measurements---we examine the decrease of \textit{inertia}, defined by the sum of squared distances between each sample and its cluster centroid and pick an elbow point where adding more clusters does not decrease the inertia by a significant amount, and (ii) by visually examining the clustering results to check if the clusters are sufficiently different from each other and have unique characteristics. We picked 8 clusters for both \deltanorm and \rationorm for consistency.
	\item \textbf{Smoothing histograms}: While doing the above analysis, we faced a limitation in the standard clustering algorithms---they are based on using probability density function (PDF) values as input vectors without considering the correlation between each bin. In reality, we also want to consider if adjacent density values of bins (e.g., the probability of a run time being in the $4^{th}$ or the $5^{th}$ bin) are correlated with each other. However, with any distance measurement (such as dot product), similarity between adjacent bins are not considered.
% 	whereas it is easy to observe cases where for job A, its $4^{th}$ bin's value equals to that of the $5^{th}$ bin for job B due to random noises. 
	Therefore, we introduce a \textit{smoothing step} after deriving the PDFs to reduce the difference between any two adjacent bins such that the two smoothed vectors mentioned above will have higher similarity. A carefully chosen bin size (as discussed above) will also help in this situation to reduce the impact of noises. 
\end{itemize}



%\begin{figure}
%	\centering
%	\centering
%	\begin{minipage}[b]{\columnwidth}
%		\includegraphics[width=\textwidth]{img/hist_normed_kmeans_8_bins_merge_tail_ratio0210_min_3/cluster_all.pdf}
%	\end{minipage}%
%	
%	\begin{minipage}[b]{\columnwidth}
%		\includegraphics[width=\textwidth]{img/hist_normed_kmeans_8_bins_merge_tail_delta0210_min_3/cluster_all.pdf}
%	\end{minipage}%
%	% 	\vspace{-3mm}
%	\caption{8 typical distribution of normalized runtime.
%	}\label{fig:clustering}
%\end{figure} 

Figure~\ref{fig:clustering} shows the distribution for the 8 clusters using \rationorm and \deltanorm policies. We can see that some distributions have two modes (e.g., Cluster 0,2 and 4 using \rationorm) and with different variances. Table~\ref{tab:statscluster} summarizes important statistics for each cluster. For example, for Cluster 0 with \rationorm, it contains 36.5\% of the total job observations; its outlier probability is 1.63\% (defined by $\geq 10$x slower than median for \rationorm); the difference between 25 and $75^{th}$ percentile is 0.06; the $95^{th}$ percentile of this distribution is 1.41, and the standard deviation is 2.46. While for Cluster 7 with \rationorm, the outlier probability decreases to 0.06\%. Clusters are ranked according to the difference between 25 and $75^{th}$ percentile.
\begin{figure}
	\centering
	\centering
	\begin{minipage}[b]{\columnwidth}
		\includegraphics[width=\textwidth]{img/hist_normed_kmeans_8_bins_merge_tail_ratio0210_min_3/cluster_all_idx_cut.pdf}
	\end{minipage}%
	
	\begin{minipage}[b]{\columnwidth}
		\includegraphics[width=\textwidth]{img/hist_normed_kmeans_8_bins_merge_tail_delta0210_min_3/cluster_all_idx_cut.pdf}
	\end{minipage}%
	% 	\vspace{-3mm}
	\caption{8 typical distribution of normalized runtime.
	}\label{fig:clustering}
\end{figure} 


% \begin{table}[]
% 	\begin{tabular}{llllllll}
% 		\toprule
% 		\multicolumn{4}{c}{Ratio}              & \multicolumn{4}{c}{Delta}             \\ \midrule
% 		cid & outlier & 25-75th         & 95th  & cid & outlier & 25-75th      & 95th    \\ \midrule
% 		0   & 0.25\%  & 0.15            & 1.31 & 0   & 0.01\%  & $\leq$3      & 13.57  \\
% 		1   & 1.63\%  & $\leq$0.02      & 1.31 & 1   & 0.04\%  & 162.81       & 502.01 \\
% 		2   & 0.25\%  & 0.15            & 1.31 & 2   & 0.00\%  & 9.05         & 22.61  \\
% 		3   & 0.06\%  & \textbf{0.20}           & \textbf{1.66} & 3   & 0.01\%  & 18.09        & 40.70  \\
% 		4   & 0.42\%  & 0.05            & 1.16 & 4   & 0.03\%  & 72.36        & 185.43 \\
% 		5   & 0.26\%  & 0.15            & 1.36 & 5   & 0.00\%  & $\leq$3      & 4.52   \\
% 		6   & \textbf{1.66\%}  & 0.10            & 1.41 & 6   & \textbf{0.26\%}  & \textbf{1591.96}    & \textbf{890.95} \\
% 		7   & 1.46\%  & 0.10            & 1.26 & 7   & 0.00\%  & $\leq$3      & 4.52  \\\bottomrule
% 	\end{tabular}
% 	\caption{Other statistics for 8 clusters.
% }\label{tab:statscluster0}
% \end{table}

% \begin{table}[]
% 	\caption{Other statistics for 8 clusters.}\label{tab:statscluster}
% \begin{adjustbox}{max width=\columnwidth}
% \begin{tabular}{lllp{0.5cm}lllllp{0.5cm}ll}
% 		\toprule
% \multicolumn{5}{c}{Ratio}             & \multicolumn{5}{c}{Delta}             \\\midrule
% cid &\% jobs& outlier & $25-75^{th}$ & $95^{th}$ & std & cid &\% jobs & outlier & $25-75^{th}$ & $95^{th}$ & std \\\midrule
% 0   &10.0& 0.25\%  & 0.17    & 1.29 & 1.45          & 0 &\textbf{40.8}&  1.93\%  & 4       & 28   & 155  \\
% 1   & \textbf{36.5}& 1.63\%  & 0.06    & 1.41 & \textbf{2.46} & 1 &9.2  & 2.43\%  & 199     & 408  & 296  \\
% 2   & 7.9& 0.25\%  & 0.19    & 1.34 & 0.82          & 2 &8.3  & 0.55\%  & 16      & 33   & 140  \\
% 3   &6.3& 0.06\%  &\textbf{0.29}& \textbf{1.46} & 0.55 & 3 &14.6  & 0.98\%  & 31      & 63   & 153  \\
% 4   &13.7& 0.42\%  & 0.11    & 1.20 & 0.93              & 4 &12.2  & 0.73\%  & 69      & 128  & 179  \\
% 5   & 9.8& 0.26\%  & 0.20    & 1.37 & 0.97              & 5 &5.7  & 0.49\%  & 11      & 19   & 140  \\
% 6   & 10.2& \textbf{1.66\%}  & 0.16    & 1.37 & 2.18     & 6 &1.7  & \textbf{24.23\%} & \textbf{936}     & \textbf{1359} & \textbf{2548} \\
% 7   & 5.6& 1.46\%  & 0.17    & 1.35 & 1.94              & 7 &7.6  & 0.53\%  & 11      & 23   & 148 \\\bottomrule
% \end{tabular}
% \end{adjustbox}
% \end{table}
% \todo{sort clusters by some characteristic, e.g., 25-75th width, so that readers can have a mental model that puts clusters numbers on a spectrum for that characteristic. Explain the semantics. Explain the first and last row of the table. Also arrange above cluster plot accordingly.}

\begin{table}[]
	\caption{Other statistics for the clusters.}\label{tab:statscluster}
\begin{adjustbox}{max width=\columnwidth}
\begin{tabular}{lllp{0.5cm}lllllp{1.0cm}p{0.8cm}l}
		\toprule
\multicolumn{5}{c}{Ratio}             & \multicolumn{5}{c}{Delta}             \\\midrule
cid &\% jobs& outlier & $25-75^{th}$ & $95^{th}$ & std & cid &\% jobs & outlier & $25-75^{th}$ (s)& $95^{th}$ (s)& std (s)\\\midrule
0   & \textbf{36.5} & 1.63\%                           & 0.06 & 1.41                           & \textbf{2.46} & 0  & \textbf{40.8} & 1.93\%                            & 4   & 28                             & 155                            \\
1   & 13.7                           & 0.42\%                           & 0.11 & 1.2                            & 0.93                           & 1  & 5.7  & 0.49\%                            & 11  & 19                             & 140                            \\
2   & 10.2                           & \textbf{1.66\%} & 0.16 & 1.37                           & 2.18                           & 2  & 7.6  & 0.53\%                            & 11  & 23                             & 148                            \\
3   & 10.0                             & 0.25\%                           & 0.17 & 1.29                           & 1.45                           & 3  & 8.3  & 0.55\%                            & 16  & 33                             & 140                            \\
4   & 5.6                            & 1.46\%                           & 0.17 & 1.35                           & 1.94                           & 4  & 14.6 & 0.98\%                            & 31  & 63                             & 153                            \\
5   & 7.9                            & 0.25\%                           & 0.19 & 1.34                           & 0.82                           & 5  & 12.2 & 0.73\%                            & 69  & 128                            & 179                            \\
6   & 9.8                            & 0.26\%                           & 0.20  & 1.37                           & 0.97                           & 6  & 9.2  & 2.43\%                            & 199 & 408                            & 296                            \\
7   & 6.3                            & 0.06\%                           & \textbf{0.29} & \textbf{1.46} & 0.55                           & 7  & 1.7  & \textbf{24.23\%} & \textbf{936} & \textbf{1359} & \textbf{2548} \\\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}
% \todo{sort clusters by some characteristic, e.g., 25-75th width, so that readers can have a mental model that puts clusters numbers on a spectrum for that characteristic. Explain the semantics. Explain the first and last row of the table. Also arrange above cluster plot accordingly.}

%\todo{add characteristics of each cluster and analysis}
% \todo{give percentages of job groups in the clusters}




==> Bayesian.tex <==
\subsection{Bayesian Network}

\todo{explain methodology}

\todo{show an example net}

\todo{Discuss some conclusions and how they overcome limitations of the correlation-based approach}


==> Challenges_Anja.tex <==
\section{Challenges and Approach}
\label{sec:challenges}
With the rise of cloud and big data systems, we have seen a shift in how system performance can be evaluated and monitored.
Specifically, we observe that reasoning about performance changes traditionally was done by experienced engineers.
They would examine different system indicators and make a decision based on certain domain or prior knowledge which can potentially lead to biased results.
However, in a cloud environment massive telemetry data is collected on a daily basis.
This includes both information about job characteristics as well as near-real-time status of the computing clusters.
With the advent of advanced data analysis methodology, we can now leverage automated techniques to facilitate a better understanding of performance data.

However, even with advanced machine learning (ML) technology at our fingertips, performance modeling in distributed systems remains a challenge, especially if we focus on a system's reliability. We observe the following challenges for runtime modeling:
\begin{description}
\item[\bf Measuring runtime (C1).] Traditional variance-based measures are unable to capture the characteristic long-tailed distributions that we observe when measuring runtime.
\item[\bf Capturing outliers (C2).] A significant portion of the runtime outliers for a reccurrent job are due to rare events such as the occasional service disruption. Historic data needs to contain such outliers to take them into consideration for ML-based modeling.
\item[\bf Resource sharing (C3).] Big Data as well as cloud systems have shared architectures, allowing multiple users to access and interact with the system simultaneously. This results in noise and other environmentally changing factors influencing runtime measurements.
\item[\bf Repeated job execution (C4).] In order to create a useful ML-model based on prior execution statistics, we need to observe the execution of the same job multiple times. Running a job just for the purpose of modeling its runtime is infeasible for many customers.
\end{description}

\smallsection{Solution Overview}
In our work, we focus on the explanation, mitigation and prediction of runtime variation on the \textit{individual} job level instead of the full-system level.
We observe that per-job runtime estimates are highly desirable from the customer's point of view to understand and monitor the execution of their pipelines.
Estimating the variation of the runtime for a particular job is different than executing a point estimate:
It requires us to determine the distribution of observed runtimes over multiple runs of the same job.
To facilitate accurate predictions, we consider a job's properties, resource allocation, and environmental setting.

Our framework takes as input...

Our framework is built to better understand the variation of a job's runtime. We use these building blocks to achieve that:
\begin{description}
\item[\bf We define metrics.] Using historic data, we examine the typical runtime distributions of various jobs. For each type of distribution, we define key metrics to depict the distribution, and quantify the variation in numeric terms that can be easily understood by users. This addresses challenge C1.
\item[\bf We develop predictors.] Using ML classification techniques, we determine which runtime profile most likely fits a given job. To overcome challenges C2 and C3, i.e.,~outliers and resource contention, we focus on frequently recurring jobs in our analysis.
\item[\bf We explain predictions.] To better understand the various influences on runtime variation, we leverage feature contribution algorithms. Furthermore, these techniques allow us to propose job improvements based on the observed characteristics.
\end{description}

==> Predict2.tex <==

\subsection{Classic ML Predictor}

RF, EBM(?) 

\todo{show prediction accuracy}

\todo{show feature importance scores and discuss shortcomings}



%\subsection{Bayesian Network}
%
%\todo{compare with RF prediction}
%


==> Results/Experiments.tex <==
\section{Experiment}\label{sec:exp}
Bayesian net

Randomforest

Boosting Machine


==> Runtime Variation in Distributed Systems (Short II) (2)/Background.tex <==
\section{Platform and Datasets}
\label{sec:bg}

%\subsection{Background}
\cosmos is an exabyte-scale big data platform developed at \msft since 2002~\cite{power2021cosmos}, consisting of more than 300k machines across multiple data centers worldwide~\cite{zhu2021kea}. Using a YARN-based~\cite{vavilapalli2013apache} resource manager, the system processes >600k jobs per day from tens of thousands of \msft internal users. Each job can be authored using a SQL-like dialect, named SCOPE~\cite{boutin2015jetscope} with heavy use of C\verb|#| and user-defined functions (UDFs). Upon submission, the job will be compiled to an optimized execution plan as a DAG of operators and distributed across different machines.
Over the past decades, a multitude of research projects and engineering efforts have been designated to improve its efficiency, security, scalability and reliability~\cite{jindal2019peregrine, zhang2012optimizing, bruno2012recurring, bruno2013continuous,boutin2014apollo,boutin2015jetscope,karanasos2015mercury,jyothi2016morpheus,curino2019hydra,qiao2019hyper,chaiken2008scope,ferguson2012jockey,ramakrishnan2017azure,zhou2012advanced,zhu2021kea,zhou2010incorporating,wing2020osdi,phoebe,sen2021autoexecutor}. As a result, \cosmos operates at consistently high utilization (>70\%) and low failure rates~\cite{zhu2021kea}. 

\subsection{Job Groups}
In this work, we focus on understanding and predicting the variation in run times over repeated runs of jobs. Variation is meaningful only when jobs recur (i.e., sample size $>$ 1). Prior studies~\cite{jyothi2016morpheus,wing2020osdi,phoebe} have shown that 40--60\% of jobs on Cosmos are recurring jobs. We identify recurrences by matching on a key that combines the following.
\begin{enumerate}[leftmargin=*]
    \item The normalized job name, which is the job name with specific information like submission time and input data set removed~\cite{phoebe,jindal2019peregrine}. 
    \item The job signature~\cite{jindal2019peregrine}, which is a hash value computed recursively over the DAG of operators in the compiled plan. The signature does not include job input parameters.
\end{enumerate}
We thus have \textit{job groups} and \textit{job instances} belonging to each group, corresponding to recurrences of the job. Job instances have the same key value within each job group.

\subsection{Potential Sources of Variation}
\label{subsec:sources-of-variation}

Within each job group, the run times of job instances can vary due to any of the following reasons.

\textbf{Intrinsic Characteristics}: The key used for grouping jobs includes information on their execution plan (e.g., type of operators, estimated cardinality, dependency between operators) while not including the job input parameters (e.g., parameters for filter predicates) or input data sets. Different instances can have different values for these parameters, data sets, and their sizes. This can lead to different run times within the group if the parameter changes are not accompanied by a change in the compiled plan. In our datasets, we have observed input data sizes vary by a factor of 50 within the same job group.

\begin{figure}
	\centering
		\includegraphics[width=\columnwidth]{img/tokenusage.pdf}
	\caption{Token usage for an example job during its run.
	}\label{fig:token}
\end{figure}
\textbf{Resource Allocation}: On \cosmos, the unit of resource allocation is a \textit{token}~\cite{power2021cosmos}, which is analogous to the notion of a container. The number of tokens guaranteed for a job can be specified by users at the time of job submission or it may be recommended by the system~\cite{autotoken}. To further improve the utilization of the existing infrastructure, unused resources are repurposed as pre-emptive opportunistic tokens~\cite{boutin2014apollo} that can be leveraged by any jobs freely. Though their availability is less predictive, which often results in longer or shorter run times. Figure~\ref{fig:token} shows the skyline of token usage for a \cosmos job that was allocated with 66 tokens; including opportunistic tokens it used up to 198 tokens in total throughout its processing time. 

The maximum number of tokens ultimately utilized by a job depends on how much parallelism it can exploit subject to the number of tokens allocated to it (guaranteed and opportunistic). In our datasets, we have observed maximum token counts vary by a factor of 10 within the same job group.

%To better manage the capacity of such enormous infrastructure, the concept of ``\textit{tokens}'' was introduced to control the amount of resources, measured by the number of containers, that can be allocated to a particular job~\cite{power2021cosmos}. 
%The allocated tokens can be specified by customers to limit the maximum number of resource that can be used simultaneously. 

While the number of tokens indicate the amount of resources used, there is also variation in the characteristics of allocated resources. Tokens map to computational resources on SKUs, and being established over the decade, the \cosmos cluster consists of 10--20 different SKUs\footnote{Stock Keeping Unit} with different processing speeds~\cite{zhu2021kea}. In our datasets, we have observed different job instances within the same job group run on 1 to 9 different SKU types.

%some of the newer generation of machines have faster processing speed~\cite{zhu2021kea} 

\begin{figure}
	\centering
	\centering
	\includegraphics[width=.6\columnwidth]{img/cpu.pdf}
	\caption{CPU utilization for different SKUs in one of the \cosmos clusters.
	}\label{fig:cpu}
\end{figure}
\textbf{Cluster Conditions}: Finally, cluster conditions can also lead to variations in run times. This includes both the availability of opportunistic tokens (discussed above) as well as load on the individual machines. Figure~\ref{fig:cpu} shows significant differences in the CPU utilizations of machines with different SKU types in one of the \cosmos clusters. For example, 
utilization for Gen6 varies from 2\% to 33\% with an average of 17\% whereas for Gen3.5 it varies from 10\% to 100\% with an average of 68\%.
Higher utilizations (loads) are likely to cause more contention for shared resources, and a larger range of loads may increase variation in run times.

\subsection{Datasets}

Since we want to develop insights into the various potential sources of variation as discussed above, we collected data along those dimensions from production workloads on our clusters. We extract information about intrinsic characteristics such as operator counts in the plan, input data sizes, and cardinalities, costs, etc. estimated by the SCOPE optimizer using the Peregrine framework~\cite{jindal2019peregrine}. We obtain token usage information from the job execution logs, and SKU and machine load information using the KEA framework~\cite{zhu2021kea}. Finally we join all this information together by matching on the job ID, machine name that execute each vertex and the corresponding job submission time.

\begin{table}[ht]
\centering
\caption{Datasets used for this study. \textit{Support} denotes the minimum number of job instances per group. We include groups after filtering for this criteria.}
\label{tab:datasets}
\resizebox{\columnwidth}{!}{\begin{tabular}{|c|c|c|c|c|}\hline
     \textbf{Dataset}&  \textbf{Interval}& \textbf{Job Groups}& \textbf{Job Instances}& \textbf{Support}\\\hline\hline
     \textbf{D1}& 6 months& 9.5K& 3.2M& 20\\\hline
     \textbf{D2}& 15 days& 11.9K& 737K& 3\\\hline
     \textbf{D3}& 5 days& 11.6K& 215K& 3\\\hline
\end{tabular}}
\end{table}
Table~\ref{tab:datasets} summarizes the datasets that we use for our study. The datasets consist of a subset of jobs run over the corresponding interval, and are included if the number of instances per group (support) exceeds a minimum theshold. We use dataset D1 to identify and group distributions of run times (see Section~\ref{sec:clustering} for details). We used dataset D2 to train a predictor for run time variation and dataset D3 to test the accuracy of the predictor (Section~\ref{sec:model}).

%In this analysis, we set-off to gather data at the job-template level, which indicates a series of recurrent jobs processing different input data sources. To evaluate the reasoning of the variances, we combine a multitude of data sources, including (1) a set of environmental variables (including the utilization of each computing machine) that reflects the system status of the execution environment, (2) job characteristics (such as information for the execution plan) to indentify the type of jobs can potentially have higher runtime variation, and (3) resource usage for a particular job as the input to the estimators to predict the coefficient of variance of the job runtime. 


\section{Characterizing Runtime Variation}
\label{sec:metrics}

We now discuss how we characterize and quantify run time variation for recurring jobs. This will form the basis for our prediction strategy that we dicuss in Section~\ref{sec:model}.

\subsection{Scalar Metrics}

As we discussed previously (Section~\ref{sec:intro}), a job's average run time does not give much insight into variations across repeated runs, or how long the next run of the job will take. Thus, it is not very useful for characterizing, predicting, or explaining the variations.

\begin{figure}
	\centering
		\subfloat[Historic Median vs Run Times]{\includegraphics[width=0.5\columnwidth]{img/median_compare_train_all.png}\label{fig:median-vs-runtime}}
		\subfloat[Historic COV vs COV]{\includegraphics[width=0.5\columnwidth]{img/cov2.png}\label{fig:cov-as-predictor}}
	\caption{Correlations between historic median run time and job run times, and historic COV and COV of all run times observations.}
	%{Job runtime/COV compared with historic median/COV.}
	\label{fig:medianbenchmark}
\end{figure}
Next, we investigate how well a job's median run time is correlated with run times over the different repetitions of the job. Figure~\ref{fig:median-vs-runtime} shows how the run times for individual repetitions of the job compared with its historic median using dataset D2. 
\yz{from Bob: I think you should point out that the stalagmite is offset from the diagonal by a fixed amount of time. This is a bigger relative delay for faster-running jobs, while for very long-running jobs this delay makes only a small difference in the total runtime (which is why a constant time delay looks curved in log space).}

We observe two distinct patterns in the figure---a set of points are clustered along the diagonal, indicating a good correlation of individual run times to the median, whereas another set of points are clustered separately in a pattern resembling a stalagmite\footnote{A stalagmite is a rocky formation that arises from the floor of a cave and may reach the ceiling~\cite{stalagmite}.}. The runs corresponding to the points in the stalagmite are much slower than the median run time and contribute to the (long) tail of the run time distributions. Such runs are rare (comprising less than 5\% of all runs), with the probability reducing with larger median values. But we have found it to be very difficult to predict upfront if the time for a new run will end up on the diagonal or on the stalagmite. The existence of these two patterns, as well as the difficulty of predicting to which pattern a new run will belong, even if the median run time is stable and known, makes the median a poor choice to use for predicting run times or for characterizing variations. A similar trend can be found for the average and $95^{th}$ percentile of historic runtime (see Figure~\ref{fig:avgbenchmark}).

\begin{figure}
	\centering
		\subfloat[Historic Average vs Runtimes]{\includegraphics[width=0.5\columnwidth]{img/avg_compare_train_all.png}\label{fig:avg-vs-runtime}}
		\subfloat[$95^{th}$ Percentile vs Runtimes]{\includegraphics[width=0.5\columnwidth]{img/p95_compare_train_all.png}\label{fig:95-vs-runtime}}
	\caption{Correlations between historic average/$95^{th}$ percentile and job runtimes using dataset D2.}
	%{Job runtime/COV compared with historic median/COV.}
	\label{fig:avgbenchmark}
\end{figure}

% \todo{can we discuss what happens with 95\% or some other quantile vs run time?}

Coefficient of Variation (COV) is another commonly-used metric that is used to characterize variation. It is defined as the ratio of standard deviation to the average, and is an unitless quantity. COV is straight-forward to compute and interpret. Prior work~\cite{schad:ec2-variance:vldb:2010} has used COV to characterize variation in job run times.
%
%Coefficient of Variation (COV), defined by the ratio of standard deviation to the average, is a commonly used metric to evaluate runtime variation. 
%
However, using COV also has several limitations as follows.
\begin{enumerate}[leftmargin=*]
    \item \textbf{Bias}: The run times of SCOPE jobs that we study range from seconds to days, with significant differences in the average values. This may cause COV to be biased and one could always observe very large COV for short-running jobs.
    \item \textbf{Instability}: The average run times can increase due to the existence of outliers (in such large distributed systems, some jobs inevitably run slow occasionally). Thus, COV can be unstable with addition of more jobs in the dataset. Unlike the average, COV does not converge with large sample size thus does not have a consistent estimator~\cite{fischer2011history}.
    \item \textbf{Coarse-grained}: COV does not capture many characteristics of a distribution, such as its shape (such as unimodal, bimodal, and the existence of outliers). Hence, it cannot readily explain variation in a fine-grained manner.
    % \item \textbf{Lack of convergence}: COV does not converge with sample size thus does not have a consistent estimator \yz{look this up}. So, in this case, it is less predictable and less stable.\todo{are (2) and (4) different, or can they be combined?}
\end{enumerate}

Figure~\ref{fig:cov-as-predictor} shows how well the COV computed from historic runs for each job instance compares with COV of times from all runs in D3. Similar to the discussion for medians above, we see multiple groups of points, with the same historic COV appearing for different COV values from new runs and it is difficult to predict for a new run to which group it will belong. Additionally, the COV metric suffers from the limitations mentioned above. 

Overall, we found that scalar metrics such as average, median, quantiles, and COV by themselves are not sufficient for understanding or predicting run time variations. 

%Several interesting findings: 

%i) a stalagmite can be observed from the left figure, indicating a group of job instances that are much slower than median runtime. By further examining those jobs, we found little evidence for their slow down reasons. Most of those jobs share no differences with other job instances that have the same job template. The occurrences are also rare (less than 5\% of job instances might encounter such slow down, and it is un-predictable). And for job templates with less occurrences, one might not observe such cases at all. Therefore, we turn to predict the existence of those job instances and their probability (see Section~\ref{sec:model}) as opposed to predicting the runtime of each job instances (or whether the job instance will be in such stalagmite).

%COV is much less predictable with historic data due to the reasons mentioned before. For customer jobs, it would be interesting to infer the probability of such slow downs with better predictors. Therefore, we change our focus on this paper to the distribution of the jobs and its detailed shapes.

\subsection{Distributions}
\label{sec:clustering}

We now turn to characterizing variations based on the detailed \textit{runtime distribution} for each recurrent job group. Although there is a large variety in the run times of SCOPE jobs, we found that many different jobs have similar shapes of their run time distribution curves. So, we first normalize the job run times, then compute their distributions, and finally group them based on similarity. This helps to generalize the analysis across similar distributions from different jobs and reduce the number of groupings to a small number that can be more easily understood and kept track of by the users.

%moreover, to better generalize the analysis across different jobs which might have significantly different ranges of job runtime (but might share similar variation/shape of distribution), we normalize the job runtime by:

We use the following two normalization strategies, corresponding to different usage scenarios, for the job run times.
\begin{enumerate}[leftmargin=*]
	\item \textbf{\rationorm}: we take the ratio of job run time to median run time. For this scenario, we are interested in understanding the similarity in variation in terms of percentage change in run times.
	\item \textbf{\deltanorm}: we take the difference of the two, i.e., job run time - median run time. For this scenario, we are interested in understanding the the similarity in variation in terms of absolute change (seconds) in run times.
\end{enumerate}  

%We believe that both the distributions of the normalized runtime by \rationorm and \deltanorm are important in different scenarios. The ratio indicates the percentage variation benchmarked to the median, while the \deltanorm reveals the absolute deviation in the unit of seconds/minutes. 


To better examine the ``typical'' distribution shape across jobs with different templates, we conduct a clustering analysis using 2021-June to 2021-Nov's data with 3.2M job instances and 9,532 job groups with $\geq 20$ occurrences in the whole period (see D1 in Table~\ref{tab:datasets}). For each job group, we derive its histogram for the distribution of normalized runtime and then use un-supervised machine learning algorithm for the clustering. 

Our principal design choices for the runtime distribution clustering method is as the following:
\begin{itemize}[leftmargin=*]
%	\item For the clustering analysis, we want to evaluate the distribution of runtime variances. In this case, we normalize the runtime by its median value in this distribution. There can be two possible way for this normalization: (1) divided by the median runtime to consider the ratio between the instance's runtime benchmarked to the median or (2) minus the median runtime to consdier the absolute deviation from the median time. Maybe we can use either one that has better predictability, i.e., if jobs runtime variation has more consistency measured in \% changes, we can use this as the prediction value and we can convert to the absolute runtime deviation. Similar for the inverse.
	\item \textbf{Bin size and Range}: For calculating the distribution of the normalized runtime, the design of the bin size and range is critical. The range should cover the majority of the values with relatively fine granularity (but not too small such that we will have a lot of fluctuation due to noises in the derived distribution). We also want to cover the outliers (points in the stalagmites, that is, tails of the distributions) such that we can predict their probability of existence. Since they are rare, we merge the outliers into one bin in this distribution (based on being $\leq$ or $\geq$ some threshold). For \deltanorm, we use [-900, 900] (where <2\% of jobs are more than 900s slower than median, and for \rationorm, we use [0, 10] (where <1.5\% of jobs are 10x slower than median. Jobs with >900s or 10x slower than median are defined as outliers. For the bins size, we evaluated 50, 100, 200 and 500 bins, and chose 200 bins that has relatively smooth PDF curves and a sufficient level of granularity.
\item \textbf{Clustering algorithm}: We evaluated several clustering algorithms. Hierarchy clustering using dendrogram~\cite{nielsen2016introduction} and Agglomerative clustering~\cite{rokach2005clustering} are both flexible and can use different distance metrics and linkage methods, and users can specify the number of clusters to be formed. However, they both result in imbalanced clusters (some with >90\% of the jobs groups in one cluster). K-means clustering~\cite{sculley2010web} results in balanced clusters and can also take number of clusters as input. Therefore, we use this K-means clustering for the following analysis. 
	\item \textbf{Number of Clusters}: We determined the the number of clusters based on: (i) numeric measurements---we examine the decrease of \textit{inertia}, defined by the sum of squared distances between each sample and its cluster centroid and pick an elbow point where adding more clusters does not decrease the inertia by a significant amount, and (ii) by visually examining the clustering results to check if the clusters are sufficiently different from each other and have unique characteristics. We picked 8 clusters for both \deltanorm and \rationorm for consistency.
	\item \textbf{Smoothing histograms}: While doing the above analysis, we faced a limitation in the standard clustering algorithms---they are based on using probability density function (PDF) values as input vectors without considering the correlation between each bin. In reality, we also want to consider if adjacent density values of bins (e.g., the probability of a run time being in the $4^{th}$ or the $5^{th}$ bin) are correlated with each other. However, with any distance measurement (such as dot product), similarity between adjacent bins are not considered.
% 	whereas it is easy to observe cases where for job A, its $4^{th}$ bin's value equals to that of the $5^{th}$ bin for job B due to random noises. 
	Therefore, we introduce a \textit{smoothing step} after deriving the PDFs to reduce the difference between any two adjacent bins such that the two smoothed vectors mentioned above will have higher similarity. A carefully chosen bin size (as discussed above) will also help in this situation to reduce the impact of noises. 
\end{itemize}



%\begin{figure}
%	\centering
%	\centering
%	\begin{minipage}[b]{\columnwidth}
%		\includegraphics[width=\textwidth]{img/hist_normed_kmeans_8_bins_merge_tail_ratio0210_min_3/cluster_all.pdf}
%	\end{minipage}%
%	
%	\begin{minipage}[b]{\columnwidth}
%		\includegraphics[width=\textwidth]{img/hist_normed_kmeans_8_bins_merge_tail_delta0210_min_3/cluster_all.pdf}
%	\end{minipage}%
%	% 	\vspace{-3mm}
%	\caption{8 typical distribution of normalized runtime.
%	}\label{fig:clustering}
%\end{figure} 

Figure~\ref{fig:clustering} shows the distribution for the 8 clusters using \rationorm and \deltanorm policies. We can see that some distributions have two modes (e.g., Cluster 0,2 and 4 using \rationorm) and with different variances. Table~\ref{tab:statscluster} summarizes important statistics for each cluster. For example, for Cluster 0 with \rationorm, it contains 36.5\% of the total job observations; its outlier probability is 1.63\% (defined by $\geq 10$x slower than median for \rationorm); the difference between 25 and $75^{th}$ percentile is 0.06; the $95^{th}$ percentile of this distribution is 1.41, and the standard deviation is 2.46. While for Cluster 7 with \rationorm, the outlier probability decreases to 0.06\%. Clusters are ranked according to the difference between 25 and $75^{th}$ percentile.
\begin{figure}
	\centering
	\centering
	\begin{minipage}[b]{\columnwidth}
		\includegraphics[width=\textwidth]{img/hist_normed_kmeans_8_bins_merge_tail_ratio0210_min_3/cluster_all_idx_cut.pdf}
	\end{minipage}%
	
	\begin{minipage}[b]{\columnwidth}
		\includegraphics[width=\textwidth]{img/hist_normed_kmeans_8_bins_merge_tail_delta0210_min_3/cluster_all_idx_cut.pdf}
	\end{minipage}%
	% 	\vspace{-3mm}
	\caption{8 typical distribution of normalized runtime.
	}\label{fig:clustering}
\end{figure} 


% \begin{table}[]
% 	\begin{tabular}{llllllll}
% 		\toprule
% 		\multicolumn{4}{c}{Ratio}              & \multicolumn{4}{c}{Delta}             \\ \midrule
% 		cid & outlier & 25-75th         & 95th  & cid & outlier & 25-75th      & 95th    \\ \midrule
% 		0   & 0.25\%  & 0.15            & 1.31 & 0   & 0.01\%  & $\leq$3      & 13.57  \\
% 		1   & 1.63\%  & $\leq$0.02      & 1.31 & 1   & 0.04\%  & 162.81       & 502.01 \\
% 		2   & 0.25\%  & 0.15            & 1.31 & 2   & 0.00\%  & 9.05         & 22.61  \\
% 		3   & 0.06\%  & \textbf{0.20}           & \textbf{1.66} & 3   & 0.01\%  & 18.09        & 40.70  \\
% 		4   & 0.42\%  & 0.05            & 1.16 & 4   & 0.03\%  & 72.36        & 185.43 \\
% 		5   & 0.26\%  & 0.15            & 1.36 & 5   & 0.00\%  & $\leq$3      & 4.52   \\
% 		6   & \textbf{1.66\%}  & 0.10            & 1.41 & 6   & \textbf{0.26\%}  & \textbf{1591.96}    & \textbf{890.95} \\
% 		7   & 1.46\%  & 0.10            & 1.26 & 7   & 0.00\%  & $\leq$3      & 4.52  \\\bottomrule
% 	\end{tabular}
% 	\caption{Other statistics for 8 clusters.
% }\label{tab:statscluster0}
% \end{table}

% \begin{table}[]
% 	\caption{Other statistics for 8 clusters.}\label{tab:statscluster}
% \begin{adjustbox}{max width=\columnwidth}
% \begin{tabular}{lllp{0.5cm}lllllp{0.5cm}ll}
% 		\toprule
% \multicolumn{5}{c}{Ratio}             & \multicolumn{5}{c}{Delta}             \\\midrule
% cid &\% jobs& outlier & $25-75^{th}$ & $95^{th}$ & std & cid &\% jobs & outlier & $25-75^{th}$ & $95^{th}$ & std \\\midrule
% 0   &10.0& 0.25\%  & 0.17    & 1.29 & 1.45          & 0 &\textbf{40.8}&  1.93\%  & 4       & 28   & 155  \\
% 1   & \textbf{36.5}& 1.63\%  & 0.06    & 1.41 & \textbf{2.46} & 1 &9.2  & 2.43\%  & 199     & 408  & 296  \\
% 2   & 7.9& 0.25\%  & 0.19    & 1.34 & 0.82          & 2 &8.3  & 0.55\%  & 16      & 33   & 140  \\
% 3   &6.3& 0.06\%  &\textbf{0.29}& \textbf{1.46} & 0.55 & 3 &14.6  & 0.98\%  & 31      & 63   & 153  \\
% 4   &13.7& 0.42\%  & 0.11    & 1.20 & 0.93              & 4 &12.2  & 0.73\%  & 69      & 128  & 179  \\
% 5   & 9.8& 0.26\%  & 0.20    & 1.37 & 0.97              & 5 &5.7  & 0.49\%  & 11      & 19   & 140  \\
% 6   & 10.2& \textbf{1.66\%}  & 0.16    & 1.37 & 2.18     & 6 &1.7  & \textbf{24.23\%} & \textbf{936}     & \textbf{1359} & \textbf{2548} \\
% 7   & 5.6& 1.46\%  & 0.17    & 1.35 & 1.94              & 7 &7.6  & 0.53\%  & 11      & 23   & 148 \\\bottomrule
% \end{tabular}
% \end{adjustbox}
% \end{table}
% \todo{sort clusters by some characteristic, e.g., 25-75th width, so that readers can have a mental model that puts clusters numbers on a spectrum for that characteristic. Explain the semantics. Explain the first and last row of the table. Also arrange above cluster plot accordingly.}

\begin{table}[]
	\caption{Other statistics for the clusters.}\label{tab:statscluster}
\begin{adjustbox}{max width=\columnwidth}
\begin{tabular}{lllp{0.5cm}lllllp{1.0cm}p{0.8cm}l}
		\toprule
\multicolumn{5}{c}{Ratio}             & \multicolumn{5}{c}{Delta}             \\\midrule
cid &\% jobs& outlier & $25-75^{th}$ & $95^{th}$ & std & cid &\% jobs & outlier & $25-75^{th}$ (s)& $95^{th}$ (s)& std (s)\\\midrule
0   & \textbf{36.5} & 1.63\%                           & 0.06 & 1.41                           & \textbf{2.46} & 0  & \textbf{40.8} & 1.93\%                            & 4   & 28                             & 155                            \\
1   & 13.7                           & 0.42\%                           & 0.11 & 1.2                            & 0.93                           & 1  & 5.7  & 0.49\%                            & 11  & 19                             & 140                            \\
2   & 10.2                           & \textbf{1.66\%} & 0.16 & 1.37                           & 2.18                           & 2  & 7.6  & 0.53\%                            & 11  & 23                             & 148                            \\
3   & 10.0                             & 0.25\%                           & 0.17 & 1.29                           & 1.45                           & 3  & 8.3  & 0.55\%                            & 16  & 33                             & 140                            \\
4   & 5.6                            & 1.46\%                           & 0.17 & 1.35                           & 1.94                           & 4  & 14.6 & 0.98\%                            & 31  & 63                             & 153                            \\
5   & 7.9                            & 0.25\%                           & 0.19 & 1.34                           & 0.82                           & 5  & 12.2 & 0.73\%                            & 69  & 128                            & 179                            \\
6   & 9.8                            & 0.26\%                           & 0.20  & 1.37                           & 0.97                           & 6  & 9.2  & 2.43\%                            & 199 & 408                            & 296                            \\
7   & 6.3                            & 0.06\%                           & \textbf{0.29} & \textbf{1.46} & 0.55                           & 7  & 1.7  & \textbf{24.23\%} & \textbf{936} & \textbf{1359} & \textbf{2548} \\\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}
% \todo{sort clusters by some characteristic, e.g., 25-75th width, so that readers can have a mental model that puts clusters numbers on a spectrum for that characteristic. Explain the semantics. Explain the first and last row of the table. Also arrange above cluster plot accordingly.}

%\todo{add characteristics of each cluster and analysis}
% \todo{give percentages of job groups in the clusters}




==> Runtime Variation in Distributed Systems (Short II) (2)/Bayesian.tex <==
\subsection{Bayesian Network}

\todo{explain methodology}

\todo{show an example net}

\todo{Discuss some conclusions and how they overcome limitations of the correlation-based approach}


==> Runtime Variation in Distributed Systems (Short II) (2)/Challenges.tex <==
\section{Goals, Challenges, and Approach}
\label{sec:challenges}

Reasoning about performance changes is often done manually by experienced engineers with strong assumptions that can potentially lead to biased results. More recently, the availability of massive telemetry data in the cloud, that includes both information about job characteristics as well as status of the physical clusters, and the advent of data analytic methods, raise expectations that this process can be improved with more systematic and rigorous approaches.

% --- Rewrite ---
% With the rise of cloud and big data systems, we have seen a shift in how system performance can be evaluated and monitored.
% Specifically, we observe that reasoning about performance changes traditionally was done by experienced engineers.
% They would examine different system indicators and make a decision based on certain domain or prior knowledge which can potentially lead to biased results.
% However, in a cloud environment massive telemetry data is collected on a daily basis.
% This includes both information about job characteristics as well as near-real-time status of the computing clusters.
% With the advent of advanced data analysis methodology, we can now leverage automated techniques to facilitate a better understanding of performance data.
% ---

Our goal is to evaluate and predict runtime variation 
%runtime aspect of the performance especially its variation 
at the \textit{individual} job level
% .
% ; 
% \jma{This is desired, but by using clusters it's not what we do. Perhaps the term ``cluster'' means something else here?} 
% While system-wide reliability measurements serve their purpose, we want to develop
with a customized and use-case specific measurement that is more insightful for customers for both monitoring and planning purposes. And this is a highly desired metric from the customer's point of view, as validated by several conversations with the program managers (PMs). 
%
We also want to provide rich information regarding variation, such as the probability that a job runtime may exceed an extreme value, or various quantitative properties of the runtime distributions, e.g., quantiles, outliers, to the user, which was difficult to capture using traditional ML methods. 


%\subsection{Challenges}
Moreover, performance modeling of computational jobs in distributed systems is difficult, especially when focusing on reliability, due to the following challenges.
% \begin{itemize}[leftmargin=*]
%     \item \textbf{Complex environmental factors (C1)}: Resource sharing in cloud computing platforms adds complexity to the modeling of the impact on the job runtime due to noisy neighbors and other environmental changing factors. It is untractable for manual approach to relay the dynamic condition of each computation node and unravel the potential issues that result in performance degradation.
%     \item \textbf{Existence of rare events (C2)}: For rare events (such as occasional service disruption) that result in outliers and longer tails of the runtime distributions, it is difficult to collect observations of outliers for a recurrent job in order to accurately estimate their distributions. It is therefore crucial to be able to leverage job instances in other job groups that have sufficient observation samples and learn from their distributions. 
%     \item \textbf{Lack of proper metrics (C3)}: How to measure variation remains a challenge in the case of the characteristic long-tailed distributions of runtime, for which conventional variance-based measures do not capture the extreme values of interest, and may not converge even with large number of observations~\cite{fischer2011history}. Metrics such as COV are commonly used to evaluate the runtime variation, however, they are not sufficient to capture detailed characteristics of various runtime distributions.
%     % \item \textbf{C3}: While cluster-wide reliability measurement serves their purpose, with significant heterogeneity among customer jobs, we lack a customized and use-case specific measurement which is more insightful for customers for both monitoring and planning purposes. \todo{this point is not clear. rephrase. if this is a goal, rather than a challenge we can remove it from here and merge in the paragraph below.} 
%     \item \textbf{Lack of labeled data (C4)}: From the customer's point of view, to evaluate the runtime reliability and determine the right label of distribution it would have, a large number of job runs are required, which is time-consuming and oftentimes infeasible for a new job. However, for the majority of machine learning models for predictive analysis, labeled data is required.
%     % \yz{maybe mention lack of a clear definition for variation and the shapes of distribution renders most of the singular scaler evaluation invalid?}
%     % \item \textbf{C5}: While the cluster environment has significant impact on the job performance, the scheduling/existence of this job will also change the resource utilization of the machine, which in turn will modify the state of the system. This complex dependency between variables renders a number of predictors invalid due to multicollinearity~\cite{myers1990classical}. 
%     % \item \textbf{C5}: There is a large number of potential factors that impact the job performance. One needs to select carefully the model approach to consider the complex correlation between the different factors. 
% \end{itemize}
\begin{itemize}[leftmargin=*]
    \item \textbf{Complex environmental factors (C1)}: Resource sharing in cloud computing platforms adds complexity to the modeling of the job runtime due to noisy neighbors and other environmental changing factors. It is untractable for manual approaches to relay the dynamic condition of each computation node and unravel the potential issues that result in performance degradation.
    
    % To illustrate the challenges, we show in Figure~\ref{fig:corr}, the correlation plot for a subset of job features (details in Section~\ref{sec:input}) using Pearson correlation~\cite{benesty2009pearson}. 
    % %Details on each feature can be seen in Section~\ref{sec:input}. 
    % The color of the shaded circles indicates the sign/direction of correlation (blue: positive, red: negative), while their size and color intensity indicate the magnitude of the correlation.
    % For example, we see that CPU variation is positively correlated to COV, and there is a group of features (including VertexCounts and DataRead) that are also positively correlated. 
    % But, selecting the right subset of important features from a large set of features is not easy. It is also difficult to capture the complex correlation between the different factors.
    % Moreover, the figure does not reveal non-linear correlation in this plot. For example, as we show later (Section~\ref{sec:model}), AvgRowLength and TotalDataRead both affect the runtime distribution and its variance, but that is not apparent from this plot. 
    % In general, for developing a machine learning model, one should avoid the existence of correlated features as much as possible. We can use the correlation plot as the first examination of the features and validate the data quality. 
    % Even for a subset of the features, the complex correlation is difficult to capture.
    % \begin{figure}[h]
    % 	\centering
    % 	%\vspace{-3ex}
    % 	    \vspace{-8pt}
    % 		\includegraphics[width=0.9\columnwidth]{img/rplot0224.PNG}
    % % 	\includegraphics[width=1\columnwidth]{img/Rplot.pdf}
    % 	% 	\vspace{-0.8cm}
    % 		\vspace{-0.2cm}
    % 	\caption{Correlation plot between a subset of job features. The first column shows their correlation with runtime COV.}\label{fig:corr}
    % 	\vspace{-8pt}
    % 	% 	\vspace{-0.6cm}
    % \end{figure}

    \item \textbf{Existence of rare events (C2)}: For rare events (such as occasional service disruption) that result in outliers and longer tails of the runtime distributions, it is difficult to collect sufficient observations of outliers for a recurring job in order to accurately estimate their distributions. It is therefore crucial to be able to leverage the learning from job instances in other job groups that have sufficient observation samples. 
    \item \textbf{Lack of proper metrics (C3)}: How to measure variation remains a challenge in the case of the characteristic long-tailed distributions of runtime, for which conventional variance-based measures do not capture the extreme values of interest.
    % , and may not converge with increasing sample sizes~\cite{fischer2011history}. 
    Metrics such as COV that are commonly used to evaluate the runtime variation are not sufficient to capture detailed characteristics of various runtime distributions.
    % \item \textbf{C3}: While cluster-wide reliability measurement serves their purpose, with significant heterogeneity among customer jobs, we lack a customized and use-case specific measurement which is more insightful for customers for both monitoring and planning purposes. \todo{this point is not clear. rephrase. if this is a goal, rather than a challenge we can remove it from here and merge in the paragraph below.} 
    \item \textbf{Lack of labeled data (C4)}: \edit{While the majority of machine learning approaches for predictive analysis require labeled data, there is no label recorded for the causes of runtime distributions or job slowdowns. Manually evaluating runtime reliability to determine the distribution \textit{category} each job belongs to is also infeasible for new jobs with a small number of occurrences. 
    % Moreover, there is not records recorded to infer the root-cause of large runtime variability.
    }
    % \yz{maybe mention lack of a clear definition for variation and the shapes of distribution renders most of the singular scaler evaluation invalid?}
    % \item \textbf{C5}: While the cluster environment has significant impact on the job performance, the scheduling/existence of this job will also change the resource utilization of the machine, which in turn will modify the state of the system. This complex dependency between variables renders a number of predictors invalid due to multicollinearity~\cite{myers1990classical}. 
    % \item \textbf{C5}: There is a large number of potential factors that impact the job performance. One needs to select carefully the model approach to consider the complex correlation between the different factors. 
\end{itemize}

% \subsection{Correlation-based Approach}
% \yz{move to challenges, difficult to select features, which is large, second, missing features}
% A simple approach to start with is to examine the correlation between the different job characteristics.
% Figure~\ref{fig:corr} shows the correlation plot for every pair of features using Pearson correlation~\cite{benesty2009pearson}. The color of the shaded circles indicates the sign/direction of correlation (blue: positive, red: negative), and their diameter and color intensity is proportional to the magnitude of the correlation.
% We can see that the CPU variation is positively correlated to the COV, and there is a cluster of features (including VertexCounts and DataRead) that are also positively correlated. However, it is difficult to reveal non-linear correlation in this plot. For example, as we showed earlier (Section~\ref{sec:model}), AvgRowLength and TotalDataRead both affect the runtime distribution and its variance, but that is not apparent from this plot.

% \begin{figure}[t]
% 	\centering
% 	%\vspace{-3ex}
% 		\includegraphics[width=1\columnwidth]{img/rplot0224.PNG}
% % 	\includegraphics[width=1\columnwidth]{img/Rplot.pdf}
% 	% 	\vspace{-0.8cm}
% 	\caption{Correlation plot.}\label{fig:corr}
% 	% 	\vspace{-0.6cm}
% \end{figure}

%\subsection{Goals}
%\yz{do we need this section, or maybe we can shorten the description in section 1 in the (1), (2), (3)?}
%Our first goal is to evaluate and predict runtime variation 
%runtime aspect of the performance especially its variation 
%at the \textit{individual} job level.
% ; 
% \jma{This is desired, but by using clusters it's not what we do. Perhaps the term ``cluster'' means something else here?} 
%While system-wide reliability measurements serve their purpose, we want to develop a customized and use-case specific measurement that is more insightful for customers for both monitoring and planning purposes. And this is a highly desired metric from the customer's point of view, as validated by several conversations with the program managers (PMs). 

%Our second goal is to provide rich information regarding variation, such as the probability that a job runtime may exceed an extreme value, or various quantitative properties of the runtime distributions, e.g., quantiles, to the user. 


%or even gives information of the full distribution if treated the job runtime as a random variable. 
%While point prediction for the job runtime is an important and challenging problem on its own~\cite{phoebe,pietri2014performance, tasq-arxiv, tasq-edbt, hu:reloca:infocom:2020, autodop, starfish:analytics-cluster-sizing:socc:2011, starfish:analytics-cluster-sizing:socc:2011, rajan2016perforator}, we want to predict the potential variation in runtimes for recurring jobs, rather than the absolute runtimes. Thus, direct prediction of job runtimes is a \textit{non-goal} for this work. %leveraging existing observations of runtimes 
%through better characterization of the
%and taking into account job properties, resource allocation, and environmental conditions such as system load [challenge \textbf{C1}].
%Previous analysis of \cosmos jobs shows a large portion of recurrent jobs~\cite{wing2020osdi}, however, for the measurement of runtime variation, a large number of observations are required, which is impossible for a majority of jobs executed at a lower frequency. Moreover, for rare events (such as occasional service disruption) that results in outlier and longer tails of the runtime distribution, we have to be ``lucky'' to have such observations for a recurrent job in order to predict its performance. In this paper, as opposed to focus on point prediction for the job runtime (which is also important as its own, and very challenging~\cite{phoebe}), we want to predict the extent of potential variation for recurrent jobs, leveraging existing observations of runtimes (if any) through better characterization of the job properties.

%\subsection{Approach}

\begin{figure}[h]
	\centering
	\vspace{-0.2cm}
			\includegraphics[width=0.7\columnwidth]{img/architecture.pdf}\vspace{-5pt}
\caption{\edit{Framework.}}
\label{fig:architecture}
\vspace{-8pt}
\end{figure}

%On the journey toward better understanding runtime variation, we address a few key steps 
%as stated in Figure~\ref{fig:architecture}, 
%leveraging information both at the job level and the machine level:

Our 2-step approach in this work is to characterize and then predict variation based on the distribution of normalized runtimes of recurring jobs (see Figure~\ref{fig:architecture}). 
% Figure~\ref{fig:architecture} shows the main components of our framework. 
% Following are the key steps that we complete for implementing it.
Leveraging information both at the job level and the machine level, we:
%\begin{itemize}[leftmargin=*]
%	\item Define Metrics: We examine typical distributions of runtimes for various jobs in historic data using \textit{Clustering Analysis}~\cite{bishop2006pattern}. For each type (single-mode, multi-mode) of distribution, we define key metrics to depict the distribution, and quantify the variation in numeric terms that can be easily understood by users [challenge \textbf{C3}, Section~\ref{sec:bg}].
	%to represent easy understandable metrics for customers.
%	\item Develop predictors: We leverage \textit{Machine Learning (ML) classification} techniques to predict which distribution of runtimes the job most likely belongs to. To overcome the challenges [\textbf{C2, C4}] of infrequent jobs and rare events while characterizing and grouping distributions, we develop the model using the observations of distributions over a long time interval and for jobs with more recurrences (Dataset D1, Table~\ref{tab:datasets}), while the model can be applied to any new jobs. [Section~\ref{sec:bg}]
	%to predict the variation, this is a typical ML task. But the challenge is how we can generate labels to learn (i.e., which is the distribution type, and the metrics, which is not available unless we have a large number of observations for a job). To achieve this, we...
%	\item Explain predictions: We use \textit{model explainer} based on feature contribution algorithms to better understand the various factors associated with runtime variation [challenge \textbf{C1}, Section~\ref{sec:explain}]. 
%	\item Analyze \textit{what-if scenarios}: based on the prediction model, we propose hypothetical scenarios and evaluate the potential improvement of runtime performance [Section~\ref{sec:prescriptive}].  
% 	\yz{another bullet point for optimization using what-if prediction?}
	%\todo{complete...?}
	%according to the prediction algorithm. 
%\end{itemize}

\begin{itemize}[leftmargin=*]
	\item \textbf{Characterize runtime distributions}: \edit{Our \textit{Clustering Analysis} uses a novel scheme of featurization to cluster~\cite{bishop2006pattern} historic jobs with distinctively-diverse runtime distributions. }
% 	This enables us to estimate the probabilities of outliers without needing to predict individual job runtimes directly. 
	We associate the job with one distribution it belongs to using an innovative and adaptive \textit{posterior likelihood} method. For each type (single-mode, multi-mode) of distribution, we define key metrics to depict the distribution, and quantify the variation in numeric terms that can be easily understood by users [challenge \textbf{C3}, Section~\ref{sec:metrics}].
	%to represent easy understandable metrics for customers.
	\item \textbf{Develop \textit{ML predictor}}: We leverage Machine Learning (ML) classification techniques to predict which distribution of runtimes the job most likely belongs to, taking into account job properties, resource allocation, and environmental conditions such as system load \edit{that potentially leads to noisy neighbors} [\textbf{C1}]. To overcome the challenges \textbf{C2} and \textbf{C4}, %of infrequent jobs and rare events while characterizing and grouping distributions, 
	we develop the model using the observations of distributions over a long time interval and for jobs with more recurrences (Dataset D1, Table~\ref{tab:datasets}), while the model can be applied to any new jobs. [Section~\ref{sec:model}]
	%to predict the variation, this is a typical ML task. But the challenge is how we can generate labels to learn (i.e., which is the distribution type, and the metrics, which is not available unless we have a large number of observations for a job). To achieve this, we...
	\item \textbf{Explain predictions}: We use \textit{Model Explainer} based on feature contribution algorithms to better understand the various factors associated with runtime variation [challenge \textbf{C1}, Section~\ref{sec:explain}]. 
	\item \textbf{Analyze \textit{what-if scenarios}}: Based on the prediction model, we propose hypothetical scenarios and evaluate the potential improvement of runtime performance quantitatively [Section~\ref{sec:prescriptive}].  
% 	\yz{another bullet point for optimization using what-if prediction?}
	%\todo{complete...?}
	%according to the prediction algorithm. 
\end{itemize}

While point prediction for the job runtime is an important and challenging problem on its own\edit{~\cite{phoebe,pietri2014performance, tasq-arxiv, tasq-edbt, hu:reloca:infocom:2020, autodop,  starfish:analytics-cluster-sizing:socc:2011, rajan2016perforator}}, we want to predict the potential variation in runtimes for recurring jobs, rather than the absolute runtimes. Thus, direct prediction of job runtimes is a \textit{non-goal} for this work. 

% \todo{how are we addressing C5?}

%In sum, ...  

==> Runtime Variation in Distributed Systems (Short II) (2)/Challenges_Anja.tex <==
\section{Challenges and Approach}
\label{sec:challenges}
With the rise of cloud and big data systems, we have seen a shift in how system performance can be evaluated and monitored.
Specifically, we observe that reasoning about performance changes traditionally was done by experienced engineers.
They would examine different system indicators and make a decision based on certain domain or prior knowledge which can potentially lead to biased results.
However, in a cloud environment massive telemetry data is collected on a daily basis.
This includes both information about job characteristics as well as near-real-time status of the computing clusters.
With the advent of advanced data analysis methodology, we can now leverage automated techniques to facilitate a better understanding of performance data.

However, even with advanced machine learning (ML) technology at our fingertips, performance modeling in distributed systems remains a challenge, especially if we focus on a system's reliability. We observe the following challenges for runtime modeling:
\begin{description}
\item[\bf Measuring runtime (C1).] Traditional variance-based measures are unable to capture the characteristic long-tailed distributions that we observe when measuring runtime.
\item[\bf Capturing outliers (C2).] A significant portion of the runtime outliers for a reccurrent job are due to rare events such as the occasional service disruption. Historic data needs to contain such outliers to take them into consideration for ML-based modeling.
\item[\bf Resource sharing (C3).] Big Data as well as cloud systems have shared architectures, allowing multiple users to access and interact with the system simultaneously. This results in noise and other environmentally changing factors influencing runtime measurements.
\item[\bf Repeated job execution (C4).] In order to create a useful ML-model based on prior execution statistics, we need to observe the execution of the same job multiple times. Running a job just for the purpose of modeling its runtime is infeasible for many customers.
\end{description}

\smallsection{Solution Overview}
In our work, we focus on the explanation, mitigation and prediction of runtime variation on the \textit{individual} job level instead of the full-system level.
We observe that per-job runtime estimates are highly desirable from the customer's point of view to understand and monitor the execution of their pipelines.
Estimating the variation of the runtime for a particular job is different than executing a point estimate:
It requires us to determine the distribution of observed runtimes over multiple runs of the same job.
To facilitate accurate predictions, we consider a job's properties, resource allocation, and environmental setting.

Our framework takes as input...

Our framework is built to better understand the variation of a job's runtime. We use these building blocks to achieve that:
\begin{description}
\item[\bf We define metrics.] Using historic data, we examine the typical runtime distributions of various jobs. For each type of distribution, we define key metrics to depict the distribution, and quantify the variation in numeric terms that can be easily understood by users. This addresses challenge C1.
\item[\bf We develop predictors.] Using ML classification techniques, we determine which runtime profile most likely fits a given job. To overcome challenges C2 and C3, i.e.,~outliers and resource contention, we focus on frequently recurring jobs in our analysis.
\item[\bf We explain predictions.] To better understand the various influences on runtime variation, we leverage feature contribution algorithms. Furthermore, these techniques allow us to propose job improvements based on the observed characteristics.
\end{description}

==> Runtime Variation in Distributed Systems (Short II) (2)/Characterizing_runtimes.tex <==
\section{Characterizing Runtime Variation}
\label{sec:metrics}

We now discuss how we characterize and quantify runtime variation for recurring jobs. This will form the basis for our prediction strategy that we discuss in Section~\ref{sec:model}.

\subsection{Scalar Metrics}

As outlined previously (Section~\ref{sec:intro}), a job's average runtime does not give much insight into variations across repeated runs, or how long the next run of the job will take. Thus, it is not very useful for characterizing, predicting, or explaining the variations.

\begin{figure}
	\centering
		\subfloat[\edit{Median vs instance runtimes}]{\includegraphics[width=0.30\columnwidth]{img/median.pdf}\label{fig:median-vs-runtime}\vspace{-0.1cm}}\quad\quad\quad
% 		\subfloat[Median vs Runtimes]{\includegraphics[width=0.45\columnwidth]{img/median_compare_train_all.png}\label{fig:median-vs-runtime}\vspace{-0.2cm}}\hfill
		\subfloat[\edit{Historic COV vs COV}]{\includegraphics[width=0.30\columnwidth]{img/cov.pdf}\label{fig:cov-as-predictor}\vspace{-0.1cm}}
% 		\subfloat[Historic COV vs COV]{\includegraphics[width=0.45\columnwidth]{img/cov2.png}\label{fig:cov-as-predictor}\vspace{-0.2cm}}
		\vspace{-0.1cm}
	\caption{\edit{Correlations between historic median and job runtimes (a), and historic COV and COV of all observations (b).}}
	%{Job runtime/COV compared with historic median/COV.}
	\label{fig:medianbenchmark}
			\vspace{-0.3cm}
\end{figure}
Next, we investigate how well a job's median runtime correlates with runtimes over the different repetitions of the job. Figure~\ref{fig:median-vs-runtime} shows how runtimes for individual repetitions of the job compare with its historic median using dataset D2 in log-scale. 

We observe two distinct patterns in Figure~\ref{fig:median-vs-runtime}---a set of points are clustered along the diagonal, indicating a good correlation of \edit{individual job instances' runtimes} to the median, and another set of points are clustered separately in a pattern resembling a stalagmite\footnote{A stalagmite is a rocky formation that arises from the floor of a cave and may reach the ceiling~\cite{stalagmite}.}. The runs corresponding to the points in the stalagmite are much slower than the median runtime and contribute to the (long) tail of the runtime distributions. 
% We observe that the stalagmite is offset from the diagonal by a fixed amount of time. This is a bigger relative delay for faster-running jobs, while for very long-running jobs this delay makes only a small difference in the total runtime (which is why a constant time delay looks curved in log space). 
Such runs are rare (comprising less than 5\% of all runs), with the probability reducing with larger median values. But we have found it to be very difficult to predict upfront if the time for a new run will end up on the diagonal or on the stalagmite. The existence of these two patterns, as well as the difficulty of predicting to which pattern a new run will belong, even if the median runtime is stable and known, makes the median a poor choice to use for predicting runtimes or for characterizing variations. A similar trend can be found for the average and $95^{\text{th}}$ percentile of historic runtime. 

% \begin{figure}
% 	\centering
% 		\subfloat[Average vs Runtimes]{\includegraphics[width=0.45\columnwidth]{img/avg_compare_train_all.png}\label{fig:avg-vs-runtime}\vspace{-0.2cm}}\hfill
% 		\subfloat[$95^{\text{th}}$ Percentile vs Runtimes]{\includegraphics[width=0.45\columnwidth]{img/p95_compare_train_all.png}\label{fig:95-vs-runtime}\vspace{-0.2cm}}		\vspace{-0.3cm}
% 	\caption{Correlations between historic average/$95^{\text{th}}$ percentile and job runtimes.}
% 	%{Job runtime/COV compared with historic median/COV, DatasetD2
% 	\label{fig:avgbenchmark}
% 	\vspace{-10pt}
% \end{figure}

% \todo{can we discuss what happens with 95\% or some other quantile vs runtime?}

The Coefficient of Variation (COV) is another commonly-used metric to characterize variation. It is defined as the (unitless) ratio of standard deviation to the average. COV is straightforward to compute and interpret, and prior work~\cite{schad:ec2-variance:vldb:2010} has used COV to characterize variation in job runtimes.
%
%Coefficient of Variation (COV), defined by the ratio of standard deviation to the average, is a commonly used metric to evaluate runtime variation. 
%
But COV has several limitations:
\begin{itemize}[leftmargin=*]
    \item \textbf{Bias}: The runtimes of SCOPE jobs that we study range from seconds to days, with significant differences in the average values. This may cause COV to be biased and one could always observe very large COV for short-running jobs.
    \item \textbf{Instability}: The average runtime can increase due to the existence of outliers (in such large distributed systems, some jobs inevitably run slow occasionally). Thus, COV can be unstable with addition of more jobs in the dataset. Unlike the average, COV does not converge with a large sample size thus does not have a consistent estimator~\cite{fischer2011history}.
    \item \textbf{Coarse-grained}: COV does not capture many characteristics of a distribution, such as its shape (such as unimodal, bimodal, and the existence of outliers). Hence it cannot readily explain variation in a fine-grained manner.
    % \item \textbf{Lack of convergence}: COV does not converge with sample size thus does not have a consistent estimator \yz{look this up}. So, in this case, it is less predictable and less stable.\todo{are (2) and (4) different, or can they be combined?}
\end{itemize}

\edit{Figure~\ref{fig:cov-as-predictor} shows how well the COV computed from historic runs (y-axis) for each job instance based on dataset D2 compares with the COV of times from all runs (x-axis) based on the observation in D3.} Similar to the discussion for medians above, we see multiple groups of points, with the same historic COV appearing for different COV values from new runs and it is difficult to predict for a new run to which group it will belong. Additionally, the COV metric suffers from the limitations mentioned above. 

Overall, we found that scalar metrics such as average, median, quantiles, and COV by themselves are not sufficient for understanding or predicting runtime variation. 

%Several interesting findings: 

%i) a stalagmite can be observed from the left figure, indicating a group of job instances that are much slower than median runtime. By further examining those jobs, we found little evidence for their slow down reasons. Most of those jobs share no differences with other job instances that have the same job template. The occurrences are also rare (less than 5\% of job instances might encounter such slow down, and it is un-predictable). And for job templates with less occurrences, one might not observe such cases at all. Therefore, we turn to predict the existence of those job instances and their probability (see Section~\ref{sec:model}) as opposed to predicting the runtime of each job instances (or whether the job instance will be in such stalagmite).

%COV is much less predictable with historic data due to the reasons mentioned before. For customer jobs, it would be interesting to infer the probability of such slow downs with better predictors. Therefore, we change our focus on this paper to the distribution of the jobs and its detailed shapes.

% \subsection{Distributions}
% \label{sec:clustering}

% We now turn to characterizing variations based on the detailed \textit{runtime distribution} for each recurrent job group. Although there is a large variety in the runtimes of SCOPE jobs, we found that many different jobs have similar shapes of their runtime distribution curves. So, we first normalize the job runtimes, then compute their distributions, and finally group them based on similarity. This helps to generalize the analysis across similar distributions from different jobs and reduce the number of groupings to a small number that can be more easily understood and kept track of by the users.

% %moreover, to better generalize the analysis across different jobs which might have significantly different ranges of job runtime (but might share similar variation/shape of distribution), we normalize the job runtime by:

% We use the following two normalization strategies, corresponding to different usage scenarios, for the job runtimes.
% \begin{enumerate}[leftmargin=*]
% 	\item \textbf{\rationorm}: we take the ratio of job runtime to median runtime. For this scenario, we are interested in understanding the similarity in variation in terms of percentage change in runtimes.
% 	\item \textbf{\deltanorm}: we take the difference of the two, i.e., job runtime - median runtime. For this scenario, we are interested in understanding the the similarity in variation in terms of absolute change (seconds) in runtimes.
% \end{enumerate}  

% %We believe that both the distributions of the normalized runtime by \rationorm and \deltanorm are important in different scenarios. The ratio indicates the percentage variation benchmarked to the median, while the \deltanorm reveals the absolute deviation in the unit of seconds/minutes. 


% To better examine the ``typical'' distribution shape across jobs with different templates, we conduct a clustering analysis using 2021-June to 2021-Nov's data with 3.2M job instances and 9,532 job groups with $\geq 20$ occurrences in the whole period (see D1 in Table~\ref{tab:datasets}). For each job group, we derive its histogram for the distribution of normalized runtime and then use un-supervised machine learning algorithm for the clustering. 

% Our principal design choices for the runtime distribution clustering method is as the following:
% \begin{itemize}[leftmargin=*]
% %	\item For the clustering analysis, we want to evaluate the distribution of runtime variances. In this case, we normalize the runtime by its median value in this distribution. There can be two possible way for this normalization: (1) divided by the median runtime to consider the ratio between the instance's runtime benchmarked to the median or (2) minus the median runtime to consdier the absolute deviation from the median time. Maybe we can use either one that has better predictability, i.e., if jobs runtime variation has more consistency measured in \% changes, we can use this as the prediction value and we can convert to the absolute runtime deviation. Similar for the inverse.
% 	\item \textbf{Bin size and Range}: For calculating the distribution of the normalized runtime, the design of the bin size and range is critical. The range should cover the majority of the values with relatively fine granularity (but not too small such that we will have a lot of fluctuation due to noises in the derived distribution). We also want to cover the outliers (points in the stalagmites, that is, tails of the distributions) such that we can predict their probability of existence. Since they are rare, we merge the outliers into one bin in this distribution (based on being $\leq$ or $\geq$ some threshold). For \deltanorm, we use [-900, 900] (where <2\% of jobs are more than 900s slower than median, and for \rationorm, we use [0, 10] (where <1.5\% of jobs are 10x slower than median. Jobs with >900s or 10x slower than median are defined as outliers. For the bins size, we evaluated 50, 100, 200 and 500 bins, and chose 200 bins that has relatively smooth PDF curves and a sufficient level of granularity.
% \item \textbf{Clustering algorithm}: We evaluated several clustering algorithms. Hierarchy clustering using dendrogram~\cite{nielsen2016introduction} and Agglomerative clustering~\cite{rokach2005clustering} are both flexible and can use different distance metrics and linkage methods, and users can specify the number of clusters to be formed. However, they both result in imbalanced clusters (some with >90\% of the jobs groups in one cluster). K-means clustering~\cite{sculley2010web} results in balanced clusters and can also take number of clusters as input. Therefore, we use this K-means clustering for the following analysis. 
% 	\item \textbf{Number of Clusters}: We determined the the number of clusters based on: (i) numeric measurements---we examine the decrease of \textit{inertia}, defined by the sum of squared distances between each sample and its cluster centroid and pick an elbow point where adding more clusters does not decrease the inertia by a significant amount, and (ii) by visually examining the clustering results to check if the clusters are sufficiently different from each other and have unique characteristics. We picked 8 clusters for both \deltanorm and \rationorm for consistency.
% 	\item \textbf{Smoothing histograms}: While doing the above analysis, we faced a limitation in the standard clustering algorithms---they are based on using probability density function (PDF) values as input vectors without considering the correlation between each bin. In reality, we also want to consider if adjacent density values of bins (e.g., the probability of a runtime being in the $4^{th}$ or the $5^{th}$ bin) are correlated with each other. However, with any distance measurement (such as dot product), similarity between adjacent bins are not considered.
% % 	whereas it is easy to observe cases where for job A, its $4^{th}$ bin's value equals to that of the $5^{th}$ bin for job B due to random noises. 
% 	Therefore, we introduce a \textit{smoothing step} after deriving the PDFs to reduce the difference between any two adjacent bins such that the two smoothed vectors mentioned above will have higher similarity. A carefully chosen bin size (as discussed above) will also help in this situation to reduce the impact of noises. 
% \end{itemize}



% %\begin{figure}
% %	\centering
% %	\centering
% %	\begin{minipage}[b]{\columnwidth}
% %		\includegraphics[width=\textwidth]{img/hist_normed_kmeans_8_bins_merge_tail_ratio0210_min_3/cluster_all.pdf}
% %	\end{minipage}%
% %	
% %	\begin{minipage}[b]{\columnwidth}
% %		\includegraphics[width=\textwidth]{img/hist_normed_kmeans_8_bins_merge_tail_delta0210_min_3/cluster_all.pdf}
% %	\end{minipage}%
% %	% 	\vspace{-3mm}
% %	\caption{8 typical distribution of normalized runtime.
% %	}\label{fig:clustering}
% %\end{figure} 

% Figure~\ref{fig:clustering} shows the distribution for the 8 clusters using \rationorm and \deltanorm policies. We can see that some distributions have two modes (e.g., Cluster 0,2 and 4 using \rationorm) and with different variances. Table~\ref{tab:statscluster} summarizes important statistics for each cluster. For example, for Cluster 0 with \rationorm, it contains 36.5\% of the total job observations; its outlier probability is 1.63\% (defined by $\geq 10$x slower than median for \rationorm); the difference between 25 and $75^{th}$ percentile is 0.06; the $95^{\text{th}}$ percentile of this distribution is 1.41, and the standard deviation is 2.46. While for Cluster 7 with \rationorm, the outlier probability decreases to 0.06\%. Clusters are ranked according to the difference between 25 and $75^{th}$ percentile.
% \begin{figure}
% 	\centering
% 	\centering
% 	\begin{minipage}[b]{\columnwidth}
% 		\includegraphics[width=\textwidth]{img/hist_normed_kmeans_8_bins_merge_tail_ratio0210_min_3/cluster_all_idx_cut.pdf}
% 	\end{minipage}%
	
% 	\begin{minipage}[b]{\columnwidth}
% 		\includegraphics[width=\textwidth]{img/hist_normed_kmeans_8_bins_merge_tail_delta0210_min_3/cluster_all_idx_cut.pdf}
% 	\end{minipage}%
% 	% 	\vspace{-3mm}
% 	\caption{8 typical distribution of normalized runtime.
% 	}\label{fig:clustering}
% \end{figure} 


% % \begin{table}[]
% % 	\begin{tabular}{llllllll}
% % 		\toprule
% % 		\multicolumn{4}{c}{Ratio}              & \multicolumn{4}{c}{Delta}             \\ \midrule
% % 		cid & outlier & 25-75th         & 95th  & cid & outlier & 25-75th      & 95th    \\ \midrule
% % 		0   & 0.25\%  & 0.15            & 1.31 & 0   & 0.01\%  & $\leq$3      & 13.57  \\
% % 		1   & 1.63\%  & $\leq$0.02      & 1.31 & 1   & 0.04\%  & 162.81       & 502.01 \\
% % 		2   & 0.25\%  & 0.15            & 1.31 & 2   & 0.00\%  & 9.05         & 22.61  \\
% % 		3   & 0.06\%  & \textbf{0.20}           & \textbf{1.66} & 3   & 0.01\%  & 18.09        & 40.70  \\
% % 		4   & 0.42\%  & 0.05            & 1.16 & 4   & 0.03\%  & 72.36        & 185.43 \\
% % 		5   & 0.26\%  & 0.15            & 1.36 & 5   & 0.00\%  & $\leq$3      & 4.52   \\
% % 		6   & \textbf{1.66\%}  & 0.10            & 1.41 & 6   & \textbf{0.26\%}  & \textbf{1591.96}    & \textbf{890.95} \\
% % 		7   & 1.46\%  & 0.10            & 1.26 & 7   & 0.00\%  & $\leq$3      & 4.52  \\\bottomrule
% % 	\end{tabular}
% % 	\caption{Other statistics for 8 clusters.
% % }\label{tab:statscluster0}
% % \end{table}

% % \begin{table}[]
% % 	\caption{Other statistics for 8 clusters.}\label{tab:statscluster}
% % \begin{adjustbox}{max width=\columnwidth}
% % \begin{tabular}{lllp{0.5cm}lllllp{0.5cm}ll}
% % 		\toprule
% % \multicolumn{5}{c}{Ratio}             & \multicolumn{5}{c}{Delta}             \\\midrule
% % cid &\% jobs& outlier & $25-75^{th}$ & $95^{\text{th}}$ & std & cid &\% jobs & outlier & $25-75^{th}$ & $95^{\text{th}}$ & std \\\midrule
% % 0   &10.0& 0.25\%  & 0.17    & 1.29 & 1.45          & 0 &\textbf{40.8}&  1.93\%  & 4       & 28   & 155  \\
% % 1   & \textbf{36.5}& 1.63\%  & 0.06    & 1.41 & \textbf{2.46} & 1 &9.2  & 2.43\%  & 199     & 408  & 296  \\
% % 2   & 7.9& 0.25\%  & 0.19    & 1.34 & 0.82          & 2 &8.3  & 0.55\%  & 16      & 33   & 140  \\
% % 3   &6.3& 0.06\%  &\textbf{0.29}& \textbf{1.46} & 0.55 & 3 &14.6  & 0.98\%  & 31      & 63   & 153  \\
% % 4   &13.7& 0.42\%  & 0.11    & 1.20 & 0.93              & 4 &12.2  & 0.73\%  & 69      & 128  & 179  \\
% % 5   & 9.8& 0.26\%  & 0.20    & 1.37 & 0.97              & 5 &5.7  & 0.49\%  & 11      & 19   & 140  \\
% % 6   & 10.2& \textbf{1.66\%}  & 0.16    & 1.37 & 2.18     & 6 &1.7  & \textbf{24.23\%} & \textbf{936}     & \textbf{1359} & \textbf{2548} \\
% % 7   & 5.6& 1.46\%  & 0.17    & 1.35 & 1.94              & 7 &7.6  & 0.53\%  & 11      & 23   & 148 \\\bottomrule
% % \end{tabular}
% % \end{adjustbox}
% % \end{table}
% % \todo{sort clusters by some characteristic, e.g., 25-75th width, so that readers can have a mental model that puts clusters numbers on a spectrum for that characteristic. Explain the semantics. Explain the first and last row of the table. Also arrange above cluster plot accordingly.}

% \begin{table}[]
% 	\caption{Other statistics for the clusters.}\label{tab:statscluster}
% \begin{adjustbox}{max width=\columnwidth}
% \begin{tabular}{lllp{0.5cm}lllllp{1.0cm}p{0.8cm}l}
% 		\toprule
% \multicolumn{5}{c}{Ratio}             & \multicolumn{5}{c}{Delta}             \\\midrule
% cid &\% jobs& outlier & $25-75^{th}$ & $95^{\text{th}}$ & std & cid &\% jobs & outlier & $25-75^{th}$ (s)& $95^{\text{th}}$ (s)& std (s)\\\midrule
% 0   & \textbf{36.5} & 1.63\%                           & 0.06 & 1.41                           & \textbf{2.46} & 0  & \textbf{40.8} & 1.93\%                            & 4   & 28                             & 155                            \\
% 1   & 13.7                           & 0.42\%                           & 0.11 & 1.2                            & 0.93                           & 1  & 5.7  & 0.49\%                            & 11  & 19                             & 140                            \\
% 2   & 10.2                           & \textbf{1.66\%} & 0.16 & 1.37                           & 2.18                           & 2  & 7.6  & 0.53\%                            & 11  & 23                             & 148                            \\
% 3   & 10.0                             & 0.25\%                           & 0.17 & 1.29                           & 1.45                           & 3  & 8.3  & 0.55\%                            & 16  & 33                             & 140                            \\
% 4   & 5.6                            & 1.46\%                           & 0.17 & 1.35                           & 1.94                           & 4  & 14.6 & 0.98\%                            & 31  & 63                             & 153                            \\
% 5   & 7.9                            & 0.25\%                           & 0.19 & 1.34                           & 0.82                           & 5  & 12.2 & 0.73\%                            & 69  & 128                            & 179                            \\
% 6   & 9.8                            & 0.26\%                           & 0.20  & 1.37                           & 0.97                           & 6  & 9.2  & 2.43\%                            & 199 & 408                            & 296                            \\
% 7   & 6.3                            & 0.06\%                           & \textbf{0.29} & \textbf{1.46} & 0.55                           & 7  & 1.7  & \textbf{24.23\%} & \textbf{936} & \textbf{1359} & \textbf{2548} \\\bottomrule
% \end{tabular}
% \end{adjustbox}
% \end{table}
% % \todo{sort clusters by some characteristic, e.g., 25-75th width, so that readers can have a mental model that puts clusters numbers on a spectrum for that characteristic. Explain the semantics. Explain the first and last row of the table. Also arrange above cluster plot accordingly.}

% %\todo{add characteristics of each cluster and analysis}
% % \todo{give percentages of job groups in the clusters}




==> Runtime Variation in Distributed Systems (Short II) (2)/Conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

% Even with tremendous advantages over on-premise services, big data analytic platforms oftentimes suffer from high variability in job's runtime due to the dynamic nature of resource provisioning, scheduling, and co-location with other jobs. 
% While customers desire high reliability of job runtimes (sometimes more than faster performance) and operators needs to meet SLOs, little attention has been draw to evaluate the runtime variability of individual jobs in the production computing clusters.

%In this work, we conducted extensive analysis of the runtime variation of different job groups in a large-scale big data analytic system by proposing an innovative approach to associate each job with a predefined probability distribution. 
% The novelty of our approach is to be able to estimate the probabilities of extreme values despite not having a predictor of individual job runtimes that directly predicts them, but instead associates the job with the distribution of the cluster it belongs to.
%We showed that the shapes of these runtime distributions differ significantly according to (1) intrinsic job characteristics, (2) resource allocation and (3) cluster condition when the job is submitted. By developing a clustering model and a classification predictor, we infer the distribution category of normalized runtime with >95\% accuracy. Using an interpretable machine learning algorithm, we examined the sources of variation such as usage of spare tokens, instability of CPU utilization level on computing nodes, and fractions of vertices executed on different machine SKUs and quantified the improvement by adjusting these control variables. Joined with models to capture the dynamics of system utilization due to workload re-balancing such as KEA~\cite{zhu2021kea}, our approach can be used to optimize dynamically customer-centric performance of individual jobs.

In this work, we did an extensive analysis of the runtime variation of recurring production jobs on Microsoft Cosmos by systematically characterizing, modeling, predicting, and explaining job runtime variations. Our original 2-step approach computes a posterior likelihood for each job to associate it with a predefined probability distribution, whose shape 
differs according to (1) intrinsic job characteristics, (2) resource allocation and (3) cluster condition when the job is submitted. 
We infer the distribution of job runtime with >96\% accuracy, out-performing the traditional regression models and capturing better the long tail of the distribution. 
Using an interpretable machine learning algorithm, we examined the sources of variation such as usage of spare tokens, skewed load on computing nodes, fractions of vertices executed on different SKUs. We quantified the improvement by adjusting these control variables. 
Our techniques can be used along with models that capture the effects on system utilization with workload re-balancing to dynamically optimize the performance of individual jobs.

%Joined with models to capture the dynamics of system utilization due to workload re-balancing, our approach can be used to optimize dynamically customer-centric performance of individual jobs.

==> Runtime Variation in Distributed Systems (Short II) (2)/Control.tex <==
\section{Controlling Runtime Variation}
\label{sec:prescriptive}

%Prescriptive Analysis. 

Using the predictive model (Section~\ref{sec:model}) and drawing from the insights from the Shapley values (Section~\ref{sec:explain}), we now identify several what-if scenarios for scheduling and resource allocation and evaluate their performance. Based on the changes of jobs' runtime, one can quantitatively evaluate the detailed monetary impact.
%  on job performance and variation
%of several changes both from the operation side and the customer side to improve job performance by calling the prediction model directly on hypothetical scenarios. 

\subsection{Scenario1: Spare Token allocation}

% Spare tokens are additional resource tokens, beyond those requested for the jobs at submission time, and are dynamically allocated to jobs depending on their token utilization and availability of resources in the cluster. 
Availability of spare tokens depends on physical cluster conditions that are affected by the execution of other jobs and hence is a source of variation. Here we use our models to estimate the impact on runtime variation if spare tokens are not allocated.

% Table~\ref{table:whatifbonus} shows an example of the change in the predicted cluster by disabling the usage of spare tokens. 

% \todo{restate numbers from the Table like in the next paragraph?}
% \todo{any reasons for using Delta instead of Ratio for this scenario? if not, do findings qualitatively hold for Ratio as well?}
 
% \begin{figure}
% 	\centering
% 	\begin{minipage}[b]{.5\columnwidth}
% 		\includegraphics[width=\textwidth]{img/SHAP/whatifdelta/whatif_BonusTokens_avg_67626_box.png}
% 	\end{minipage}%
% 	\caption{Reduce spare tokens results in shift from Cluster 7 to 5 (\deltanorm). 
% 	\todo{can be combined (a), (b) with next fig for space savings.}
% 	}\label{fig:whatifbonus}
% \end{figure} 


% \begin{table}[]
% 	\caption{Reducing spare tokens shifts predictions from Cluster 2 to 1 (\deltanorm). 
% % 	\todo{can be combined (a), (b) with next fig for space savings.}
% 	}\label{table:whatifbonus}
% 	\begin{adjustbox}{max width=\columnwidth}
% \begin{tabular}{ccccccc}
% \toprule
% Name        & \multicolumn{6}{c}{Value}                                                  \\\midrule
% SpareTokensAvg & 0        & 2        & 4        & \textbf{6 (Origin)}       & 8        & 10             \\
% Prediction  & Cluster1 & Cluster2 & Cluster2 &\textbf{ Cluster2} & Cluster2 & Cluster2 \\\bottomrule
% \end{tabular}
% \end{adjustbox}
% \end{table}

With the predictor, we disable spare tokens for all jobs in the test set (dataset D3 as in Table~\ref{tab:datasets}). 
% Figure~\ref{fig:whatifbonusagg} shows the transition matrix, in percentages, of jobs with a different prediction for the cluster label.
%the changes of predicted labels among the jobs with a different prediction. 
%
% We can see that the most likely change is for jobs from Cluster 2 to 7, which indicates a >60\% reduction in the variation measure by the difference between $25^{\text{th}}$ and $75^{\text{th}}$ percentile (from 9.05s to less than 3s) as well as an 80\% reduction in the $95^{\text{th}}$ percentile (from 22.61s to 4.52s). The second and third significant change is for Cluster 1 to 4 and Cluster 6 to 1, which also indicates an improvement for the runtime distribution.
With \rationorm, 15\% of jobs that were predicted in Cluster 2 are now in Cluster 1, where the outlier probabilities gap between $25^{\text{th}}$ and $75^{\text{th}}$ percentiles, and the $95^{\text{th}}$ percentile of the normalized runtime are reduced (also see Table~\ref{tab:statscluster}). 
The second significant change is from Cluster 3 to 5 where the gap between 25 and $75^{\text{th}}$ percentile increased slightly from 0.17 to 0.19, while the standard deviation decreased dramatically (from 1.45 to 0.82). 
% However, we also observe a portion of jobs from Clusters 3, 4, 5 and 6 shifting to Cluster 1. Even though the gap between 25 and $75^{\text{th}}$ percentile is reduced, for some of such transitions, the probability of outliers increased, indicating a trade-off between more stable performance in general and a higher probability of extreme slowdown.
Similar changes can be seen for \deltanorm. Based on the predictor,
% and different job characteristics 
for the set of jobs desiring low variances, we propose disabling their usage of spare tokens to maximize performance improvement. \edit{In the production system, there has been work ongoing to reduce the maximum number for spare tokens as a multiplier of the number of allocated tokens. We observed that the jobs with fewer spare tokens runs slower but with less variance, which agrees with our model predictions.}

% \begin{figure}
% 	\centering
%     \subfloat[\rationorm]{	 
% 		\includegraphics[width=.5\columnwidth]{img/SHAP/whatif_agg/ratio/cm_lgbm_bonus_update_i.pdf}
%     \label{fig:whatifbonusaggratio}\vspace{-0.2cm}}
%     \subfloat[\deltanorm]{	 		\includegraphics[width=.5\columnwidth]{img/SHAP/whatif_agg/delta/cm_lgbm_bonus_update_i.pdf}
% 	\label{fig:whatifbonusaggdelta}\vspace{-0.2cm}}
% 	\vspace{-0.2cm}
% 	\caption{Transition matrix of prediction result after disabling spare tokens (\deltanorm).}\label{fig:whatifbonusagg}
% \end{figure} 

% \todo{can we also tell the corresponding impact on average performance? then we can discuss about stability vs high performance trade-off}

\subsection{Scenario2: Scheduling on later generation of machines}

A job's vertices can be executed by multiple machines in a distributed manner and as discussed in Section~\ref{subsec:sources-of-variation}, different job instances within the same group can be allocated to many different SKUs. Here we estimate the impact on runtime variation if we execute more vertices on later generations of machines.
% Figure~\ref{fig:whatifgen} shows one example where increasing the fraction of vertices to be finished on Gen3.5 machines shifts the prediction from Cluster 0 to 7 with \deltanorm where both the outlier probability and the $95^{\text{th}}$ percentile of the normalized runtime are reduced (also see Table~\ref{tab:statscluster}).

% \todo{restate numbers from the Table like in the next paragraph?}
% \yz{SKU fraction, summary for some features}

% \begin{figure}
% 	\centering
% 	\begin{minipage}[b]{.5\columnwidth}
% 		\includegraphics[width=\textwidth]{img/SHAP/whatifdelta/whatif_Wiwynn15_6TB_frac_avg_87684_box.png}
% 	\end{minipage}%
% 	\caption{Increase fraction of vertices on Gen3.5 machines results in shift from Cluster 0 to 7 (\deltanorm).
% 	\todo{can be combined (a), (b) with next fig for space savings.}
% 	}\label{fig:whatifgen}
% \end{figure} 

% Figure~\ref{fig:whatiffrac} shows the percentage of changed cluster labels among the jobs 
By shifting all the vertices (both fractions and count) from Gen3.5 to Gen5.2,
%
%changes of predicted label among the jobs with a different prediction 
%
the most likely change for 20.95\% of jobs is from Cluster 2 to 0, with a significant drop in the gap between 25 and $75^{\text{th}}$ percentile for \rationorm. And for \deltanorm, the most likely prediction change is from Cluster 1 to 0 where the gap between 25 and $75^{\text{th}}$ percentile dropped from 11s to 4s.

% \begin{figure}
% 	\centering
% 	    \subfloat[\rationorm]{
% 		\includegraphics[width=.5\columnwidth]{img/SHAP/whatif_agg/ratio/cm_lgbm_gen_S0.pdf}
% 	\label{fig:whatiffracratio}}%
% 	\subfloat[\deltanorm]{
% 		\includegraphics[width=.5\columnwidth]{img/SHAP/whatif_agg/delta/cm_lgbm_gen_S0.pdf}
%     \label{fig:whatiffracdelta}}%
%     \vspace{-3mm}
% 	\caption{Transition matrix of prediction result after shifting all vertices from Gen3.5 to 5.2}\label{fig:whatiffrac}
% \end{figure} 

% \todo{any reasons for using Delta instead of Ratio for this scenario? if not, do findings qualitatively hold for Ratio as well?}

%We find that 
Hence, it's better to run more vertices on later generation SKUs. However, our model doesn't capture the compounding of changes due to workload re-balancing, such as the changes of CPU utilization levels.
% (e.g., increasing for Gen5.2).
Models that can predict the utilization levels given different workload distributions can be easily integrated, such as in KEA~\cite{zhu2021kea}, to quantitatively capture this dynamic impact.
% in monetary values.

% this can increase operational costs, since more machines have to be provisioned for each SKU type to support reduced heterogeneity during scheduling, and may also reduce cluster utilization and increase job latencies as they wait for enough homogeneous resources to be available.

%it is more desired to have the change machine type (potentially the same machine) to process the full job, which can improve stability at the expense of provisioning cost.

\subsection{Scenario3: Improving load balance
%across machines
}

As discussed in Section~\ref{subsec:sources-of-variation}, physical cluster conditions such as load differences across machines are a source of runtime variation. Here we estimate this impact of more uniformly distributed loads.

% Figure~\ref{fig:whatifbalance} shows one example where reducing the standard deviation of CPU utilization shifts the prediction from Cluster 6 to 1 with \rationorm where the outlier probability is significantly reduced (also see Table~\ref{tab:statscluster}).

% \todo{restate numbers from the Table like in the next paragraph?}

% \begin{figure}
% 	\centering
% 	\begin{minipage}[b]{.5\columnwidth}
% 		\includegraphics[width=\textwidth]{img/SHAP/whatifratio/whatif_avg_Wiwynn17_cpu_std_70842_box.pdf}
% 	\end{minipage}%
% 	\caption{Reduce CPU utilization standard deviation results in shift from Cluster 6 to 1 (\rationorm).
% 	\todo{can be combined (a), (b) with next fig for space savings.}
% 	}\label{fig:whatifbalance}
% \end{figure} 

%
%changes of predicted label among the jobs with a different prediction 
%
If the standard deviation of CPU utilization could be reduced to 0 (i.e., equal load on all machines and at all times), with \rationorm, the most likely change is from Cluster 2 to 0 (29.78\% of jobs), with outlier probability reduced from 1.66\% to 1.63\% and the variation measured by the difference between the $25^{\text{th}}$ and $75^{\text{th}}$ percentiles reduced from 0.16 to 0.06. Similar improvement can be seen for \deltanorm. 
Thus there is significant monetary value that can be realized by a better scheduling system that further motivates other research projects for \cosmos.
% These  quantitative estimates show the improvements of better load balancing on  runtime stability.

% \todo{any reasons for using Ratio instead of Delta for this scenario? if not, do findings qualitatively hold for Delta as well?}

% From this analysis we conclude that balancing the load well across machines in the cluster is important for reducing the runtime variation of jobs running on those machines. While this is expected, 


% \begin{figure}
% 	\centering
% 	\subfloat[\rationorm]{
% 		\includegraphics[width=.5\columnwidth]{img/SHAP/whatif_agg/ratio/cm_lgbm_cpustd_i.pdf}
% 	\label{fig:whatifcpuratio}}%
% 	\subfloat[\rationorm]{
% 		\includegraphics[width=.5\columnwidth]{img/SHAP/whatif_agg/delta/cm_lgbm_cpustd_i.pdf}
% 	\label{fig:whatifcpudelta}}%
% 	\vspace{-3mm}
% 	\caption{Transition matrix of prediction result after reducing the standard deviation of CPU utilization (\rationorm).}\label{fig:whatifcpu}
% 	\vspace{-5pt}
% \end{figure} 


==> Runtime Variation in Distributed Systems (Short II) (2)/Distributions.tex <==
\subsection{Distributions}
\label{sec:clustering}


 
We represent runtime variation for each recurring job group by its \textit{runtime distribution}. Although there is a large variety in the runtimes of SCOPE jobs, we found that runtimes of many different jobs have similar probability distributions. We refer to these as \textit{shapes}. Knowing a job's distribution is sufficient to determine any characteristic of its variation, including the risk that its runtime will exceed a specified threshold. 
% represented as Probability Mass Functions (PMFs).

% we found that many different jobs have similar shapes of their runtime distribution curves. 
To compute the shapes, we first normalize the job runtimes, then compute their empirical Probability Mass Functions (PMFs, i.e., histogram).
Jobs are \textit{clustered}
% into \textit{groups} 
based on the similarity of their runtime distributions, and for any new job, we can predict the cluster it belongs to. We identify the job's PMF as that of the cluster it belongs to. This methodology allows us to generalize our analysis across different jobs and work instead with a small number of clusters that can be easily understood by the users.
% . This smaller number (in this case, just 8) can be easily understood by the user.

%moreover, to better generalize the analysis across different jobs which might have significantly different ranges of job runtime (but might share similar variation/shape of distribution), we normalize the job runtime by:

We used the following two normalization strategies to transform job runtimes, using medians computed on ``historic'' data from Dataset D1 as in Table~\ref{tab:datasets}:
% \begin{enumerate}[leftmargin=*]
% 	\item \textbf{\rationorm}: we take the ratio of job runtime to median runtime. For this scenario, we are interested in understanding the similarity in variation in terms of percentage change in runtimes in a relative term.
% 	\item \textbf{\deltanorm}: we take the difference of the two, i.e., job runtime - median runtime. For this scenario, we are interested in understanding the the similarity in variation of runtimes in an absolute term (seconds).
% \end{enumerate}  

\begin{definition}
\textit{The} \textbf{\rationorm}\textit{ is defined by the ratio of job runtime to its historic median, i.e., job runtime / median runtime. And }\textbf{\deltanorm}\textit{ is defined by the difference, job runtime - median runtime.}
\end{definition}

The \rationorm distribution measures relative change in runtimes, while the \deltanorm distribution measures the absolute deviation from median, measured in seconds. \edit{Note that runtime with various ranges can be normalized more effectively using ratio-normalization. E.g., absolute variations for long-running jobs are typically higher (1h$\pm$10min), whereas those for short-running jobs can be a lot lower. In this regard, ratio-normalization improves consistency and lumps together comparable distributions with different runtime ranges.
On the other hand, for very short or very long jobs, it might be less insightful to measure variances in percentage. For short-running jobs, the percentage can be very large (e.g., 5s$\pm$300\%). For long jobs, the percentage can be very small, leading to a very "thin" distribution measured by the ratio-normalization. Therefore, in this work, we leverage the delta-normalization combined with ratio-normalization to capture the variation in absolute terms.}
%We believe that both the distributions of the normalized runtime by \rationorm and \deltanorm are important in different scenarios. The ratio indicates the percentage variation benchmarked to the median, while the \deltanorm reveals the absolute deviation in the unit of seconds/minutes. 

Our clustering analysis to recover the ``typical'' distribution shape across jobs uses dataset D1 where only jobs with >20 occurrences are included for more accurate estimation for their runtime distribution. For each job group, we derive its histogram for the distribution of normalized runtimes and then use an unsupervised machine learning algorithm to cluster them. Note that the inputs to the clustering analysis are the PMF probabilities of each bin of the histogram as opposed to the job features (e.g., input size, etc.). 

Our principal design choices for the runtime distribution clustering method are as follows:
\begin{itemize}[leftmargin=*]
%	\item For the clustering analysis, we want to evaluate the distribution of runtime variances. In this case, we normalize the runtime by its median value in this distribution. There can be two possible way for this normalization: (1) divided by the median runtime to consider the ratio between the instance's runtime benchmarked to the median or (2) minus the median runtime to consdier the absolute deviation from the median time. Maybe we can use either one that has better predictability, i.e., if jobs runtime variation has more consistency measured in \% changes, we can use this as the prediction value and we can convert to the absolute runtime deviation. Similar for the inverse.
	\item \textbf{Bin size and Range}: 
% 	For calculating the distribution of the normalized runtime, the design of the bin size and range is critical. 
	The range should cover the majority of values with relatively fine granularity but not too small to capture fluctuation due to noise. 
% 	We also want to cover outliers (points in the stalagmites, that is, tails of the distributions) such that we can predict their probability of existence. Since they are rare, w
	We merge the outliers into one bin (based on being $\leq$ or $\geq$ some thresholds)\footnote{For \deltanorm, we use [-900, 900] (where 1\% of jobs are 1066s slower than median, we round down to 900s, i.e., 15 min), and for \rationorm, we use [0, 10] (where 1\% of jobs are 10.6x slower than median, we round down to 10x). Jobs >900s or 10x slower than median are defined as outliers.}.  
	We evaluated 50, 100, 200 and 500 bins, and chose 200 bins that has relatively smooth PMF curves, and different shapes of distributions are observable.
    \item \textbf{Clustering algorithm}: Hierarchy clustering based on dendrogram~\cite{nielsen2016introduction} and Agglomerative clustering~\cite{rokach2005clustering} take different distance metrics, linkage methods, and user-specified number of clusters. However, they result in imbalanced clusters (some with >90\% of the data in one cluster). K-means clustering~\cite{sculley2010web} resulted in more balanced clusters, so is chosen for the following analysis. 
	\item \textbf{Number of clusters}: It is determined based on: (i) numeric analysis of \textit{inertia}, defined by the sum of squared distances between each sample and its cluster centroid (we pick an elbow point where adding more clusters does not significantly decrease the inertia), %by a significant amount %(see Figure~\ref{fig:k})%, 
	and (ii) by visually examining the clustering results to check if the clusters are sufficiently different from each other and have unique characteristics. 
% 	We picked 8 clusters for both \deltanorm and \rationorm for consistency.
	\item \textbf{Smoothing histograms}: The standard clustering algorithms are based on using PMF probabilities as input vectors assuming each dimension is independent. In reality, adjacent density values of bins (e.g., the probability of a runtime being in the $4^{\text{th}}$ or $5^{\text{th}}$ bin) are correlated. However, with any distance measurement (e.g., dot product), correlation between adjacent bins is not considered.
% 	whereas it is easy to observe cases where for job A, its $4^{\text{th}}$ bin's value equals to that of the $5^{\text{th}}$ bin for job B due to random noises. 
	Therefore, we introduce a \textit{smoothing step} after deriving the PMFs to jointly consider any adjacent bins' values such that the two smoothed vectors mentioned above will have a higher affinity. 
% 	Carefully chosen bin size (as discussed above) also helps 
	%in this situation 
% 	reduce the effect of variation due to noises and smooth the curve. 
\end{itemize}

%\begin{figure}[t]
%	\centering
%	%\vspace{-3ex}
%	\includegraphics[width=0.6\columnwidth]{img/k.pdf}
%	% 	\vspace{-0.8cm}
%	\caption{Picking the optimal number of clusters.}\label{fig:k}
%	% 	\vspace{-0.6cm}
%\end{figure}


%\begin{figure}
%	\centering
%	\centering
%	\begin{minipage}[b]{\columnwidth}
%		\includegraphics[width=\textwidth]{img/hist_normed_kmeans_8_bins_merge_tail_ratio0210_min_3/cluster_all.pdf}
%	\end{minipage}%
%	
%	\begin{minipage}[b]{\columnwidth}
%		\includegraphics[width=\textwidth]{img/hist_normed_kmeans_8_bins_merge_tail_delta0210_min_3/cluster_all.pdf}
%	\end{minipage}%
%	% 	\vspace{-3mm}
%	\caption{8 typical distribution of normalized runtime.
%	}\label{fig:clustering}
%\end{figure} 

Figure~\ref{fig:clustering} shows the distributions for the 8 clusters using \rationorm and \deltanorm policies. We see that some distributions have two modes (e.g., Cluster 0, 2, 4 using \rationorm) and with different variances. Table~\ref{tab:statscluster} summarizes important statistics for each cluster. 
% For example, Cluster 0 with \rationorm contains 36.5\% of the total job observations; its outlier probability is 1.63\% (defined by $\geq 10$x slower than median for \rationorm); 
For example, Cluster 0 with \rationorm has a outlier probability of 1.63\% (defined by $\geq 10$x slower than median for \rationorm);
the difference between 25 and $75^{\text{th}}$ percentile is 0.06; the $95^{\text{th}}$ percentile of this distribution is 1.41, and the standard deviation is 2.46. 
%While for Cluster 7 with \rationorm, 
The outlier probability decreases to 0.06\% for Cluster 7 with \rationorm.
Clusters are ranked according to the difference between the $25^{\text{th}}$ and $75^{\text{th}}$ percentiles.
% \begin{figure}
% 	\centering
% 	\centering
% 	\begin{minipage}[b]{\columnwidth}
% 		\includegraphics[width=\textwidth]{img/hist_normed_kmeans_8_bins_merge_tail_ratio0210_min_3/cluster_all_idx_cut.pdf}
% 	\end{minipage}%
	
% 	\begin{minipage}[b]{\columnwidth}
% 		\includegraphics[width=\textwidth]{img/hist_normed_kmeans_8_bins_merge_tail_delta0210_min_3/cluster_all_idx_cut.pdf}
% 	\end{minipage}%
% 	% 	\vspace{-3mm}
% 	\caption{8 typical distribution of normalized runtime.
% 	}\label{fig:clustering}
% \end{figure} 


		
% \begin{table}[]
% 	\begin{tabular}{llllllll}
% 		\toprule
% 		\multicolumn{4}{c}{Ratio}              & \multicolumn{4}{c}{Delta}             \\ \midrule
% 		cid & outlier & 25-75th         & 95th  & cid & outlier & 25-75th      & 95th    \\ \midrule
% 		0   & 0.25\%  & 0.15            & 1.31 & 0   & 0.01\%  & $\leq$3      & 13.57  \\
% 		1   & 1.63\%  & $\leq$0.02      & 1.31 & 1   & 0.04\%  & 162.81       & 502.01 \\
% 		2   & 0.25\%  & 0.15            & 1.31 & 2   & 0.00\%  & 9.05         & 22.61  \\
% 		3   & 0.06\%  & \textbf{0.20}           & \textbf{1.66} & 3   & 0.01\%  & 18.09        & 40.70  \\
% 		4   & 0.42\%  & 0.05            & 1.16 & 4   & 0.03\%  & 72.36        & 185.43 \\
% 		5   & 0.26\%  & 0.15            & 1.36 & 5   & 0.00\%  & $\leq$3      & 4.52   \\
% 		6   & \textbf{1.66\%}  & 0.10            & 1.41 & 6   & \textbf{0.26\%}  & \textbf{1591.96}    & \textbf{890.95} \\
% 		7   & 1.46\%  & 0.10            & 1.26 & 7   & 0.00\%  & $\leq$3      & 4.52  \\\bottomrule
% 	\end{tabular}
% 	\caption{Other statistics for 8 clusters.
% }\label{tab:statscluster0}
% \end{table}

% \begin{table}[]
% 	\caption{Other statistics for 8 clusters.}\label{tab:statscluster}
% \begin{adjustbox}{max width=\columnwidth}
% \begin{tabular}{lllp{0.5cm}lllllp{0.5cm}ll}
% 		\toprule
% \multicolumn{5}{c}{Ratio}             & \multicolumn{5}{c}{Delta}             \\\midrule
% cid &\% jobs& outlier & $25-75^{\text{th}}$ & $95^{\text{th}}$ & std & cid &\% jobs & outlier & $25-75^{\text{th}}$ & $95^{\text{th}}$ & std \\\midrule
% 0   &10.0& 0.25\%  & 0.17    & 1.29 & 1.45          & 0 &\textbf{40.8}&  1.93\%  & 4       & 28   & 155  \\
% 1   & \textbf{36.5}& 1.63\%  & 0.06    & 1.41 & \textbf{2.46} & 1 &9.2  & 2.43\%  & 199     & 408  & 296  \\
% 2   & 7.9& 0.25\%  & 0.19    & 1.34 & 0.82          & 2 &8.3  & 0.55\%  & 16      & 33   & 140  \\
% 3   &6.3& 0.06\%  &\textbf{0.29}& \textbf{1.46} & 0.55 & 3 &14.6  & 0.98\%  & 31      & 63   & 153  \\
% 4   &13.7& 0.42\%  & 0.11    & 1.20 & 0.93              & 4 &12.2  & 0.73\%  & 69      & 128  & 179  \\
% 5   & 9.8& 0.26\%  & 0.20    & 1.37 & 0.97              & 5 &5.7  & 0.49\%  & 11      & 19   & 140  \\
% 6   & 10.2& \textbf{1.66\%}  & 0.16    & 1.37 & 2.18     & 6 &1.7  & \textbf{24.23\%} & \textbf{936}     & \textbf{1359} & \textbf{2548} \\
% 7   & 5.6& 1.46\%  & 0.17    & 1.35 & 1.94              & 7 &7.6  & 0.53\%  & 11      & 23   & 148 \\\bottomrule
% \end{tabular}
% \end{adjustbox}
% \end{table}
% \todo{sort clusters by some characteristic, e.g., 25-75th width, so that readers can have a mental model that puts clusters numbers on a spectrum for that characteristic. Explain the semantics. Explain the first and last row of the table. Also arrange above cluster plot accordingly.}
\begin{figure}[h]
\vspace{-0.2cm}
	\centering
	\subfloat[\edit{\rationorm}]{\includegraphics[width=0.7\columnwidth]{img/hist_normed_kmeans_8_bins_merge_tail_ratio0210_min_3/cluster_all_idx.pdf}\vspace{-0.1cm}}\\
    \subfloat[\edit{\deltanorm}]{
		\includegraphics[width=0.7\columnwidth]{img/hist_normed_kmeans_8_bins_merge_tail_delta0210_min_3/cluster_all_idx.pdf}\vspace{-0.3cm}}
	 	\vspace{-1mm}
	\caption{\edit{Typical distributions of normalized runtime.
	}}\label{fig:clustering}
	% \vspace{-0.6cm}
\end{figure} 
\begin{table}[h]
	\caption{Statistics for the clusters of runtime distributions.}\label{tab:statscluster}
	% \vspace{-0.3cm}
\begin{adjustbox}{max width=0.67\columnwidth}
\begin{tabular}{lp{0.8cm}p{0.5cm}ll|lp{0.8cm}p{1.0cm}p{0.8cm}l}
		\toprule
\multicolumn{5}{c}{Ratio}             & \multicolumn{5}{c}{Delta}             \\\midrule
cid & outlier (\%) & $25-75^{\text{th}}$ & $95^{\text{th}}$ & std & cid & outlier (\%) & $25-75^{\text{th}}$ (s)& $95^{\text{th}}$ (s)& std (s)\\\midrule
0   &  1.63                           & 0.06 & 1.41                           & \textbf{2.46} & 0  & 1.93                            & 4   & 28                             & 155                            \\
1   &  0.42                           & 0.11 & 1.2                            & 0.93                           & 1  & 0.49                            & 11  & 19                             & 140                            \\
2   &  \textbf{1.66} & 0.16 & 1.37                           & 2.18                           & 2  & \edit{0.53}                            & 11  & 23                             & 148                            \\
3   &  0.25                           & 0.17 & 1.29                           & 1.45                           & 3  & 0.55                            & 16  & 33                             & 140                            \\
4   & 1.46                           & 0.17 & 1.35                           & 1.94                           & 4  & 0.98                            & 31  & 63                             & 153                            \\
5   & 0.25                           & 0.19 & 1.34                           & 0.82                           & 5  & 0.73                            & 69  & 128                            & 179                            \\
6   & 0.26                           & 0.20  & 1.37                           & 0.97                           & 6  & 2.43                            & 199 & 408                            & 296                            \\
7   & 0.06                           & \textbf{0.29} & \textbf{1.46} & 0.55                           & 7  & \textbf{24.23} & \textbf{936} & \textbf{1359} & \textbf{2548} \\\bottomrule
\end{tabular}
\end{adjustbox}
	\vspace{-0.4cm}
\end{table}
% \begin{table}[h]
% 	\caption{Statistics for the clusters of runtime distributions.}\label{tab:statscluster}
% 	\vspace{-0.2cm}
% \begin{adjustbox}{max width=\columnwidth}
% \begin{tabular}{llp{0.8cm}p{0.5cm}ll|llp{0.8cm}p{1.0cm}p{0.8cm}l}
% 		\toprule
% \multicolumn{5}{c}{Ratio}             & \multicolumn{5}{c}{Delta}             \\\midrule
% cid &\% jobs& outlier (\%) & $25-75^{\text{th}}$ & $95^{\text{th}}$ & std & cid &\% jobs & outlier (\%) & $25-75^{\text{th}}$ (s)& $95^{\text{th}}$ (s)& std (s)\\\midrule
% 0   & \textbf{36.5} & 1.63                           & 0.06 & 1.41                           & \textbf{2.46} & 0  & \textbf{40.8} & 1.93                            & 4   & 28                             & 155                            \\
% 1   & 13.7                           & 0.42                           & 0.11 & 1.2                            & 0.93                           & 1  & 5.7  & 0.49                            & 11  & 19                             & 140                            \\
% 2   & 10.2                           & \textbf{1.66} & 0.16 & 1.37                           & 2.18                           & 2  & 7.6  & 0.53\%                            & 11  & 23                             & 148                            \\
% 3   & 10.0                             & 0.25                           & 0.17 & 1.29                           & 1.45                           & 3  & 8.3  & 0.55                            & 16  & 33                             & 140                            \\
% 4   & 5.6                            & 1.46                           & 0.17 & 1.35                           & 1.94                           & 4  & 14.6 & 0.98                            & 31  & 63                             & 153                            \\
% 5   & 7.9                            & 0.25                           & 0.19 & 1.34                           & 0.82                           & 5  & 12.2 & 0.73                            & 69  & 128                            & 179                            \\
% 6   & 9.8                            & 0.26                           & 0.20  & 1.37                           & 0.97                           & 6  & 9.2  & 2.43                            & 199 & 408                            & 296                            \\
% 7   & 6.3                            & 0.06                           & \textbf{0.29} & \textbf{1.46} & 0.55                           & 7  & 1.7  & \textbf{24.23} & \textbf{936} & \textbf{1359} & \textbf{2548} \\\bottomrule
% \end{tabular}
% \end{adjustbox}
% 	\vspace{-0.5cm}
% \end{table}
% \todo{sort clusters by some characteristic, e.g., 25-75th width, so that readers can have a mental model that puts clusters numbers on a spectrum for that characteristic. Explain the semantics. Explain the first and last row of the table. Also arrange above cluster plot accordingly.}

%\todo{add characteristics of each cluster and analysis}
% \todo{give percentages of job groups in the clusters}



==> Runtime Variation in Distributed Systems (Short II) (2)/Explain.tex <==
\section{Explaining Runtime Variation}
\label{sec:explain}

In this section, we conduct \textit{descriptive analysis} to better understand the job characteristics that lead to different runtime distributions. 
Starting with the classification models from the previous section, we use machine learning explanation tools to better understand the sources of runtime variation. 

% \subsection{Correlation-based Approach}
% % \yz{a little bit too long to move to challenges... keep the same place, difficult to select features, which is large, second, missing features}
% A simple approach to start with is to examine the correlation between the different job characteristics. 
% Figure~\ref{fig:corr} shows the correlation plot for every pair of features using Pearson correlation~\cite{benesty2009pearson}. The color of the shaded circles indicates the sign/direction of correlation (blue: positive, red: negative), and their diameter and color intensity is proportional to the magnitude of the correlation.
% We can see that the CPU variation is positively correlated to the COV, and there is a cluster of features (including VertexCounts and DataRead) that are also positively correlated. However, it is difficult to reveal non-linear correlation in this plot. For example, as we showed earlier (Section~\ref{sec:model}), AvgRowLength and TotalDataRead both affect the runtime distribution and its variance, but that is not apparent from this plot. 
% % Even for a subset of the features, the complex correlation is difficult to capture.

% \begin{figure}[t]
% 	\centering
% 	%\vspace{-3ex}
% 		\includegraphics[width=1\columnwidth]{img/rplot0224.PNG}
% % 	\includegraphics[width=1\columnwidth]{img/Rplot.pdf}
% 	% 	\vspace{-0.8cm}
% 	\caption{Correlation plot.}\label{fig:corr}
% 	% 	\vspace{-0.6cm}
% \end{figure}

\subsection{Shapley Value}

Shapley values~\cite{shapley1953value,lundberg2017unified} that explain the contribution of each ``player'' in a game-theoretic setting have been adopted for explaining the contribution of features in ML models. In our context, based on the predictors developed in Section~\ref{sec:model}, they explain the quantitative contribution of each feature by randomly permuting other feature values and evaluating the marginal changes of the predictions~\cite{molnar2020interpretable}. 

% Specifically, for a data point with observed feature values, $x_1, x_2, \cdots, x_p$, the Shapley value for feature $j$, $\Delta_j(v)$, is calculated as the weighted sum over the marginal changes of the prediction before and after setting the feature $j$ to its observed value (i.e., $x_j$), while the other features are marginalized as in Equation~\ref{eq:margin}. For each randomly selected subset of features $S \ \mbox{s.t.} j \notin S$, we compute the difference between (1) the prediction marginalized over all other features not in $S$, which would include $x_j$, and (2) the prediction marginalized over all other features not in $S\cup j$, which would \textit{not} include $x_j$:

% \begin{align}
% &	\Delta_j(v) = \sum_{S \subseteq \{1,\cdots, p\} \setminus
% 		\{j\}} \frac{|S|!\; (p-|S|-1)!}{p!}\left(v(S\cup\{j\})-v(S)\right) \\
% &	v(S) = \int_{\mathbb{R}}\hat f(x_1, \cdots , x_p) d\mathbb{P}_{x \notin S} - E_X(\hat f (X)) \label{eq:margin}
% \end{align}
% where $\hat f$ is the prediction function, and $v(S)$ is the prediction for feature values that are marginalized over ones that are not included in set $S$.

% Figure~\ref{fig:waterfall} shows an example of the Shapley values for one job instance and the contribution of different features to the prediction score of Cluster 2 (with \rationorm). Starting at the bottom of the list of features, one sees that the baseline prediction of likelihood score is $E[f(x)]=-6.1$. Then one sums the incremental contributions from the bottom up starting with the 86 other feature values for this particular job instance, which decrease the predicted likelihood by $1.6$, MaxTokenAvg=58.059, which decreases the predicted likelihood by $0.5$,  HistCluster2=-41.336, which increases the likelihood by $0.84$, and so on.
% Thus the sum of the contributions of all features (e.g., $-1.6, -0.2, 0.84\ldots$) and the baseline prediction, -6.1, is equal to the final prediction, -7.519. 
% Since the feature value HistCluster2=-41.336 (representing the likelihood of belonging to Cluster 2 with historic data) increases the prediction score significantly by 0.84, it indicates that this feature increases the likelihood of this job belonging to Cluster 2 in the future (target value). This shows that past run profiles are good indicators for future runs. 
% % Though, we also tested the model without using such features (e.g., HistClusterX) and the accuracy didn't decrease significantly, which indicates that the other features are also informative to predict the cluster.

% % \todo{should we understand this as a small/large increase? mention if it is surprising/contrary to what one would expect.}
% % \todo{make the distinction between Cluster and Cluster clear. maybe in previous section?}
% % \todo{explain blue vs red color in the waterfall plot}

% % \begin{figure}[t]
% % 	\centering
% % 	%\vspace{-3ex}
% % 	\includegraphics[width=1\columnwidth]{img/SHAP/waterfall/shap_indi_2_1002_lgbm.png}
% % 		\vspace{-0.8cm}
% % 	\caption{Waterfall plot (blue is negative contribution, and red is positive).}\label{fig:waterfall}
% % 		\vspace{-0.4cm}
% % \end{figure}

% Figure~\ref{fig:summary} shows the Shapley value distribution for Cluster 6's prediction with \deltanorm for the top-20 important features\footnote{The result of feature importance based on Shapley value and the Gini importance used as in Figure~\ref{fig:fimportance} can be different. While the Shapley values are both consistent and accurate in terms of measuring feature contribution~\cite{lundberg2017unified}, its computation is usually quite time-consuming. More discussion on the comparison between the two can be seen at~\cite{rodriguez2019interpretation,fimportance}.}, ranked by the mean of absolute Shapley values. 
% % \yz{added importance metrics differences}
% It shows the distribution of Shapley values (along the x-axis) for each corresponding feature (color-coded). For TotalDataReadAvg, towards the right of the x-axis, the red color indicates that jobs with a higher value of TotalDataReadAvg tend to have higher Shapley values, which leads to a higher likelihood of being in Cluster 6. Similarly, we can see that jobs with large input size (e.g., TotalDataReadAvg, TotalDataReadStd colored red), small AvgTokensAvg but large MaxTokensAvg are with higher Shapley score contribution to the prediction of this cluster (to the right of the x-axis), indicating that jobs with these characteristics are more likely to be in Cluster 6.
%Note Cluster 6 has large variation and high probability of outliers. 
% On the contrary, for Cluster 0 with \rationorm, the jobs with small input size have higher Shapley values, which indicates that small jobs are more likely to be in Cluster 0. One can also observe that the distributions of CPU, such as avgGen5.2CPUAvg and avgGen3.5CPUStd also play an important role for the score.

% \todo{tie it back to high-level semantics -- what it does it mean for variation, probability of belonging to the tail, etc. also refer to Cluster 1 characteristics in Table~\ref{tab:statscluster}.}
% \todo{are these surprising findings? explain if so.}
% \begin{figure}[h]
% 	\centering
% % 	\begin{minipage}[b]{.65\columnwidth}
% % 	\includegraphics[width=\textwidth]{img/SHAP/summary/shap_ratio_1_ST.png}
% % 	\end{minipage}%
% % 	\begin{minipage}[b]{.35\columnwidth}
% % 	\includegraphics[width=\textwidth]{img/SHAP/summary/cluster_0_idx_ratio.pdf}
% % 	\end{minipage}%
% 	\begin{minipage}[b]{.65\columnwidth}
% 		\includegraphics[width=\textwidth]{img/SHAP/summary/shap_delta_1_ST.png}
% 	\end{minipage}%
% 	\begin{minipage}[b]{.35\columnwidth}
% 	\includegraphics[width=\textwidth]{img/SHAP/summary/cluster_6_idx_delta.pdf}
% 	\end{minipage}%
% 		\vspace{-0.2cm}
% 	\caption{Summary plot that shows the distribution of Shapley values with respect to the feature value (color-coded).}\label{fig:summary}
% \end{figure} 
 \begin{figure}
	\centering
    \subfloat[By Input Size\label{fig:indi_contribution}]{			\includegraphics[width=.4\columnwidth]{img/SHAP/indi_contribution/delta/Shap_total_data_read.pdf}\vspace{-8pt}}
    \subfloat[By operator counts\label{fig:indi_contribution2}]{			\includegraphics[width=.4\columnwidth]{img/SHAP/delta_op/indexlookup.pdf}\vspace{-8pt}}
    \vspace{-2mm}
	\caption{SHAP value distribution.}
	\vspace{-0.6cm}
\end{figure} 
% To better understand the detailed contribution change, 
Figure~\ref{fig:indi_contribution} illustrates the distribution of Shapley values with respect to the total input data read, where each dot corresponds to one job instance. We can see that jobs with large input size are more likely to be in Cluster 6 (as their feature values lead to higher Shapley values and a thus higher likelihood of being in Cluster 6) using \deltanorm. Note that Cluster 6 has a relatively high variance and high probability of outliers. 
Similar trends can be found for jobs with fewer tokens.
\begin{center}
\shadowbox{
\begin{minipage}{0.9\linewidth}
    \textbf{Insight:} 
    % For \deltanorm, 
    Jobs with larger inputs and using fewer tokens are more likely to have a large variation. A larger number of tokens can potentially evacuate other jobs from the same machine, which potentially reduces interference and the impact of noisy neighbors.
\end{minipage}
}\vspace{-3pt}
\end{center}
Similarly, job characteristics such as operator counts significantly impact the prediction, indicating that the existence of certain operators more likely results in different runtime distributions (see Figure~\ref{fig:indi_contribution2} for Shapley values for Cluster 6 with \deltanorm). 


% \todo{list some operators, will be particularly interesting to DB community}

% \begin{figure}
% 	\centering
% 	\begin{minipage}[b]{.45\columnwidth}
% 		\includegraphics[width=\textwidth]{img/SHAP/delta_op/shap_PhyOp_IdxLookup_Time_1_box.pdf}
% 	\end{minipage}\hfill%
% 	\begin{minipage}[b]{.45\columnwidth}
% 		\includegraphics[width=\textwidth]{img/SHAP/delta_op/shap_PhyOp_Window_Time_1_box.pdf}
% 	\end{minipage}%
% 		\vspace{-0.2cm}
% 	\caption{SHAP value vs. operator counts.}\label{fig:indi_contribution2}
% 		\vspace{-0.4cm}
% \end{figure} 

\begin{center}
\shadowbox{
\begin{minipage}{0.9\linewidth}
    \textbf{Insight:} Certain operator counts, such as Index-Lookup, Window, and Range, increase the variation.
\end{minipage}
}\vspace{-3pt}
\end{center}



% \todo{what are our conclusion from the figures? what are the high-level takeaways? what are surprising findings?}

%  \begin{figure}
%  	\centering
%  	\begin{minipage}[b]{.45\columnwidth}
%  		\includegraphics[width=\textwidth]{img/SHAP/indi_contribution/ratio/1/shap_avg_Dell17_cpu_avg_1.png}
%  	\end{minipage}\hfill%
%  	\begin{minipage}[b]{.45\columnwidth}
%  		\includegraphics[width=\textwidth]{img/SHAP/indi_contribution/ratio/1/shap_avg_Dell17_cpu_avg_6.png}
%  	\end{minipage}%
 
%   	\begin{minipage}[b]{.45\columnwidth}
% 	 	\includegraphics[width=\textwidth]{img/SHAP/indi_contribution/ratio/1/shap_avg_Gen6_cpu_std_1.png}
% 	 \end{minipage}\hfill%
% 	 \begin{minipage}[b]{.45\columnwidth}
% 	 	\includegraphics[width=\textwidth]{img/SHAP/indi_contribution/ratio/1/shap_avg_Gen6_cpu_std_6.png}
% 	 \end{minipage}%
 
% 	 \begin{minipage}[b]{.45\columnwidth}
% 		\includegraphics[width=\textwidth]{img/SHAP/indi_contribution/ratio/1/shap_BonusTokens_avg_1.png}
% 	\end{minipage}\hfill%
% 	\begin{minipage}[b]{.45\columnwidth}
% 		\includegraphics[width=\textwidth]{img/SHAP/indi_contribution/ratio/1/shap_BonusTokens_avg_6.png}
% 	\end{minipage}%
%  	\caption{SHAP value distributions with respect to feature values.}\label{fig:indi_contribution3}
%  	\vspace{-5pt}
%  \end{figure}  

Using \rationorm, Cluster 0 has smaller variance and smaller probability of outliers than Cluster 2, while both have two modes. Focusing on a set of high-importance features, we compare the Shapley values for predicting these two clusters and found that, with lower CPU utilization, standard deviation and low usage of spare tokens, jobs are more likely to be in Cluster 0 (with more reliable performance) compared to Cluster 2. In general, we expect that machines with high utilization levels or standard deviations will have less reliable performance, which coincides with our observations here. The usage of spare tokens (whose availability is less predictable) can also lead to less stable runtimes. 
% With our method, one can quantitatively evaluate the resulting performance change based on the cluster properties as in Table~\ref{tab:statscluster}.

\begin{center}
\shadowbox{
\begin{minipage}{0.9\linewidth}
    \textbf{Insight:} 
    %Comparing two similar clusters, we conclude that 
    Lower CPU utilization (load), lower standard deviation, and less use of spare tokens can improve runtime reliability.
\end{minipage}
}\vspace{-3pt}
\end{center}

% \todo{what about other clusters? summarize findings.}
% \todo{what are the new/surprising things that we found from this analysis? Are there new insights that we can add to our list of contributions?}

% One can calculate the Shapley value for all the job instances to examine the contribution of each feature given its values and compare their contribution to the raw scores of different classes. 
% Expanding to the prediction for all clusters, Figure~\ref{fig:shapcorr} summarizes the Pearson-correlation between the Shapley values and the feature values for the top-10 important features across the prediction for all clusters (the joint set, excluding HistCluserX features as they are obviously important for prediction of the corresponding cluster). The x-axis shows the index of the clusters and y-axis lists the different features. 
% By examining Pearson-correlation between the Shapley values and the feature values for the top-10 important features across the prediction for all clusters, we found that
% : (1) for the \deltanorm, the feature values of TempDataReadAvg and TotalDataReadAvg have a high positive correlation with the Shapley value for Clusters 6 and 7 but a negative correlation with the Shapley value for Clusters 0 and 1. For a job instance with a larger input size (potentially a longer runtime), these features tend to increase the predicted likelihood of being in Clusters 6 and 7 (as Shapley values would increase with a positive correlation with the feature value) and decrease for Clusters 0 and 1.  For \rationorm, the trend is less visible, indicating that variance measured by the absolute difference between the runtime and the median is more sensitive to the size of the job; (2) many operators also have a significant impact on the cluster prediction and some have a clear trend of pushing towards Clusters 6 and 7 with higher values, such as PhyOpRangeCount; (3) 
For \rationorm, increasing the vertex count on Gen5 and Gen6 (newer generations) tends to shift the prediction to Clusters 0 and 1, indicating that running vertices on those machine SKUs can potentially help with the runtime variation. Compared with Gen3 and Gen4 machines, those are in general faster and with large resource capacity~\cite{zhu2021kea}. 
% Though for some features, the trend from Clusters 0 to 7 is less visible and detailed analysis with respect to each cluster is needed.
% Comparing Clusters 0 and 1 with \rationorm, the value of AvgGen3.5CPUStd has a positive correlation with Cluster 0 (with higher probability of outliers) while a negative correlation with Cluster 1 where the outlier probability is lower but with a larger gap between the 25 and $75^{th}$ percentile. 
% We also observe that in general, higher CPU utilization results in higher probability of being in Clusters 5, 6, and 7, which indicates the potential impact of noisy neighbours. 
% \begin{figure}
%  	\centering
%     \subfloat[\rationorm]{	 		\includegraphics[width=.48\columnwidth]{img/SHAP/summary/corr_shap_ratio_imp.pdf}
%     \label{fig:shapcorrratio}\vspace{-0.2cm}}\hfill
%     \subfloat[\deltanorm]{	 		\includegraphics[width=.48\columnwidth]{img/SHAP/summary/corr_shap_delta_imp.pdf}
%     \label{fig:shapcorrdelta}\vspace{-0.2cm}}
%     \vspace{-0.2cm}
% \caption{Shapley value and feature value correlation (blue means positively correlated, and red means negative).}\label{fig:shapcorr}
%  \end{figure}  
 
 \begin{center}
\shadowbox{
\begin{minipage}{0.9\linewidth}
    \textbf{Insight:} The model identified certain SKUs where larger vertex count on those machines increases the likelihood of Clusters 0 and 1, which have smaller variance.
    % with \rationorm.
\end{minipage}
}\vspace{-3pt}
\end{center}

% To accurately evaluate the quantitative impact of the prediction change, examining the Shapley values might not be sufficient as it only captures the changes of the prediction score but not directly the final predicted cluster label.

==> Runtime Variation in Distributed Systems (Short II) (2)/Introduction2.tex <==

\section{Introduction}
\label{sec:intro}



Big Data platforms have become ubiquitous over the last decade, enabling scalable data processing with high efficiency, security, and usability~\cite{zaharia2010spark, thusoo2009hive,tigani2014google,chaiken2008scope,diaz2018azure,ramakrishnan2017azure,aws-athena, sarkar2018learning}. 
% Cloud and serverless computing in particular offers greater flexibility and ease of dynamically provisioning resources on demand, in contrast to fixed-resource on-premises computing systems, while also transparently and efficiently managing the resources and meeting Service Level Objectives (SLOs) for performance and availability.
However, the dynamic nature of resource provisioning, scheduling, and co-location with other jobs can cause occasional job slowdowns. Additionally, intrinsic properties of the job such as parameter values and input data sizes can change across repeated runs leading to variations in runtime. Figure~\ref{fig:example-variation} shows a set of recurring jobs in \cosmos~\cite{power2021cosmos}, a Big Data analytics platform at Microsoft, submitted with different frequencies. We can see that some jobs have more stable runtime while some have occasional slow downs with non-regular patterns. But, it is not apparent \textit{why such variations are happening}, \textit{how they can be mitigated}, or \textit{how likely it is for the next job run to be an outlier} compared to historic runs.

%With increasing data volume, 
\begin{figure}[t]
	\centering
%			\vspace{-0.3cm}
			\includegraphics[width=0.65\columnwidth]{img/jobs/jobs85.pdf}
			\vspace{-0.4cm}
\caption{\edit{Recurring jobs with runtime variation.}}
			\vspace{-0.4cm}
\label{fig:example-variation}
\end{figure}
%with more reliable services and identify potential issues of the clusters.  

%Other than fast performance, 
% Customers desire high reliability of their job runtimes~\cite{jyothi2016morpheus}. In production scenarios, jobs are often scheduled or pipelined with strong data dependencies (jobs using other jobs' output data as inputs)~\cite{chung2020unearthing}. Stability and predictability of job runtimes is an important factor that affects the fundamental design and architecture of data processing pipelines. 
% Unfortunately, they are oftentimes neglected by operators due to the difficulties of assessment.
% %In order to set up the data processing pipelines, the runtime predictability is a crucial input for developers and sometimes affects their architecture design.
% Occasional job slowdowns are inevitable~\cite{shao2019griffon}, a quantitative prediction of the variation helps to appropriately account for such slowdowns. A better understanding of job runtime variation is thus valuable both to users, for managing their computation jobs, and to cloud service providers for meeting SLOs while minimizing resource provisioning costs, for analyzing and mitigating performance violations, and for improving the service quality.

% --- Rewrite ---
% A better understanding of job runtime variations is valuable for users to be able to rely on the predictability of their pipeline execution~\cite{jyothi2016morpheus}, and for cloud service providers to meet SLOs while minimizing resource provisioning costs, to analyze and mitigate performance violations, and to improve service quality.
In production systems, jobs are often scheduled or pipelined with strong data dependencies
(jobs using other jobs' output data as inputs)
~\cite{chung2020unearthing}.
Stability and predictability of job runtimes are important factors that affect the fundamental design and architecture of data processing pipelines.
Unfortunately, they are often neglected by operators due to the difficulties of assessment even though job slowdowns are inevitable~\cite{shao2019griffon}. 
Even with massive amounts of telemetry data, cloud providers still default to a manual triage process due to the difficulty of capturing the compounding factors that impact job runtime and its stability, which is not scalable and error-prone.
% ---

%there is a strong need to create an accurate quantitative estimate of the runtime variation beforehand such that they can be accounted for. 

%For the cloud operators, to offer Service-level-objectives (SLOs), it is important to better understand and measure the reliability of their services and identify the causes. 

%A comprehensive analysis for the reliability measurement and its reasoning opens up great potential to improve the service quality and identify existing issues in the cluster. 


% Prior work~\cite{schad:ec2-variance:vldb:2010} conducted an evaluation of Amazon EC2~\cite{ec2}'s performance in terms of runtime variation using standardized benchmark such as Ubench~\cite{ubench} and Iperf benchmark~\cite{iperf} on a 50-node cluster. However, they do not model or predict the variation of production jobs, which involves significant heterogeneity in job characteristics.

%Predicting and modeling the variation in production jobs is a contribution of our work and has not been examined by prior work like \cite{schad:ec2-variance:vldb:2010} which has focused on standardized benchmarks such as Ubench~\cite{ubench} and Iperf benchmark~\cite{iperf}.

% across different jobs that might have different behavior under the same computing cluster.
%Griffon~\cite{shao2019griffon} developed an interpretable random forest model to infer the slowdown of job execution time for a selected number of production workloads. 
%But their model cannot predict significant slowdowns that appear as outliers.
% However, the model cannot capture outliers with significant slowdowns, which is unpredictable. 
%For the same reason, time-series based approaches~\cite{naghshnejad2018adaptive,sonmez2009trace} are not applicable.
% \todo{Are there other related works? Morpheus? mention and identify gaps.}
%Despite these initial investigations, little work has been done to systematically examine runtime variation for production workloads in big data analytic systems. 

Although prior works\edit{~\cite{schad:ec2-variance:vldb:2010, feitelson1995job, zrigui2022improving} have empirically characterized runtime variation, they do not propose methods to predict the variation nor the likelihood of a new run being an outlier compared to the average or median runtimes.} Other works such as Griffon~\cite{shao2019griffon} used machine learning models to predict the minor slowdown in runtimes \edit{for a limited number of job templates. They are} unable to predict significant slowdowns that appear as outliers. As ML models are notoriously bad at handling outliers especially with a low existence, prior time-series based approaches~\cite{naghshnejad2018adaptive,sonmez2009trace} are not applicable. \edit{In this paper, we aim to address this gap for production data analytics systems by developing a novel and systematic approach for modeling, predicting, and explaining the job runtime variation, allowing for finer-grained differentiation in characteristics.}

%Popular scalar metrics such as the Coefficient of Variation (COV) are not sufficient to characterize runtime variation for production workloads. To users, knowing the {\it probability} that a job runtime may exceed an extreme value, or various quantitative properties of the distributions, such as quantiles, is also important. 
%We propose a novel scheme of clustering runtimes to recover distributions. This lets us estimate the probabilities of extreme values despite not being able to predict individual job runtimes directly (e.g., a regression model to predict runtime of each individual job). Instead, {\it we associate the job with the distribution of the cluster it belongs to and infer its runtime distribution, which provide much more comprehensive information on the reliability of the performance.} Combined with telemetry data on job characteristics and physical cluster conditions, these predictions help us identify sources of variation and develop targeted remedies to resolve them.

%In this paper, we conduct a comprehensive quantitative analysis of millions of recurring jobs on \cosmos to examine their runtime distributions. Our key contributions are: 
% i) descriptive: by examining historic data including intrinsic job properties, resource allocation, and cluster conditions, we provide a better understanding of the factors affecting runtime variation for each individual job; ii) predictive: we show how to use a machine learning models to predict, with at least 95\% accuracy, the distribution of runtimes for recurring jobs; and iii) prescriptive: based on the predictor, we can evaluate what-if scenarios, and identify potential opportunities to reduce the variation by limiting spare tokens, scheduling on newer generations of machines, and better load balancing across machines.
% The key contributions of our work are along the following three axes.
%inferring the reasoning of performance variation for recurring jobs, leveraging millions of job records in \cosmos, an internal big data analytics platform at \msft. A set of applications are supported:
%\begin{itemize}[leftmargin=*]
%	\item \textit{Descriptive} analysis: by examining historic data including (1) intrinsic job properties, (2) resource allocation, and (3) physical cluster conditions, we develop a better understanding of the factors affecting runtime variation for individual jobs. [Section~\ref{sec:explain}]
% 	We show that a naive approach of correlating prediction model features with the predicted variation is not sufficient to explain the predictions. Instead, we use game-theoretic Shapley values~\cite{shapley1953value} for explaining predictions and quantitatively analyze the contributions of different features to the predicted variation. 
	%The tool can be used to automatically identify the bottleneck and help with resolving performance concerns from customer, to replace the manual triage which is time-consuming and error-prone. 
%	\item \textit{Predictive} analysis: for a newly-submitted job, we develop a predictor for the runtime distribution that provides richer information to customers, such as the probability of outliers, quantiles, and shapes of the distribution. [Section~\ref{sec:model}]
	%we propose to use Bayesian Network (BN) compared with classic machine learning  models to predict the coefficient of variation of each job templates. The information can be provided to customers to build up the right level of expectation.
%	\item \textit{Prescriptive} analysis: based on the predictor, we evaluate what-if scenarios and identify potential opportunities to reduce variation by limiting spare tokens, scheduling on newer generations of machines, and better load balancing across machines. [Section~\ref{sec:prescriptive}]
	%improve the reliability of each job and propose customized remedy for both the jobs and the computing cluster. 
%\end{itemize}

% The key contributions of our work are along the following three axes.
% %inferring the reasoning of performance variation for recurring jobs, leveraging millions of job records in \cosmos, an internal big data analytics platform at \msft. A set of applications are supported:
For our study, we comprehensively examine the runtime variation for millions of production SCOPE~\cite{chaiken2008scope} jobs on Cosmos~\cite{power2021cosmos}, an exabyte-scale analytics platform at Microsoft that supports a broad spectrum of \msft products~\cite{power2021cosmos}. Our key contribution is a framework for systematically analyzing, predicting and explaining runtime variation that includes:
\begin{enumerate}[leftmargin=*]
 	\item \textit{Descriptive} analysis: by examining historic data including intrinsic job properties, resource allocation, and physical cluster conditions, we provide a better understanding of the factors affecting runtime variation for each individual job. In particular:
 	\begin{enumerate}[leftmargin=14pt]
 	    \item We show that popular scalar metrics, such as Coefficient of Variation (COV) considered by prior work~\cite{schad:ec2-variance:vldb:2010}, are not sufficient to characterize variation with the existence of outliers. Instead,  we propose a novel scheme of characterizing variation using properties of the distribution of normalized runtime of the jobs \edit{that provides fine-grained information %  	 predictor, with $> 96\%$ accuracy, for the runtime distribution for a new run of a recurring job that provides richer information, 
 	such as the probability of outliers, quantiles, and shapes of the distribution.} [Section~\ref{sec:metrics}]
 	    \item We make novel use of Shapley values~\cite{shapley1953value} for explaining predictions for variation and quantitatively analyze the contributions of different features. [Section~\ref{sec:explain}]
 	\end{enumerate}
 	%The tool can be used to automatically identify the bottleneck and help with resolving performance concerns from customer, to replace the manual triage which is time-consuming and error-prone. 
 %	\item As a \textit{predictive} analysis,  Various quantitative properties of the distributions, such as quantiles and probability of extreme values, can then be used as a measure of the variation for a newly-submitted job. [Section~\ref{sec:model}]
 	%we propose to use Bayesian Network (BN) compared with classic machine learning  models to predict the coefficient of variation of each job templates. The information can be provided to customers to build up the right level of expectation.
 	\item \textit{Predictive} analysis: we develop an innovative \edit{approach based on likelihood to identify distinctively-diverse runtime distributions, and predict the distribution with >96\% accuracy, out-performing previous methods~\cite{shao2019griffon}}. [Section~\ref{sec:model}]
 	\item \textit{Prescriptive} analysis: based on the predictor, we quantitatively analyze what-if scenarios and identify potential opportunities to reduce variation by limiting spare tokens, scheduling on newer generations of machines, and better load balancing. [Section~\ref{sec:prescriptive}]
 	%\item As a \textit{prescriptive} analysis, based on the predictor, we can evaluate what-if scenarios, and identify potential opportunities to reduce the variation by limiting spare tokens, scheduling on newer generations of machines, and better load balancing across machines. [Section~\ref{sec:prescriptive}]
 	%improve the reliability of each job and propose customized remedy for both the jobs and the computing cluster. 
\end{enumerate}

%To address the high correlation between variables, we use Bayesian Network to systematically learn the dependency and use domain knowledge to fine-tune the structure of the dependency graph. The learned network is then used to identify the different causes of runtime variation both at the aggregate level and at the individual job-template level and compared with classic machine learning algorithms, such as Explainable Boosting Machine (EBM). The method is generalizable to other similar causal inference problem and can be validated with out labeled data (to reveal the real reasoning of runtime variation).

%\todo{Highlight key new findings about (1) factors affecting variation, and (2) modeling methodology or novel application to this domain.}
%In sum, our contributions are the following:
%\yz{description of each section?}

The rest of this paper is organized as follows. Section~\ref{sec:challenges} discusses challenges in estimating and predicting runtime variation and our goals and approach in this work. Section~\ref{sec:bg} gives a brief overview of \scope jobs in \cosmos, potential sources of variation, and the datasets that we study. Sections~\ref{sec:metrics}--\ref{sec:prescriptive} present the descriptive, predictive and prescriptive analyses as outlined above. Section~\ref{sec:related} discusses related work in this space and Section~\ref{sec:conclusion} concludes the paper.

%\begin{figure}[!t]
%	\centering
%	\vspace{0.4cm}
%	\includegraphics[width=0.75\columnwidth]{trend3}
%	\vspace{-0.3cm}
%	\caption{\cosmos job size}\label{fig:trend}
%	\vspace{-0.5cm}
%\end{figure}



%The remainder of this paper is organized as follows. 
%Section~\ref{sec:background} describes the problem.
%Section~\ref{sec:overview} discusses the general architecture of Phoebe.
%Sections~\ref{sec:module1} describes in detail the cost models,
%Sections~\ref{sec:ttl} describes the method to estimate the time to live for each stage, and
%Sections~\ref{sec:opt} describes the optimization module.
%Sections~\ref{sec:result} presents the experiment results and the evaluation for temp data savings in production environment.
%Section~\ref{sec:related} discusses related work, and Section~\ref{sec:conclude} draws our conclusions.



==> Runtime Variation in Distributed Systems (Short II) (2)/Platform_and_Datasets.tex <==
\section{Platform and Datasets}
\label{sec:bg}

%\subsection{Background}
\cosmos~\cite{power2021cosmos} is an exabyte-scale big data platform developed at \msft since 2002, with more than 300k machines across multiple data centers worldwide~\cite{zhu2021kea}. Using a YARN-based~\cite{vavilapalli2013apache} resource manager, the system processes >600k jobs per day from tens of thousands of \msft internal users. It is a big internal shared-cluster where efficiency is paramount. Over the past decades, a multitude of research projects and engineering efforts have improved its efficiency, security, scalability and reliability~\cite{jindal2019peregrine, zhang2012optimizing, bruno2012recurring, bruno2013continuous,boutin2014apollo,boutin2015jetscope,karanasos2015mercury,jyothi2016morpheus,curino2019hydra,qiao2019hyper,chaiken2008scope,ferguson2012jockey,ramakrishnan2017azure,zhou2012advanced,zhu2021kea,zhou2010incorporating,wing2020osdi,phoebe,sen2021autoexecutor, zhu2021kea}. 
% As a result, \cosmos operates at consistently high utilization (>70\%) and low failure rates~\cite{zhu2021kea}. 

\cosmos jobs can be authored using a SQL-like dialect, named SCOPE~\cite{boutin2015jetscope} with heavy use of C\verb|#| and user-defined functions (UDFs). Upon submission, a job is compiled to an optimized execution plan as a DAG of operators, and distributed across different machines. 
Each job consists of multiple \textit{Vertices}, i.e., an individual process that will be executed on a container assigned to one physical machine.

% \yz{mention vertex}
\subsection{Job Groups}
Our work focuses on understanding and predicting variation in runtimes over repeated runs of jobs that we assemble into \textit{job groups}. Variation is meaningful only when jobs recur (i.e., sample size $>$ 1). Prior studies~\cite{jyothi2016morpheus,wing2020osdi,phoebe} have shown that 40--60\% of jobs on Cosmos are recurring jobs. Others~\cite{feitelson1995job} have also reported a significant fraction of jobs as recurring on their systems. 
We identify recurrences by matching on a key that combines the following.
\begin{itemize}[leftmargin=*]
    \item The normalized job name, which has specific information like submission time and input dataset removed~\cite{phoebe,jindal2019peregrine}. 
    \item The job signature~\cite{jindal2019peregrine}, which is a hash value computed recursively over the DAG of operators in the compiled plan. The signature does not include job input parameters.
\end{itemize}
We thus have \textit{job groups} with \textit{job instances} belonging to each group, corresponding to recurrences of the job. Job instances have the same key value within each job group.

\subsection{Sources of Variation}
\label{subsec:sources-of-variation}

Within each job group, runtimes of job instances can vary due to any of the following reasons:

\smallsection{Intrinsic \edit{characteristics}} The key used for grouping jobs includes information on the execution plan (e.g., type of operators, estimated cardinality, dependency between operators) while not including the job input parameters (e.g., parameters for filter predicates) or input datasets. Different instances can have different values for these parameters, datasets, and their sizes. This can lead to different runtimes within the group if the parameter changes are not accompanied by a change in the compiled plan. In our datasets, we have observed that input data sizes can vary by up to a factor of 50 within the same job group.
\begin{figure}
	\centering
		\includegraphics[width=0.65\columnwidth]{img/tokenusage.pdf}
	\vspace{-0.3cm}
	\caption{\edit{Token usage for an example job during its run.}
		\vspace{-0.4cm}
	}\label{fig:token}
\end{figure}

\smallsection{Resource \edit{allocation}} 
In \cosmos, the unit of resource allocation is a \textit{token}~\cite{power2021cosmos}, which is analogous to the notion of a container. 
The number of tokens guaranteed for a job can be specified by users at the time of job submission or it may be recommended by the system~\cite{autotoken}. To further improve the utilization of the existing infrastructure, unused resources are repurposed as preemptive spare tokens~\cite{boutin2014apollo} that can be leveraged by any jobs freely\footnote{The usage of spare tokens is capped by the allocation as specified by users.}. The availability of these spare tokens is difficult to predict, and can have meaningful effects on runtimes. Figure~\ref{fig:token} shows the skyline of token usage for a \cosmos job that was allocated with 66 tokens (dashed line). Including spare tokens, the job consumed up to 198 tokens in total throughout its processing time. 

The maximum number of tokens used by a job depends on how much parallelism it can exploit subject to the number of tokens allocated. While observing the execution of various workloads on \cosmos, we have seen maximum token counts vary by a factor of 10 within the same job group.
%
%To better manage the capacity of such enormous infrastructure, the concept of ``\textit{tokens}'' was introduced to control the amount of resources, measured by the number of containers, that can be allocated to a particular job~\cite{power2021cosmos}. 
%The allocated tokens can be specified by customers to limit the maximum number of resource that can be used simultaneously. 
%
%While the number of tokens indicate the amount of resources used, 
There is also variation in the characteristics of allocated resources. Tokens map to computational resources on compute nodes with different Stock Keeping Units (SKUs). Having evolved for over a decade, the \cosmos cluster consists of 10--20 different SKUs with different processing speeds~\cite{zhu2021kea}. In our datasets, we have observed different job instances within the same job group run on one to nine different SKUs simultaneously.
%some of the newer generation of machines have faster processing speed~\cite{zhu2021kea} 
% \begin{figure}
% 	\centering
% 	\centering
% 	\includegraphics[width=.6\columnwidth]{img/cpu.pdf}
% 	\vspace{-0.4cm}
% 	\caption{CPU utilization by SKU.
% 			\vspace{-0.4cm}
% 	}\label{fig:cpu}
% \end{figure}

\smallsection{Physical cluster environment} Finally, physical cluster environment also leads to variations in runtimes. This includes both the availability of spare tokens (discussed above) and the load on the individual machines. 
% Figure~\ref{fig:cpu} shows significant differences in CPU utilization of machines with different SKUs in one of the \cosmos clusters. For example, 
% utilization for Gen6 varies from 2\% to 33\% with an average of 17\% whereas for Gen3.5 it varies from 10\% to 100\% with an average of 68\%.
Higher utilization (load) is likely to cause more contention for shared resources, and a larger range of loads may increase runtime variation.

\subsection{Datasets}

To develop insights into the sources of variation as discussed above, we collected data by:
% along those dimensions from production workloads on our clusters. 
i) extracting information about intrinsic characteristics such as operator counts in the plan, input data sizes, and cardinalities, costs, etc., estimated by the SCOPE optimizer using the Peregrine framework~\cite{jindal2019peregrine}; ii) obtaining token usage information from the job execution logs, and SKU and machine load information using the KEA framework~\cite{zhu2021kea}; and
iii) joining all this information together by matching on the job ID, name of the machine that executes each vertex, and the corresponding vertex start/end time.

\begin{table}[ht]
\centering
\vspace{-0.2cm}
\caption{Datasets used for this study. 
% \textit{Support} denotes the minimum number of job instances per group. We include groups after filtering for this criterion.
}\vspace{-0.26cm}
% \label{tab:datasets}
% \resizebox{0.9\columnwidth}{!}{\begin{tabular}{|c|c|c|c|c|}\hline
%      \textbf{Dataset}&  \textbf{Interval}& \textbf{Job Groups}& \textbf{Job Instances}& \textbf{Support}\\\hline\hline
%      \textbf{D1}& 6 months& 9.5K& 3.2M& 20\\\hline
%      \textbf{D2}& 15 days& 11.9K& 737K& 3\\\hline
%      \textbf{D3}& 5 days& 11.6K& 215K& 3\\\hline
% \end{tabular}}
% \end{table}
\label{tab:datasets}
\resizebox{0.6\columnwidth}{!}{\begin{tabular}{|c|c|c|c|c|}\hline
     \textbf{Dataset}&  \textbf{Interval}& \textbf{Job Groups}& \textbf{Job Instances}& \textbf{Support}\\\hline\hline
     \textbf{D1}& 6 months& >9K& >3M& 20\\\hline
     \textbf{D2}& 15 days& >11K& >700K& 3\\\hline
     \textbf{D3}& 5 days& >11K& >200K& 3\\\hline
\end{tabular}}
% \vspace{-0.3cm}
\end{table}

Table~\ref{tab:datasets} summarizes the datasets that we use for our study. The datasets consist of a subset of jobs run over the corresponding interval, and are included if the number of instances per group (support) exceeds a minimum threshold. With a support of minimum 3 occurrences, 53\% of jobs are included. 
In this research, we only focus on batch jobs as opposed to streaming jobs or interactive jobs that \cosmos also supports. 
We use dataset D1 to identify and group distributions of runtimes (see Section~\ref{sec:clustering}) for jobs with a large number of occurrences (>20).
% , and only job runtime information is needed. 
We used D2 to train a predictor for runtime variation and D3 to test its accuracy (Section~\ref{sec:model}).

%In this analysis, we set-off to gather data at the job-template level, which indicates a series of recurrent jobs processing different input data sources. To evaluate the reasoning of the variances, we combine a multitude of data sources, including (1) a set of environmental variables (including the utilization of each computing machine) that reflects the system status of the execution environment, (2) job characteristics (such as information for the execution plan) to indentify the type of jobs can potentially have higher runtime variation, and (3) resource usage for a particular job as the input to the estimators to predict the coefficient of variance of the job runtime. 




==> Runtime Variation in Distributed Systems (Short II) (2)/Predict.tex <==
\section{Predicting Runtime Variation}
\label{sec:model}

% To provide runtime distribution for a newly-submitted job, a prediction model is required, leveraging information that is known at compile time. In this section, we use explainable machine learning to better characterize the jobs that have different runtime distribution shapes. Specifically, we develop a classification model to predict what type of shape (see Figure~\ref{fig:clustering}) a distribution of a job group might have, i.e., cluster membership/cluster prediction.
% % , and (2) as a comparison, use a regression model to predict the runtime distribution directly, which leverages the job runtime observations for job instances sharing similar characteristics.
% In this section, we used dataset D2 as the training set, and D3 as the testing set.

We now develop a prediction model based on explainable ML to 
%better characterize jobs and 
predict the \textit{shape} of runtime distribution (as in Figure~\ref{fig:clustering}) of jobs. We use dataset D2 as training set and D3 as testing set.

\subsection{Feature Selection}\label{sec:input}

We consider three classes of predictive features that are available at the job compile time: those derived from the job execution plan ("intrinsic"), those representing statistics of the job's past resource use, and features describing the load in the physical cluster where the job will run. We describe the classes below.
% and in Table~\ref{table:featurelist}.

\smallsection{Intrinsic characteristics}
We leverage information on the job execution plan obtained from the query optimizer~\cite{jindal2019peregrine} at compile time as input, which can be indicative of the query type, data schema and its potential computation complexity. It includes the number of operators in each type (e.g., Extract, Filter), estimated cardinality, etc.. 
For a newly submitted job, its detailed input data size is unknown, and the estimated cardinality can be quite off~\cite{phoebe}. Therefore, using historic job instances of the same job group, we extract statistics for the total data read, temp data read, as well as the statistics related to the execution plan as additional input features that can be informative for the size of the job. 

We also derive the fraction of vertices running on each SKU as the input features, which indicates the resource consumption by each SKU. A previous study~\cite{zhu2021kea} shows that, in \cosmos, some newer SKUs might process data faster than the others; therefore, we believe that the \edit{fractions} of vertices executed on different SKUs would impact the runtime distribution. 
% We use the 10 vertex fraction features together with the total counts in the model.
% We have 69 features in total in this group.
% Discuss input variables related to execution graph, data size, etc.

\smallsection{Resource allocation}
\edit{The token allocation is a good indicator for the resources being utilized by a particular job thus impacting the runtime. However, \cite{autotoken} detects that users are often over-allocating (e.g., user selects to allocate 1000 tokens, but the peak actual usage is only 600). In this work, we integrated historic token utilization with token allocation as the input. For historic job instances of the same job group, we extract the resource utilization (min, max, and average token usage based on the skyline as in Figure~\ref{fig:token}) and use the historic statistics as features (historic average and standard deviation). We also created a new variable for spare tokens (historic average). The model learned to place less importance on token allocation as a feature compared to actual utilization, and we corroborate this from the Shapley scores in Section~\ref{sec:exp}.}

% We have 7 features in this group.

\smallsection{Physical cluster environment}
The job runtime can be affected by the utilization of the machines that execute its vertices---a higher utilization level indicates a hotter machine that is likely to have more severe issues related to noisy neighbors and resource contention. Therefore, we extract the CPU utilization level of the corresponding machines in each SKU at the job submission time as the input. \edit{Compared to existing methods, such as~\cite{shao2019griffon} and~\cite{zrigui2022improving}, incorporating new-real-time machine status information improves the model accuracy (see Section~\ref{sec:model}).}

\edit{Work is ongoing to record the per container usage for both CPU and memory that includes more targeted information on the particular job and captures more accurately the resource consumption compared to the machine-level counters~\cite{cpuwrong}. Once available, features can easily be replaced or added to our models. We expect them to be strong indicators for the job runtime as they capture more job-level charateristics. They might also reveal if a job that is CPU intensive or memory intensive is more likely to have large runtime variances.}
% We have 22 features in this group.

% Table~\ref{table:featurelist} shows examples of features used in the model, where ``H" represents features derived using historic data, including historic average (with a suffix of ``Avg'') or standard deviation (with a suffix of ``Std''), and ``N'' represents features of the new job. We can see that only the features that can be obtained from the query optimizer are from the new jobs, and the other features are calculated based on historic observations as such information is unknown at the compile time when we need to make the prediction. Note that some of the features listed in Table~\ref{table:featurelist} might not be used directly in the prediction model as the feature selection step might remove some of the less indicative factors that will not impact the runtime variation.
    

% \begin{table}[]
% 	\caption{Feature Examples.}\label{table:featurelist}
% 		\vspace{-0.2cm}
% \begin{adjustbox}{max width=\columnwidth}
% \begin{tabular}{p{2cm}llp{3.6cm}}
% \toprule
% Category                  & Name                                       & H/N & Description                                                                                                  \\\midrule
% Intrinsic characteristics (Total: 69) & Temp/TotalDataReadAvg                      & H   & Temporary/total data read of each job                                                                        \\
%                           & Est/InputCardinality(Avg/Std)                       & N/H   & Estimated (input) cardinality                                                                                \\
%                           & GenXVertexCount/FracAvg                    & H   & Average number/fraction of vertices executed on GenX               \\
%                           & VertexCountTotal(Std)                      & H   & Total number of vertices (average/standard deviation)                                                                \\
%                           & HistClusterX                          & H   & Log-likelihood of belonging to ClusterX (e.g., Cluster6) using historic observations                     \\
%                           & Est(Exclusive)Cost(Std/Avg)                & N/H & Estimated (Exclusive) cost (standard deviation/average over historic observations)                       \\
%                           & PhyOp\textless{}OperatorName\textgreater{}Count & N   & Number of operators in the execution plan with \textless{}OperatorName\textgreater{}, such as ``Filter''     \\
%                           & AvgRowLength(Std/Avg)                               & N/H & Average row length from query optimizer                                                                      \\
%                           & CountHistOccurences                        & H   & Number of historic job observations so far                                                                   \\\midrule
% Resource allocation (Total: 7)      & Max/min/avgTokensStd/Avg                       & H   & Max/min/average token usage, average/standard deviation over historic observations                                              \\
%                           & VirtualClusterAllocationStd                & H   & Token allocation specified by users upon submission, standard deviation                                      \\
%                           & SpareTokensStd/Avg                             & H   & Usage of spare tokens                                                                                        \\\midrule
% Cluster condition (Total: 22)        & avgGenXCPUStd/Avg                          & H   & CPU utilization statistics (average or standard deviation) of GenX (e.g., Gen3.1) machines for historic jobs \\
%                           & CPUUtlizationAll(Avg/Std)                           & N/H   & CPU utilization statistics (average or standard deviation) for all machines  \\\bottomrule
% \end{tabular}
% \end{adjustbox}
% \vspace{-10pt}
% \end{table}

% \yz{a little bit too long to move to challenges... keep the same place, difficult to select features, which is large, second, missing features}
%  to start with is to examine the correlation between the different job characteristics. 

\subsection{Cluster membership prediction}\label{sec:exp}
% While the clustering analysis (see Section~\ref{sec:clustering}) was conducted using historic observations of a large number of job instances, 
For a new job to be submitted, we want to \textit{predict} its runtime distribution shape based on information that is available at compile time. This naturally maps to a classification problem, where the prediction target is to map each job to a particular distribution shape (e.g., one among the 8 different shapes as in Figure~\ref{fig:clustering}).
% , \textit{Cluster 0} as one of the possible labels). 

% For each job group, we have a multitude of job instances, and the histogram of runtime observations is a reliable estimator of the job's empirical runtime PMF as shown in Figure~\ref{fig:clustering}.

\smallsection{Cluster membership based on posterior likelihood}
%We conduct clustering analysis using a long period of observations and cluster similar distributions as a group (i.e., clusters). For a new job, based on its historic runtime distribution, we determine which cluster it belongs to and more specifically, the posterior distribution of the mixture weights for this particular job.
For each job instance, to determine which distribution shape it has, we leverage the set of similar job instances in the analyzed period with the same job group (i.e., same job name and execution plan) to derive the group's empirical Probability Mass Function (PMF), i.e., the histogram of the runtime distribution. 
% Specifically, we compute the likelihood of this job group belonging to each of the clusters as in Section~\ref{sec:clustering} by comparing the EPMF of this job group and the ones for the existing clusters.
Based on even a small number of runtime observations, we derive the posterior likelihood of these observations to be drawn from any one of the pre-defined distribution shapes as in Figure~\ref{fig:clustering}. 
% Intuitively, if for those observations, their variance is very large, they are more likely to be drawn from the distribution of Cluster 7 (which has a larger variance).

Based on Bayes' Theorem~\cite{bishop2006pattern}, the \textit{posterior log-likelihood} that a job group with $N$ runtime observations, $x_{n=1 \cdots N}$, belongs to a cluster $z_{i=1 \cdots K}$ can be derived based on the PMF of these $N$ observations, $\phi_{h = 1 \cdots H}$, and the PMFs of the $K=8$ pre-defined clusters, $\theta^{i = 1 \cdots K}_{h = 1 \cdots H}$, which is adaptive to larger sample size:\vspace{-5pt} 

{\small
\begin{align}
p(x_1, x_2 \cdots x_N|z_i) &= \prod_{n=1 \cdots N} F(x_n|\theta^{i}_{h = 1 \cdots H}) \\
&= \prod_{n=1 \cdots N} \theta^{i}_{h(x_n)}\\
\log p(x_1, x_2 \cdots x_N|z_i) &= \sum_{n=1 \cdots N} \log (\theta^{i}_{h(x_n)})\\
p(z_i|x_1, x_2 \cdots x_N) &= \frac{ p(x_1, x_2 \cdots x_N|z_i)p(z_i)}{\sum_{i=1 \cdots K}p(x_1, x_2 \cdots x_N|z_i)p(z_i)} \\
&= \frac{ \prod_{n=1 \cdots N} \theta^{i}_{h(x_n)}}{\sum_{i=1 \cdots K}\prod_{n=1 \cdots N} \theta^{i}_{h(x_n)}}\\
&\sim \prod_{n=1 \cdots N} \theta^{i}_{h(x_n)}\\
%\end{align}
%\begin{align}
\log p(z_i|x_1, x_2 \cdots x_N) &= \sum_{n=1 \cdots N} \log \left(\theta^{i}_{h(x_n)}\right) - \text{constant}\\
&= \sum_{h=1 \cdots H} n_h \log \left(\theta^{i}_{h}\right)- \text{constant}\\
%&= N \sum_{h=1 \cdots H} \frac{n_h}{N}  \log \left(\theta^{i}_{h}\right)- \text{constant}\\
%&=N \sum_{h=1 \cdots H} \phi_h  \log \left(\theta^{i}_{h}\right) - \text{constant}\\
&\sim \sum_{h=1 \cdots H} \phi_h  \log \left(\theta^{i}_{h}\right)\label{eq:loglikelihood}
\vspace{-60pt}
\end{align}
}Where,


\begin{tabular}[h]{lp{11.7cm}}
% 	$K$:& number of mixture clusters from the clustering analysis, e.g., K=8 clusters of distributions.\\
% 	$N$:& number of runtime observations for a particular job group. 	\\
	$H$:& number of discrete bins when we derive the PMF for each distribution, a constant across all distributions.	\\
	$\theta^{i = 1 \cdots K}_{h = 1 \cdots H}$:& parameter of normalized runtime distribution for cluster $i$, specifically, the PMF value for bin $h$.\\
	$\phi_{h = 1 \cdots H}$:& parameter of distribution based on observations for a particular job group (i.e., $x_{n=1,2 \cdots N}$), specifically, the probability for bin $h$ of the PMF.\\
	$h(x_n)$:& the bin index that observation $x_n$ belongs to.\\
	$n_{h}$:& number of observations of runtime (i.e., $x_{i=1 \cdots N}$) for the job group that belongs to bin $h$.\\
% 	$z_{i=1 \cdots K}$:& cluster labels.\\
	$x_{n=1 \cdots N}$:& runtime observation $n$, where
	$x_{n=1 \cdots N}|z_{i=1 \cdots K} \sim F(\theta^{i = 1 \cdots K}_{h = 1 \cdots H})$.\\
%\end{tabular}
%
%\begin{tabular}[h]{lp{6.5cm}}	
	$p(z_i)$:& prior on the probability of each cluster, assuming to be a constant across all clusters (non-informative prior~\cite{bishop2006pattern}).\\
\end{tabular}

% Based on Equation~\ref{eq:loglikelihood}, 
It is interesting to point out that the log-posterior-likelihood is proportional to the dot product of the PMF of observations for the particular job group, i.e. $\phi_{h}$,  and the one of the pre-defined 8 clusters (after taking the log), i.e., $\theta^{i}_{h}$ (see Equation~\ref{eq:loglikelihood}).

 
% Moreover, the same likelihood estimation process can be applied to using only historic occurrences (might have very limited number of observations, i.e., $N$, but is known at the time of making predictions) and the likelihood can be used as features. 
Figure~\ref{fig:ll} shows an example of normalized runtime distribution (by \deltanorm) for a job with 10 occurrences compared with 2 clusters. The dashed line is the PMF for observations for this job group, i.e. $\phi_{h}$, and the solid line is for the predefined clusters, $\theta^{i}_{h}$. We see that Cluster 5, with the highest log-likelihood of -422.9, has the most similar shape \edit{(see Figure~\ref{fig:ll1}), while Cluster 0 has the least similar shape (see Figure~\ref{fig:ll2}).} Each job instance together with its job group is then associated with a cluster label with the highest likelihood as the prediction target (label).
\edit{This cluster association algorithm will always place a job in the most likely cluster. We observed that jobs with fewer observations may not be similar to any existing cluster’s runtime distribution. Therefore, we focus only on job groups with sufficient samples. We employ the inertia curve to tune the number of clusters as proposed in Section~\ref{sec:clustering} to avoid overfitting.
% , but we can increase the number of clusters to fit corner cases.
}
% , e.g., \textit{Cluster 5} for the job indicated in Figure~\ref{fig:ll}.

% \begin{figure}
% 	\centering
% 	\begin{minipage}[b]{.45\columnwidth}
% 		\includegraphics[width=\textwidth]{img/test_likelihood/ll_Activity.ARR.ArrDeviceIdMerge_top_0_cluster_4_idx.pdf}
% 	\end{minipage}%
% % 	\begin{minipage}[b]{.45\columnwidth}
% % 		\includegraphics[width=\textwidth]{img/test_likelihood/ll_Activity.ARR.ArrDeviceIdMerge_top_1_cluster_1_idx.pdf}
% % 	\end{minipage}%

% % 	\begin{minipage}[b]{.45\columnwidth}
% % 		\includegraphics[width=\textwidth]{img/test_likelihood/ll_Activity.ARR.ArrDeviceIdMerge_top_6_cluster_5_idx.pdf}
% % 	\end{minipage}\hfill%
% 	\begin{minipage}[b]{.45\columnwidth}
% 		\includegraphics[width=\textwidth]{img/test_likelihood/ll_Activity.ARR.ArrDeviceIdMerge_top_7_cluster_0_idx.pdf}
% 	\end{minipage}%
% 		\vspace{-3mm}
% 	\caption{Examples of likelihood values (higher values indicate more probable).}\label{fig:ll}
% 	\vspace{-10pt}
% \end{figure} 

\begin{figure}
	\centering
	\subfloat[\edit{Most likely cluster\label{fig:ll1}}]{			\includegraphics[width=.31\columnwidth]{img/test_likelihood/ll_Activity.ARR.ArrDeviceIdMerge_top_0_cluster_4_idx.pdf}\vspace{-8pt}}\quad\quad
	 \subfloat[\edit{Least likely cluster\label{fig:ll2}}]{			\includegraphics[width=.31\columnwidth]{img/test_likelihood/ll_Activity.ARR.ArrDeviceIdMerge_top_7_cluster_0_idx.pdf}\vspace{-8pt}}
	 \vspace{-8pt}
	\caption{\edit{Examples of likelihood values (higher values indicate more probable).}}\label{fig:ll}
	\vspace{-0.5cm}
\end{figure} 

% \begin{figure}
% 	\centering
% 	\begin{minipage}[b]{.48\columnwidth}
% 		\includegraphics[width=\textwidth]{img/test_likelihood/ll_Activity.ARR.ArrDeviceIdMerge_top_0_cluster_4_idx.pdf}
% 	\end{minipage}
% 	\begin{minipage}[b]{.48\columnwidth}
% 		\includegraphics[width=\textwidth]{img/test_likelihood/ll_Activity.ARR.ArrDeviceIdMerge_top_7_cluster_0_idx.pdf}
% 	\end{minipage}%
% 	\vspace{-0.5cm}
% 	\caption{\edit{Examples of likelihood values (higher values indicate more probable).}}\label{fig:ll}
% 	\vspace{-0.5cm}
% \end{figure} 
\smallsection{Classification model}
Based on the inputs, we conduct (1) passive-aggressive feature selection~\cite{zheng2015online} based on feature importance to avoid the use of correlated features, (2) parameter sweeping to select the best hyper-parameters for the classification algorithm, such as the number of trees for tree-based algorithms, and (3) fitting using \edit{RandomForestClassifier~\cite{rf}, LightGBMClassifier~\cite{lgbm} and EnsembledClassifier~\cite{es} by combining a set of popular classification algorithms, such as RandomForestClassifier, LightGBMClassifier, GradientBoostingClassifier~\cite{gb}, GaussianNB~\cite{gn}, and XGBClassifier~\cite{xgb}, using soft voting.} Note that RandomForestClassifier and LightGBMClassifier are well-known to have high accuracy for ML tasks using tabular data\edit{, especially for out-of-sample tests}. \edit{In this work, among the classifiers,} LightGBMClassifier has the highest accuracy\edit{, thus we report its result for the rest of the paper. By analyzing the prediction results, we noticed:}


% \begin{figure}
% 	\centering
%     \subfloat[\rationorm]{		\includegraphics[width=\columnwidth]{img/hist_normed_kmeans_8_bins_merge_tail_ratio0210_min_3/importance_lgbm_f.pdf}\vspace{-8pt}}
    
%     \subfloat[\deltanorm]{			\includegraphics[width=\columnwidth]{img/hist_normed_kmeans_8_bins_merge_tail_delta0210_min_3/importance_lgbm_f.pdf}\vspace{-8pt}}
% 	 	\vspace{-3mm}
% 	\caption{Feature importance.}\label{fig:fimportance}
% 	\vspace{-10pt}
% \end{figure} 
% To better understand which feature impacts the prediction the most (possibly affects the variation as well), Figure~\ref{fig:fimportance} shows the Gini importance~\cite{louppe2013understanding}, which is one of the easiest ways to rank the features, for LightGBMClassifier based on \bothnorm respectively. 
% We see that the features related to the computation complexity and input data sizes (such as VertexCountTotal, i.e., vtctotal, and DataRead) are significant. 

By examining the Gini importance~\cite{louppe2013understanding} of the input features, we found that features related to the computation complexity and input data sizes (such as count of vertices, and data read) are significant and the features related to the historic runtime observations are also significant.
% (such as HistClusterX indicating the cluster likelihood derived using historic observations). 
The token utilization (such as the max), and compile time information (such as cardinality estimates) are also important. The CPU utilization of machines
% (such as Gen3.5CPUAvg) 
also impacts the prediction, which coincides with our belief that the physical cluster environment will affect the runtime variation of jobs. 
\edit{We also noticed that many of the operators turned out to be less important. The total vertex count is less important than the data size (total data read or cardinality-related metrics). It is possibly due to the huge variation in data processed by each vertex.}
In Section~\ref{sec:explain}, we dive into more details on the contribution of some features.
\begin{figure}
	\centering
    \subfloat[Confusion matrix\label{fig:cm}]{			\includegraphics[width=.43\columnwidth]{img/hist_normed_kmeans_8_bins_merge_tail_ratio0210_min_3/cm_lgbm_new_idx.pdf}\vspace{-8pt}}
        \subfloat[Accuracy by occurrences\label{fig:accuracy}]{			\includegraphics[width=.42\columnwidth]{img/hist_normed_kmeans_8_bins_merge_tail_ratio0210_min_3/accuracy_by_count_lgbm.pdf}\vspace{-8pt}}
    \vspace{-3mm}
	\caption{\edit{Prediction accuracy for \rationorm.}}\label{fig:cm2}
	\vspace{-10pt}
\end{figure} 
\begin{center}
\shadowbox{
\begin{minipage}{0.9\linewidth}
    \textbf{Insight:} \edit{The feature importance learned from the model is mostly consistent with our expectation.}
\end{minipage}
}\vspace{-3pt}
\end{center}


% \begin{figure}
% 	\centering
%     \subfloat[\rationorm]{			\includegraphics[width=.5\columnwidth]{img/hist_normed_kmeans_8_bins_merge_tail_ratio0210_min_3/cm_lgbm_new_idx.pdf}\vspace{-8pt}}
%     \subfloat[\deltanorm]{			\includegraphics[width=.5\columnwidth]{img/hist_normed_kmeans_8_bins_merge_tail_delta0210_min_3/cm_lgbm_new_idx.pdf}\vspace{-8pt}}
%     \vspace{-3mm}
% 	\caption{Confusion matrix of Predicted vs Actual clusters.}\label{fig:cm}
% 	\vspace{-10pt}
% \end{figure} 

Figure~\ref{fig:cm} shows the confusion matrix on test data comparing the predicted label (the x-axis) and the actual label (the y-axis) where each cell shows the portion of jobs of each category.
% (e.g., the top-left cell indicates the portion of jobs with a predicted label of Cluster 0 and actual label of Cluster 0). 
Predictions using both \bothnorm achieve overall accuracy of >96\%.
Figure~\ref{fig:accuracy} (orange line) shows the accuracy for jobs with different numbers of historic occurrences. We can see that for jobs with more historic occurrences, the prediction accuracy is higher, which indicates that the model prediction can be further refined by adding more observations from the same job group. The blue bar shows the count of job groups based on the number of job occurrences (1-5, 6-10, etc.). We can see that most of the jobs have 16-50 historic observations over the analyzed period. 
% Later analysis shows that without the set of features of historic cluster, the prediction accuracy is not significantly degraded, which dramatically reduces the computation complexity of feature construction and indicates the informativeness of other features for this prediction problem (by not only relying on the historic observation statistics). 
Similar trend can be seen for \deltanorm.
\begin{center}
\shadowbox{
\begin{minipage}{0.9\linewidth}
    \textbf{Insight:} \edit{Model predictions using both \bothnorm achieve high accuracy.}
\end{minipage}
}\vspace{-3pt}
\end{center}


% \subsubsection*{Predictions using both \bothnorm achieve overall accuracy of >96\%.}
% \edit{\textit{The proposed method outperforms existing model in predicting outliers.}}
\edit{We extended the traditional random forest regression model as proposed in~\cite{shao2019griffon} by adding more query optimizer and near-real-time machine status information as features to predict the job runtime as the label}. Figure~\ref{fig:compare} compares the predicted distribution for all job runtimes based on the proposed method (using classification model to predict the distribution shape) and the regression model against the actual job runtime distribution using Quantile-Quantile Plot~\cite{gnanadesikan1968probability}, plotting the mean absolute error (MAE) in the y-axis. If two distributions are identical, the plotted quantile should align and the MAE=0. We can see that the proposed classification model (Figure~\ref{fig:compare_class}) has better accuracy compared with the traditional regression model (Figure~\ref{fig:compare_regre}) especially for higher percentiles as it captures better the existence of outliers in the distributions of clusters of jobs (see Figure~\ref{fig:clustering}). The Kolmogorov–Smirnov distance~\cite{karson1968handbook} is also reduced by 9.2\%, indicating better accuracy. 
\begin{figure}
	\centering
    \subfloat[Regression\label{fig:compare_regre}]{
    \includegraphics[width=.42\columnwidth]{img/compare_regre2.pdf}\vspace{-8pt}}
    \subfloat[Proposed approach\label{fig:compare_class}]{			
    \includegraphics[width=.42\columnwidth]{img/compare_class2.pdf}\vspace{-8pt}}
    \vspace{-2mm}
	\caption{Prediction accuracy for \deltanorm compared with traditional regression model.\label{fig:compare}}
	\vspace{-10pt}
\end{figure}
\begin{center}
\shadowbox{
\begin{minipage}{0.9\linewidth}
    \textbf{Insight:} \edit{The proposed method outperforms existing model in predicting outliers.}
\end{minipage}
}\vspace{-3pt}
\end{center}
% \begin{figure}
% 	\centering
%     \subfloat[\rationorm]{			\includegraphics[width=.5\columnwidth]{img/hist_normed_kmeans_8_bins_merge_tail_ratio0210_min_3/accuracy_by_count_lgbm.pdf}\vspace{-8pt}}
%     \subfloat[\deltanorm]{			\includegraphics[width=.5\columnwidth]{img/hist_normed_kmeans_8_bins_merge_tail_delta0210_min_3/accuracy_by_count_lgbm.pdf}\vspace{-8pt}}
% 		\vspace{-3mm}
% 	\caption{Accuracy by historic occurrence count.}\label{fig:accuracy}
% 	\vspace{-10pt}
% \end{figure} 


% \todo{discuss shortcomings}

% Even though the 8 predefined clusters provide good insight into the distributions for different jobs, there might be still a small fraction of job groups whose runtime distribution shapes might not fall in any of the clusters. This is difficult to capture with the current model. A future direction may be to have more flexible distribution shapes that can be defined with tunable and continuous parameters, such as mean, variance, etc. to allow for more customized distribution shapes. However, the high accuracy of our clustering predictions provides a solid foundation for the analysis in the following section, where we quantitatively attribute runtime variation to each feature. 
% Moreover, for jobs with small number of observations, their derived runtime distribution might be biased, which might potentially result in larger prediction error as can be seen in Figure~\ref{fig:accuracy}.





















==> Runtime Variation in Distributed Systems (Short II) (2)/Predict2.tex <==

\subsection{Classic ML Predictor}

RF, EBM(?) 

\todo{show prediction accuracy}

\todo{show feature importance scores and discuss shortcomings}



%\subsection{Bayesian Network}
%
%\todo{compare with RF prediction}
%


==> Runtime Variation in Distributed Systems (Short II) (2)/RelatedWork.tex <==
\section{Related Work}
\label{sec:related}

%Prior work has focused on analyzing system failures, predicting job runtimes, and potential anomalies using machine learning methods for Big Data analytics systems~\cite{bhaduri2011detecting,chitrakar2012anomaly,duan2009fa}. 

%Pietri et al.~\cite{pietri2014performance} developed a performance model to estimate execution time of scientific workflows on the cloud with respect to different amounts of resource allocation. 
%Similarly, \cite{autotoken} estimated the job runtime based on different token allocations in \cosmos. 
A number of works have studied the problem of predicting job runtimes under different resource allocations and platform parameter settings~\edit{\cite{pietri2014performance, tasq-arxiv, tasq-edbt, hu:reloca:infocom:2020, autodop, starfish:analytics-cluster-sizing:socc:2011, starfish:analytics-cluster-sizing:socc:2011, rajan2016perforator, guo2018machine}}.
Morpheus~\cite{jyothi2016morpheus} examines resource usages of recurring jobs and finds the best-fitting pattern that it uses for better resource allocation and scheduling, but does not predict the outlier probability for a given job. \edit{Runtime estimation has also been used to infer job scheduling to support policies, such as Shortest Processing time First (SPF)~\cite{tsafrir2007backfilling, gaussier2015improving, kuchnik2019ml, zotkin1999job}. Zrigui et al.~\cite{zrigui2022improving} clustered job instances into small and large based on runtime and used a classification algorithm to inform their job scheduler with high accuracy. 
In our work, we derived a larger number of clusters for delta- and ratio-normalized runtime distributions with richer information (percentiles, variances, etc.), providing a comprehensive oversight of customer experiences. 
% However, they do not predict the runtime variation, which is an important aspect of the customer experience. 
}

Schad et al.~\cite{schad:ec2-variance:vldb:2010} studied performance variation on Amazon EC2~\cite{ec2} by running benchmarks for CPU and Memory performance, Disk I/O, and network bandwidth. 
Feitelson et al.~\cite{feitelson1995job} examined 
%the job characteristics of a production 
a parallel scientific workload on a 128-node cluster at NASA Ames and presented the changes of 
%the environment factors such as 
job submission rate, system utilization, and the distributions of job characteristics such as job type, runtime, and degree of parallelism. 
However, they do not model or predict the job runtime variation.

Prior works have proposed automated methods, including ML techniques, for analyzing system failures, slowdowns, and potential anomalies~\cite{bhaduri2011detecting,chitrakar2012anomaly,duan2009fa, shao2019griffon}. 
%ML models can also be used for anomaly reasoning. 
%Griffon~\cite{shao2019griffon} explored  inferring the possible causes of job slowdowns at the job group level using a regression model to predict runtime of each job instance for a selection of job groups with SLAs, and a feature attribution algorithm to infer the reason. 
Causal inference and dependency/graph learning may also be used~\cite{heckerman1996causal,mandros2017discovering,zhang2020statistical,loh2014high,raskutti2018learning,nori2019interpretml,zheng2018hound} for these applications. However, in our work, where there is a large number of feature dimensions and complex correlation between groups of features, such methods require manual input to tune the dependency structure \edit{such as adding or deleting a detected dependency link} and might still be biased. \edit{In our work, we do not manually craft dependencies among causes of variation but use Shapley scores for inference.}
% , considering occasional slowdowns less predictable. We want to unravel the causes of the unpredictability and variation, which is the key to provide more reliable services as customers are looking for consistency in the job runtime.

% \subsection{Causal inference and Dependency/Graph Learning}

% Causal Independence for Probability Assessment and Inference Using Bayesian Networks ~\cite{heckerman1996causal}.

% Discovering Reliable Approximate Functional Dependencies~\cite{mandros2017discovering}

% A statistical perspective on discovering functional dependencies in noisy data~\cite{zhang2020statistical}

% High-Dimensional Learning of Linear Causal Networks via Inverse Covariance Estimation~\cite{loh2014high}

% Learning directed acyclic graph models based on sparsest permutations~\cite{raskutti2018learning}

% InterpretML: A Unified Framework for Machine Learning Interpretability~\cite{nori2019interpretml}

% Hound: Causal Learning for Datacenter-scale Straggler Diagnosis~\cite{zheng2018hound}

Huang et al.~\cite{huang2016identifying, huang2017top} investigated the causes for query latency variation in transactional databases.
% and proposed new locking and scheduling methods for more predictable performance. 
%They introduced a novel profiling and source code instrumentation framework, 
They used variance (and covariance) as the primary metric for quantifying variation and built a variance tree corresponding to the call graph for gaining insights into the contributors of variance. In contrast, we use runtime \textit{distributions} for predicting variation, instead of scalar metrics due to the insufficiency of the latter in fully characterizing or explaining variation. Additionally, we use feature importance and Shapley scores to identify the main contributors to the prediction for the distribution to which a new run of a job may belong.

Prior work has also explored reducing performance variation with concurrent queries. Crescando~\cite{unterbrunner2009predictable} presents a relational table implementation that prioritizes predictable query performance 
%for a range of update loads and diverse/evolving queries 
over optimal performance 
%at low update loads or for a given workload, 
through design choices such as having a scan-only architecture without indexes and new collaborative scan and update-join algorithms. CJOIN~\cite{candea2011predictable} introduces a new join operator and shares computation and resources among concurrent queries to improve both throughput and performance stability. Augmenting our prescriptive analysis with capabilities for evaluating the impact of computation sharing and other optimizations for concurrent queries is an interesting direction for future work. 

\edit{For tuning job performance, Black-box optimization such as Bayesian optimization~\cite{bishop2006pattern,curino2020mlos}, gradient descent~\cite{zhang2019end,van2017automatic}, etc. requires multiple runs of experiments. In this work, we provide a one-shot method that can directly determine the best course of action.
}

==> Runtime Variation in Distributed Systems (Short II) (2)/Results/Experiments.tex <==
\section{Experiment}\label{sec:exp}
Bayesian net

Randomforest

Boosting Machine


==> Runtime Variation in Distributed Systems (Short II) (2)/abstract.tex <==
%!TEX root = main.tex


% Cloud and serverless computing platforms offer tremendous advantages to users compared to on-premises compute, by provisioning resources on demand, handling scalability at ease, and transparently managing the needs of security and availability. However, the dynamic nature of resource allocations and runtime conditions on such platforms can result in high variability in a job’s runtime across multiple iterations, a lack of understanding of which can result in a poor experience for the user. Identifying the sources of such variation and being able to predict and adjust for them is also important to cloud service providers for designing reliable data processing pipelines, provisioning and allocating resources, pricing services and meeting SLOs, and debugging performance hazards. 

% %Hence, it is imperative to understand the sources of runtime variation as we have done in this work.  
%  %One such example is Cosmos, an exabyte-scale analytics platform at Microsoft that hosts millions of production SCOPE  jobs. 
 
% In this paper we analyze the runtime variation of millions of production \scope jobs on \cosmos, an exabyte-scale analytics platform at Microsoft, by accounting for 
% %Cosmos jobs runtime distributions as determined by 
% factors such as job plan characteristics and inputs, resource allocation, cluster heterogeneity and utilization, and scheduling policies.   
% %Plotting predicted versus actual runtime revealed consistent off-diagonal patterns, including subsets of jobs that run faster than expected, and other subsets   that run with characteristic patterns of fixed delays.
% Clustering of jobs reveals significantly different distributions of runtimes with characteristic long tails. We propose novel methods to predict runtime distribution categories for incoming jobs, with an average accuracy of >95\%, using interpretable machine-learning models trained on a large corpus of historical data. While we cannot predict which individual cases will end up in these subsets, we can make useful predictions of the probability distribution of the runtime for an individual job. To the best of our knowledge, this is the first study on predicting categories of runtime distribution for enterprise analytics workloads at scale. We also show how our methods can be used for analyzing what-if scenarios about the impact of resource allocation, scheduling, and cluster provisioning decisions on a job’s runtime consistency and predictability.


\begin{abstract}

% Cloud and serverless computing platforms offer tremendous advantages to users compared to on-premises compute, by provisioning resources on demand, handling scalability at ease, and transparently managing the needs of security and availability.
The dynamic nature of resource allocation and runtime conditions on Cloud
% and serverless computing platforms 
can result in high variability in a job’s runtime across multiple iterations, leading to a poor experience.
% for the users who expect reliable services.
Identifying the sources of such variation and being able to predict and adjust for them is crucial to cloud service providers to design reliable data processing pipelines, provision and allocate resources, adjust pricing services, meet SLOs and debug performance hazards.

In this paper, we analyze the runtime variation of millions of production \scope jobs on \cosmos, an exabyte-scale internal analytics platform at Microsoft.
We propose an innovative 2-step approach to predict job runtime distribution by characterizing typical distribution shapes combined with a classification model with an average accuracy of >96\%,
% , using an innovative interpretable machine-learning algorithm
out-performing traditional regression models and better capturing long tails.
We examine factors such as job plan characteristics and inputs, resource allocation, physical cluster heterogeneity and utilization, and scheduling policies.
% which all impact a system's runtime.   
% Using clustering analysis, we identify different runtime distributions with characteristic long tails.

To the best of our knowledge, this is the first study on predicting categories of runtime distributions for enterprise analytics workloads at scale.
Furthermore, we examine how our methods can be used to analyze what-if scenarios, focusing on the impact of resource allocation, scheduling, and physical cluster provisioning decisions on a job’s runtime consistency and predictability.
\end{abstract}


==> Runtime Variation in Distributed Systems (Short II) (2)/runtime_variation.tex <==
% Notes on the current version  
% JMA  24 Feb 2022
\section{Characterizing Runtime Variation}
\label{sec:metrics}

We now discuss how we characterize and quantify runtime variation for recurring jobs. This will form the basis for our prediction strategy that we discuss in Section~\ref{sec:model}.

\subsection{Measuring Variation}
\label{sec:variation}
\jma{
"Variation" is a term we use to refer generally to the need to look beyond a single predicted job runtime value, to the probability distribution as it depends on the job and its features. As we will show, runtime distributions have characteristically long tails, with some fraction of their mass appearing in modes of the distribution an order of magnitude or more above the distribution mean. Statistics derived from the distribution variance are inadequate to describe these extremes, in fact, for such distributions, the variance may not exist and conventional fitting techniques do not apply. \cite{Clauset2009} We resort instead to histograms of the empirical distribution of runtimes from which we can estimate the ``excess''; the probability mass of a runtime occuring above a given threshold value. 
}

\jma{
Prediction from the models we employ do not capture the distribution tail structure, despite having conventionally measured accuracies above 95\%. This is evident in the error plots of predicted versus actual runtime, shown in Figure 4. A notable artifact visible in these plots is an``icicle'' mode at a constant offset from the main mode of between XX and YY minutes. For a user, knowing the probability a job may fall in such an extreme mode is valuable, even if we cannot predict with high certainty that it will. 
}

\jma{
The standard regression technique to predict extreme values relies on quantile regression---a non-parametric method that finds a regression line offset at a specified quantile as a function of the independent variables. \cite{Kroenker1978} Sadly, as the error plot shows, we do not have the luxury of employing this method, since predicted values do not capture the extreme values in the tail structure as observed in actual runtime distributions. 
Our challenge is to find an alternative way to estimate the extremes of runtime distributions. 
}

\jma{
As an alternative, we demonstrate that runtimes can be grouped into a collection of clusters, each with a measureable runtime distribution, and for any job, we can predict the cluster it belongs to. Then we ascribe to the job the cluster's characteristic runtime distribution.  Thus we have a sound and workable method to estimate a job's runtime distribution and so the probability that its runtime will fall above a specified threshold. 
}

\jma{
A straightforward demonstration of this is to create clusters by dividing predicted runtimes into 10 horizontal bands as shown in Figure X, and considering the {\it actual} runtimes in that band as characteristic of the runtime distribution of any job whose predicted value falls in that band. We call these ``decile'' custers, since each consists of one decile of the predicted runtimes.  {\it The novelty of our approach is to be able to estimate these excess probabilities despite not having a predictor of individual job runtimes that directly predicts the excess, but instead associates the job with the distribution of the cluster it belongs to.} This method's accuracy is testable by comparing the probability over a set of predictions with their distribution of the set, as we show.
}

\jma{
The presumption of using ``decile'' clusters is that jobs with similar predicted runtimes will have similar runtime distributions.  Another reasonable clustering criterion is that jobs from the same job group share distributions, and that it makes sense to cluster groups by similarity among actual runtime distributions. This is the method we present in the bulk of the paper.  
}

% [1]
% @article{2009,
%   title={Power-Law Distributions in Empirical Data},
%   volume={51},
%   ISSN={1095-7200},
%   url={http://dx.doi.org/10.1137/070710111},
%   DOI={10.1137/070710111},
%   number={4},
%   journal={SIAM Review},
%   publisher={Society for Industrial & Applied Mathematics (SIAM)},
%   author={Clauset, Aaron and Shalizi, Cosma Rohilla and Newman, M. E. J.},
%   year={2009},
%   month={Nov},
%   pages={661–703} }

% [2] Koenker, R. W. and Bassett, G. W. (1978). Regression  quantiles, Econometrica, 46, 33–50.


==> runtime_variation.tex <==
% Notes on the current version  
% JMA  24 Feb 2022
\section{Characterizing Runtime Variation}
\label{sec:metrics}

We now discuss how we characterize and quantify runtime variation for recurring jobs. This will form the basis for our prediction strategy that we discuss in Section~\ref{sec:model}.

\subsection{Measuring Variation}
\label{sec:variation}
\jma{
"Variation" is a term we use to refer generally to the need to look beyond a single predicted job runtime value, to the probability distribution as it depends on the job and its features. As we will show, runtime distributions have characteristically long tails, with some fraction of their mass appearing in modes of the distribution an order of magnitude or more above the distribution mean. Statistics derived from the distribution variance are inadequate to describe these extremes, in fact, for such distributions, the variance may not exist and conventional fitting techniques do not apply. \cite{Clauset2009} We resort instead to histograms of the empirical distribution of runtimes from which we can estimate the ``excess''; the probability mass of a runtime occuring above a given threshold value. 
}

\jma{
Prediction from the models we employ do not capture the distribution tail structure, despite having conventionally measured accuracies above 95\%. This is evident in the error plots of predicted versus actual runtime, shown in Figure 4. A notable artifact visible in these plots is an``icicle'' mode at a constant offset from the main mode of between XX and YY minutes. For a user, knowing the probability a job may fall in such an extreme mode is valuable, even if we cannot predict with high certainty that it will. 
}

\jma{
The standard regression technique to predict extreme values relies on quantile regression---a non-parametric method that finds a regression line offset at a specified quantile as a function of the independent variables. \cite{Kroenker1978} Sadly, as the error plot shows, we do not have the luxury of employing this method, since predicted values do not capture the extreme values in the tail structure as observed in actual runtime distributions. 
Our challenge is to find an alternative way to estimate the extremes of runtime distributions. 
}

\jma{
As an alternative, we demonstrate that runtimes can be grouped into a collection of clusters, each with a measureable runtime distribution, and for any job, we can predict the cluster it belongs to. Then we ascribe to the job the cluster's characteristic runtime distribution.  Thus we have a sound and workable method to estimate a job's runtime distribution and so the probability that its runtime will fall above a specified threshold. 
}

\jma{
A straightforward demonstration of this is to create clusters by dividing predicted runtimes into 10 horizontal bands as shown in Figure X, and considering the {\it actual} runtimes in that band as characteristic of the runtime distribution of any job whose predicted value falls in that band. We call these ``decile'' custers, since each consists of one decile of the predicted runtimes.  {\it The novelty of our approach is to be able to estimate these excess probabilities despite not having a predictor of individual job runtimes that directly predicts the excess, but instead associates the job with the distribution of the cluster it belongs to.} This method's accuracy is testable by comparing the probability over a set of predictions with their distribution of the set, as we show.
}

\jma{
The presumption of using ``decile'' clusters is that jobs with similar predicted runtimes will have similar runtime distributions.  Another reasonable clustering criterion is that jobs from the same job group share distributions, and that it makes sense to cluster groups by similarity among actual runtime distributions. This is the method we present in the bulk of the paper.  
}

% [1]
% @article{2009,
%   title={Power-Law Distributions in Empirical Data},
%   volume={51},
%   ISSN={1095-7200},
%   url={http://dx.doi.org/10.1137/070710111},
%   DOI={10.1137/070710111},
%   number={4},
%   journal={SIAM Review},
%   publisher={Society for Industrial & Applied Mathematics (SIAM)},
%   author={Clauset, Aaron and Shalizi, Cosma Rohilla and Newman, M. E. J.},
%   year={2009},
%   month={Nov},
%   pages={661–703} }

% [2] Koenker, R. W. and Bassett, G. W. (1978). Regression  quantiles, Econometrica, 46, 33–50.

